HELMHOLTZ: A Verifier for Tezos Smart Contracts Based on Refinement Types

A smart contract is a program executed on a blockchain, based on which many cryptocurrencies are implemented, and is being used for automating transactions. Due to the large amount of money that smart contracts deal with, there is a surging demand for a method that can statically and formally verify them. This article describes our type-based static verification tool HELMHOLTZ for Michelson, which is a statically typed stack-based language for writing smart contracts that are executed on the blockchain platform Tezos. HELMHOLTZ is designed on top of our extension of Michelson's type system with refinement types. HELMHOLTZ takes a Michelson program annotated with a user-defined specification written in the form of a refinement type as input; it then typechecks the program against the specification based on the refinement type system, discharging the generated verification conditions with the SMT solver Z3. We briefly introduce our refinement type system for the core calculus Mini-Michelson of Michelson, which incorporates the characteristic features such as compound datatypes (e.g., lists and pairs), higher-order functions, and invocation of another contract. \HELMHOLTZ{} successfully verifies several practical Michelson programs, including one that transfers money to an account and that checks a digital signature.

==> figures/tsyntax.tex <==
\begin{grammar}
  \scriptsize
    <annotation> ::= \ 
    \alt "Assert" $\Phi$
    $\mid$ "Assume" $\Phi$
    $\mid$ "LoopInv" $\Phi$
    \alt "LambdaAnnot" $\Phi_{{\mathrm{1}}} \rightarrow \Phi_{{\mathrm{2}}} " & " \Phi_{{\mathrm{3}}}\ (\ottmv{x_{{\mathrm{1}}}}:\ottnt{T_{{\mathrm{1}}}},\dots,\ottmv{x_{\ottmv{n}}}:\ottnt{T_{\ottmv{n}}})$ % $\Phi$ "->" $\Phi$ "&" $\Phi$ "(" $\ottmv{x_{{\mathrm{1}}}}$ ":" $\ottnt{T_{{\mathrm{1}}}}$, ..., $\ottmv{x_{\ottmv{n}}}$ ":" $\ottnt{T_{\ottmv{n}}}$ ")" % \{"," <var> ":" <sort>\} ")"]
    \alt "Measure" $\ottmv{x} : \ottnt{T_{{\mathrm{1}}}} \rightarrow \ottnt{T_{{\mathrm{2}}}}$ "where" $p_1 = e_1 \mid \dots \mid p_n = e_n$
    \alt "ContractAnnot" $\Phi_{{\mathrm{1}}} \rightarrow \Phi_{{\mathrm{2}}} " & " \Phi_{{\mathrm{3}}} (\ottmv{x_{{\mathrm{1}}}}:\ottnt{T_{{\mathrm{1}}}},\dots,\ottmv{x_{\ottmv{n}}}:\ottnt{T_{\ottmv{n}}})$

    % <rtype> ::= "{" <pattern> \{":" <pattern>\} "|" <exp> "}"

\iffullver
    <exp> ::= "(" <exp> ")"
    | <number>
    | <string>
    | <bytes>
    | <op> \{<exp>\}
    | <exp> <bop> <exp>
    | "Key" <string>
    | "Address" <string>
    | <exp> "." <accessor>
    | "if" <exp> "then" <exp> "else" <exp>
    | <constructor> \{<exp>\}
    | <exp> "," <exp>
    | "[" "]"
    | "[" <exp> \{";" <exp>\} "]"
    | "match" <exp> "with" ["|"] <patterns>

    <op> ::= <var> | "-" | "!" | "source" | "sender" | "self" | "now" |
    "balance" | "amount" | "empty_map" | "empty_set" | "not" | "first" |
    "second" | "unpack" | "data" | "hash" | "blake2b" | "sha512" | "get_str" |
    "find_opt" | "mem" | "add" | "remove" | "sig" | "update" | "call"

    <bop> ::= "+" | "-" | "*" | "/" | "<" | ">" | "<=" | ">=" | "=" | "<>" |
    "&&" | "||" | "mod" | "::"

    <accessor> ::= "first" | "second"

    <patterns> ::= <pattern> "->" <exp> \{"|" <pattern> "->" <exp>\}

    <pattern> ::= "(" <pattern> ")"
    | <constructor> ["<" <sort> ">"] \{<pattern>\}
    | <pattern> "," <pattern>
    | <pattern> "::" <pattern>
    | "[" "]"
    | "[" <pattern> \{";" <pattern>\} "]"
    | <var>
    | "_"

    <sort> ::= "(" <sort> ")" | "int" | "unit" | "nat" | "mutez" | "timestamp" |
    "bool" | "string" | "bytes" | "key" | "address" | "signature" | "operation"
    | "pair" <sort> <sort> | "list" <sort> | "contract" <sort> | "option" <sort>
    | "or" <sort> <sort> | "fun" <sort> <sort> | "map" <sort> <sort> | "set"
    <sort> <sort>

    <constructor> ::= "Nil" | "Cons" | "Left" | "Right" | "Some" | "None" |
    "True" | "False" | "Unit" | "Pack" | "Contract" | "SetDelegate" |
    "TransferTokens" | "Error" | "Overflow" | "EmptyMap" | "Bind" | "EmptySet" |
    "Add"
\fi
\end{grammar}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper.otex"
%%% End:


==> proofs/correctnessAuxStatements.tex <==
\begin{prop}[name=Correctness of loop invariant]{typing/sound/loop}
  If
  \begin{gather}
    \left(
      \begin{split}
        \text{For any } & \ottnt{S'_{{\mathrm{1}}}}, \ottnt{S'_{{\mathrm{2}}}}, \\
        \text{ if } & \ottnt{S'_{{\mathrm{1}}}}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S'_{{\mathrm{2}}}} \text{ and } \\
        & \sigma  \ottsym{:}  \Gamma  \models  \ottnt{S'_{{\mathrm{1}}}}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \neq  0  \ottsym{\}}, \\
        \text{ then } & \sigma  \ottsym{:}  \Gamma  \models  \ottnt{S'_{{\mathrm{2}}}}  \ottsym{:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}}
      \end{split}
    \right) \hyp{OIH}\\
    \ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{LOOP} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{eval}\\
    \sigma  \ottsym{:}  \Gamma  \models  \ottnt{S_{{\mathrm{1}}}}  \ottsym{:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{semty}
  \end{gather}
  then \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{S_{{\mathrm{2}}}}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  0  \ottsym{\}}\).

  \proof The proof is done by induction on the given derivation of
  \hypref{eval}.
  \begin{match}
  \item[\ruleref{E-LoopT}] We have
    \begin{gather}
      \ottnt{i}  \neq  0 \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{i}  \triangleright  \ottnt{S}  \hyp{2}\\
      \ottnt{S}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S'} \hyp{3}\\
      \ottnt{S'}  \vdash  \ottkw{LOOP} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{4}
    \end{gather}
    for some \(\ottnt{i}\), \(\ottnt{S}\), and \(\ottnt{S'}\).  By
    \propref{semty/logic}, \hypref{semty}, and \hypref{2}, we have
    \begin{gather}
      \sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{i}  \ottsym{\}} \hyp{5}.
    \end{gather}
    By \propref{semty/logic/imply}, \propref{semty/wf}, \propref{fol/thm/misc(if-t)}, \hypref{1},
    and \hypref{5}, we have
    \begin{gather}
      \sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \neq  0  \ottsym{\}} \hyp{6}.
    \end{gather}
    By \hypref{OIH}, \hypref{3}, and \hypref{6}, we have
    \begin{gather}
      \sigma  \ottsym{:}  \Gamma  \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{7}.
    \end{gather}
    Now the goal follows from applying IH of \hypref{4} to \hypref{7}.

  \item[\ruleref{E-LoopF}] We have the following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} 0  \triangleright  \ottnt{S_{{\mathrm{2}}}}  \hyp{1}
    \end{gather}
    So the goal follows by \propref{semty/logic}, \hypref{semty}, and
    \hypref{1}.  \qedhere
  \end{match}
\end{prop}


\begin{prop}[name=Correctness of iter invariant]{typing/sound/iter}
  If
  \begin{gather}
    \ottmv{x_{{\mathrm{1}}}}  \neq  \ottmv{x_{{\mathrm{2}}}} \hyp{fv1}\\
     \ottmv{x_{{\mathrm{1}}}}  \notin   \text{dom}( \Gamma  \ottsym{,}   \widehat{  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon }  )   \hyp{fv2}\\
     \ottmv{x_{{\mathrm{2}}}}  \notin   \text{dom}( \Gamma  \ottsym{,}   \widehat{  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon }  )   \hyp{fv3}\\
    \left(
      \begin{split}
        \text{For any } & \ottnt{S'_{{\mathrm{1}}}}, \ottnt{S'_{{\mathrm{2}}}}, \sigma', \\
        \text{ if } & \ottnt{S'_{{\mathrm{1}}}}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S'_{{\mathrm{2}}}}, \text{ and }\\
        & \sigma'  \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \models  \ottnt{S'_{{\mathrm{1}}}}  \ottsym{:}  \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{\}},\\
        \text{ then } & \sigma'  \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \models  \ottnt{S'_{{\mathrm{2}}}}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{\}}
      \end{split}
    \right) \hyp{OIH}\\
    \ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{ITER} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{eval}\\
    \sigma  \ottsym{:}  \Gamma  \models  \ottnt{S_{{\mathrm{1}}}}  \ottsym{:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{semty}
  \end{gather}
  then \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{S_{{\mathrm{2}}}}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  \ottsym{\}}\).

  \proof The proof is done by induction on the given derivation of
  \hypref{eval}.
  \begin{match}
  \item[\ruleref{E-IterNil}] We have
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{[}  \ottsym{]}  \triangleright  \ottnt{S_{{\mathrm{2}}}}  \hyp{1}.
    \end{gather}
    So the goal follows by \propref{semty/logic}, \hypref{semty}, and
    \hypref{1}.

  \item[\ruleref{E-IterCons}] We have the following hypothesis for some
    \(\ottnt{V_{{\mathrm{1}}}}\), \(\ottnt{V_{{\mathrm{2}}}}\), \(\ottnt{S}\), and \(\ottnt{S'}\).
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{1}\\
      \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{S}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S'} \hyp{2}\\
      \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S'}  \vdash  \ottkw{ITER} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{3}
    \end{gather}
    By \propref{semty/logic}, \hypref{semty}, and \hypref{1}, we have
    \begin{gather}
      \sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \ottsym{\}} \hyp{5}.
    \end{gather}
    By \propref{semty/logic/imply}, \propref{semty/wf}, \propref{fol/thm/misc(if-cons)},
    \hypref{fv1}, \hypref{fv2}, \hypref{fv3}, and \hypref{5}, we have
    \begin{gather}
      \sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{\}} \hyp{6}.
    \end{gather}
    By \propref{semty/logic}, and \hypref{6}, we have
    \begin{gather}
       \sigma  [  \ottmv{x_{{\mathrm{2}}}}  \mapsto  \ottnt{V_{{\mathrm{2}}}}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{\}} \hyp{7}.
    \end{gather}
    By \propref{semty/logic} and \hypref{7}, We have
    \begin{gather}
       \sigma  [  \ottmv{x_{{\mathrm{2}}}}  \mapsto  \ottnt{V_{{\mathrm{2}}}}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \models  \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{S}  \ottsym{:}  \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{\}} \hyp{10}
    \end{gather}
    Now we can have
    \begin{gather}
       \sigma  [  \ottmv{x_{{\mathrm{2}}}}  \mapsto  \ottnt{V_{{\mathrm{2}}}}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{\}}
      \hyp{12}
    \end{gather}
    by \hypref{OIH}, \hypref{2}, and \hypref{10}.  By
    \propref{semty/logic} and \hypref{12}, we have
    \begin{gather}
      \sigma  \ottsym{:}  \Gamma  \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{\}} \hyp{13}.
    \end{gather}
    By \propref{semty/wf} and \hypref{semty}, we have
    \( \Gamma  \ottsym{,}   \widehat{  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon }    \vdash   \varphi  : \mathord{*} \), and so by
    \propref{fol/wf/strut(f-closed)}, we have
    \(  \text{fvars}( \varphi )   \subseteq   \text{dom}( \Gamma  \ottsym{,}   \widehat{  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon }  )  \).  Therefore,
    \begin{gather}
       \ottmv{x_{{\mathrm{2}}}}  \notin   \text{fvars}( \varphi )   \hyp{13.1}
    \end{gather}
    follows by \hypref{fv3}.  By \propref{semty/logic/imply}, \propref{semty/wf},
    \propref{fol/thm/misc(iter)}, \hypref{13}, and \hypref{13.1}, we have
    \begin{gather}
      \sigma  \ottsym{:}  \Gamma  \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{\}} \hyp{14}.
    \end{gather}
    Now we can have
    \begin{gather}
      \sigma  \ottsym{:}  \Gamma  \models  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S'}  \ottsym{:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{15}
    \end{gather}
    by \propref{semty/logic} and \hypref{14}.  So the goal follows by
    applying IH of \hypref{3} to \hypref{15}.  \qedhere
  \end{match}
\end{prop}


==> proofs/eval.tex <==
\subsection{Soundness of the simple type system}

\begin{prop}[name=Inversion for the evaluation]{eval/inv} Every following statement holds.
  \begin{statements}
  \item[nop] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottsym{\{}  \ottsym{\}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{S_{{\mathrm{2}}}} \).
  \item[seq] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottsym{\{}  \ottnt{I}  \ottsym{;}  \mathit{IS}  \ottsym{\}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottnt{I}  \Downarrow  \ottnt{S}\) and
    \(\ottnt{S}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\) for some $\ottnt{S}$.
  \item[dip] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{DIP} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S'_{{\mathrm{1}}}} \),
    \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S'_{{\mathrm{2}}}} \), and \(\ottnt{S'_{{\mathrm{1}}}}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S'_{{\mathrm{2}}}}\) for some $\ottnt{V}$,
    $\ottnt{S'_{{\mathrm{1}}}}$, and $\ottnt{S'_{{\mathrm{2}}}}$.
  \item[drop] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{DROP}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S_{{\mathrm{2}}}} \) for some
    $\ottnt{V}$.
  \item[dup] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{DUP}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S} \) and
    \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{V}  \triangleright  \ottnt{S} \) for some $\ottnt{V}$ and $\ottnt{S}$.
  \item[swap] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{SWAP}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S} \) and
    \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{S} \) for some $\ottnt{V_{{\mathrm{1}}}}$, $\ottnt{V_{{\mathrm{2}}}}$, and $\ottnt{S}$.
  \item[push] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{PUSH} \, \ottnt{T} \, \ottnt{V}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S_{{\mathrm{1}}}} \).
  \item[not] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{NOT}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then either
    \begin{itemize}
    \item \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{i}  \triangleright  \ottnt{S} \), \(\ottnt{i}  \neq  0\), and \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=} 0  \triangleright  \ottnt{S} \) for some
      $\ottnt{i}$ and $\ottnt{S}$; or
    \item \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} 0  \triangleright  \ottnt{S} \) and \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=} 1  \triangleright  \ottnt{S} \) for some $\ottnt{S}$.
    \end{itemize}
  \item[add] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{ADD}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{i_{{\mathrm{1}}}}  \triangleright  \ottnt{i_{{\mathrm{2}}}}  \triangleright  \ottnt{S} \),
    \( \ottnt{i_{{\mathrm{1}}}}  \ottsym{+}  \ottnt{i_{{\mathrm{2}}}} \ottsym{=} \ottnt{i_{{\mathrm{3}}}} \), and \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{i_{{\mathrm{3}}}}  \triangleright  \ottnt{S} \) for some $\ottnt{i_{{\mathrm{1}}}}$, $\ottnt{i_{{\mathrm{2}}}}$,
    $\ottnt{i_{{\mathrm{3}}}}$, and $\ottnt{S}$.
  \item[pair] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{PAIR}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S} \) and
    \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \triangleright  \ottnt{S} \) for some $\ottnt{V_{{\mathrm{1}}}}$, $\ottnt{V_{{\mathrm{2}}}}$, and $\ottnt{S}$.
  \item[car] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{CAR}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \triangleright  \ottnt{S} \) and
    \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{S} \) for some $\ottnt{V_{{\mathrm{1}}}}$, $\ottnt{V_{{\mathrm{2}}}}$, and $\ottnt{S}$.
  \item[cdr] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{CDR}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \triangleright  \ottnt{S} \) and
    \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S} \) for some $\ottnt{V_{{\mathrm{1}}}}$, $\ottnt{V_{{\mathrm{2}}}}$, and $\ottnt{S}$.
  \item[nil] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{NIL} \, \ottnt{T}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottsym{[}  \ottsym{]}  \triangleright  \ottnt{S_{{\mathrm{1}}}} \).
  \item[cons] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{CONS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S} \) and
    \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S} \) for some $\ottnt{V_{{\mathrm{1}}}}$, $\ottnt{V_{{\mathrm{2}}}}$, and $\ottnt{S}$.
  \item[if] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{IF} \, \mathit{IS}_{{\mathrm{1}}} \, \mathit{IS}_{{\mathrm{2}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then either
    \begin{itemize}
    \item \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{i}  \triangleright  \ottnt{S} \), \(\ottnt{i}  \neq  0\), and \(\ottnt{S}  \vdash  \mathit{IS}_{{\mathrm{1}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\) for
      some $\ottnt{i}$ and $\ottnt{S}$; or
    \item \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} 0  \triangleright  \ottnt{S} \) and \(\ottnt{S}  \vdash  \mathit{IS}_{{\mathrm{2}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\) for some $\ottnt{S}$.
    \end{itemize}
  \item[loop] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{LOOP} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then there are two cases:
    \begin{itemize}
    \item \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{i}  \triangleright  \ottnt{S'_{{\mathrm{1}}}} \), \(\ottnt{i}  \neq  0\), \(\ottnt{S'_{{\mathrm{1}}}}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S}\), and
      \(\ottnt{S}  \vdash  \ottkw{LOOP} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\) for some $\ottnt{i}$, $\ottnt{S'_{{\mathrm{1}}}}$, and $\ottnt{S}$; or
    \item \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} 0  \triangleright  \ottnt{S_{{\mathrm{2}}}} \).
    \end{itemize}
  \item[ifcons] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \texttt{IF\symbol{95}CONS} \, \mathit{IS}_{{\mathrm{1}}} \, \mathit{IS}_{{\mathrm{2}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then either
    \begin{itemize}
    \item \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S} \) and \(\ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \vdash  \mathit{IS}_{{\mathrm{1}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\) for
      some $\ottnt{V_{{\mathrm{1}}}}$, $\ottnt{V_{{\mathrm{2}}}}$, and $\ottnt{S}$; or
    \item \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{[}  \ottsym{]}  \triangleright  \ottnt{S} \) and \(\ottnt{S}  \vdash  \mathit{IS}_{{\mathrm{2}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\) for some $\ottnt{S}$.
    \end{itemize}
  \item[iter] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{ITER} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then either
    \begin{itemize}
    \item \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S'_{{\mathrm{1}}}} \), \(\ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{S'_{{\mathrm{1}}}}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S}\), and
      \(\ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \vdash  \ottkw{ITER} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\) for some $\ottnt{V_{{\mathrm{1}}}}$, $\ottnt{V_{{\mathrm{2}}}}$, $\ottnt{S'_{{\mathrm{1}}}}$
      and $\ottnt{S}$; or
    \item \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{[}  \ottsym{]}  \triangleright  \ottnt{S_{{\mathrm{2}}}} \).
    \end{itemize}
  \item[lambda] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{LAMBDA} \, \ottnt{T_{{\mathrm{1}}}} \, \ottnt{T_{{\mathrm{2}}}} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then
    \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=}  \langle  \mathit{IS}  \rangle   \triangleright  \ottnt{S_{{\mathrm{1}}}} \).
  \item[exec] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{EXEC}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright   \langle  \mathit{IS}  \rangle   \triangleright  \ottnt{S} \),
    \(\ottnt{V_{{\mathrm{1}}}}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Downarrow  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ddagger\), and \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S} \) for some
    $\ottnt{V_{{\mathrm{1}}}}$, $\ottnt{V_{{\mathrm{2}}}}$, $\mathit{IS}$, and $\ottnt{S}$.
  \item[transfertokens] If \(\ottnt{S_{{\mathrm{1}}}}  \vdash  \texttt{TRANSFER\symbol{95}TOKENS} \, \ottnt{T}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), then
    \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{i}  \triangleright  \ottnt{a}  \triangleright  \ottnt{S} \) and \( \ottnt{S_{{\mathrm{2}}}} \ottsym{=}  \texttt{Transfer}  (  \ottnt{V} ,  \ottnt{i} ,  \ottnt{a}  )   \triangleright  \ottnt{S} \) for
    some $\ottnt{V}$, $\ottnt{i}$, $\ottnt{a}$, and $\ottnt{S}$.
  \end{statements}

  \proof Easy by definition.
\end{prop}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper.otex"
%%% End:


==> proofs/fol.tex <==
\subsection{Properties for assertion language}


\begin{prop}{fol/wf/inv}
  Every following statement holds.
  \begin{statements}
  \item[equal] If \( \Gamma   \vdash   \ottmv{x}  \ottsym{=}  \ottnt{t}  : \mathord{*} \) and \(\Gamma  \vdash  \ottmv{x}  \ottsym{:}  \ottnt{T}\), then \(\Gamma  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T}\).
  \item[call] If \( \Gamma   \vdash    \ottkw{call} ( \ottnt{t_{{\mathrm{1}}}} ,  \ottmv{x} ) =  \ottmv{y}   : \mathord{*} \), \(\Gamma  \vdash  \ottmv{x}  \ottsym{:}  \ottnt{T_{{\mathrm{1}}}}\), and
    \(\Gamma  \vdash  \ottmv{y}  \ottsym{:}  \ottnt{T_{{\mathrm{2}}}}\), then \(\Gamma  \vdash  \ottnt{t_{{\mathrm{1}}}}  \ottsym{:}  \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}\).
  \item[and] If \( \Gamma   \vdash   \varphi_{{\mathrm{1}}}  \wedge  \varphi_{{\mathrm{2}}}  : \mathord{*} \), then \( \Gamma   \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) and \( \Gamma   \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \).
  \item[imply] If \( \Gamma   \vdash   \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}}  : \mathord{*} \), then \( \Gamma   \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) and \( \Gamma   \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \).
  \item[exists] If \( \Gamma   \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  : \mathord{*} \), then \( \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}    \vdash   \varphi  : \mathord{*} \).
  \end{statements}

  \proof Easy by definition.  Note that restricting some sub-terms to variables
  in (1) and (2) is important because a sort of a term is not unique in general.
\end{prop}


\begin{prop}{fol/wf/strut}
  Every following statement holds.
  \begin{statements}
  \item[t-closed] If \(\Gamma  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T}\), then \(  \text{fvars}( \ottnt{t} )   \subseteq   \text{dom}( \Gamma )  \).
  \item[f-closed] If \( \Gamma   \vdash   \varphi  : \mathord{*} \), then \(  \text{fvars}( \varphi )   \subseteq   \text{dom}( \Gamma )  \).
  \item[t-perm] If \(\Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}  \Gamma'  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T''}\), then
    \(\Gamma  \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma'  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T''}\).
  \item[f-perm] If \( \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}  \Gamma'   \vdash   \varphi  : \mathord{*} \), then
    \( \Gamma  \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma'   \vdash   \varphi  : \mathord{*} \).
  \item[t-weaken] If \( \ottmv{x}  \notin   \text{dom}( \Gamma  \ottsym{,}  \Gamma' )  \) and \(\Gamma  \ottsym{,}  \Gamma'  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T}\), then
    \(\Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}  \Gamma'  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T}\).
  \item[f-weaken] If \( \ottmv{x}  \notin   \text{dom}( \Gamma  \ottsym{,}  \Gamma' )  \) and \( \Gamma  \ottsym{,}  \Gamma'   \vdash   \varphi  : \mathord{*} \), then
    \( \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}  \Gamma'   \vdash   \varphi  : \mathord{*} \).
  \item[t-drop] If \( \ottmv{x}  \notin   \text{fvars}( \ottnt{t} )  \) and \(\Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma'  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T}\), then
    \(\Gamma  \ottsym{,}  \Gamma'  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T}\).
  \item[f-drop] If \( \ottmv{x}  \notin   \text{fvars}( \varphi )  \) and \( \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma'   \vdash   \varphi  : \mathord{*} \), then
    \( \Gamma  \ottsym{,}  \Gamma'   \vdash   \varphi  : \mathord{*} \).
  \end{statements}

  \proof The proof is straightforward by induction on the given well-sortedness
  derivation.  Some proofs depend on former results.
\end{prop}


\begin{prop}{fol/strut}
  Every following statement holds.
  \begin{statements}
  \item[t-perm] \( \lBrack  \ottnt{t}  \rBrack_{ \sigma : \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}  \Gamma' }   \ottsym{=}   \lBrack  \ottnt{t}  \rBrack_{ \sigma : \Gamma  \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma' } \).
  \item[f-perm] If \(\sigma  \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}  \Gamma'  \models  \varphi\), then
    \(\sigma  \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma'  \models  \varphi\).
  \item[t-weaken] If \( \ottmv{x}  \notin   \text{dom}( \Gamma  \ottsym{,}  \Gamma' )  \) and \( \sigma  \ottsym{(}  \ottmv{x}  \ottsym{)}  :  \ottnt{T} \), then \( \lBrack  \ottnt{t}  \rBrack_{ \sigma : \Gamma  \ottsym{,}  \Gamma' }   \ottsym{=}   \lBrack  \ottnt{t}  \rBrack_{ \sigma : \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma' } \).
  \item[f-weaken] If \( \ottmv{x}  \notin   \text{dom}( \Gamma  \ottsym{,}  \Gamma' )  \), \( \sigma  \ottsym{(}  \ottmv{x}  \ottsym{)}  :  \ottnt{T} \),  and \(\sigma  \ottsym{:}  \Gamma  \ottsym{,}  \Gamma'  \models  \varphi\), then
    \(\sigma  \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma'  \models  \varphi\).
  \item[t-drop] If \( \ottmv{x}  \notin   \text{fvars}( \ottnt{t} )  \), then \( \lBrack  \ottnt{t}  \rBrack_{ \sigma : \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma' }   \ottsym{=}   \lBrack  \ottnt{t}  \rBrack_{ \sigma : \Gamma  \ottsym{,}  \Gamma' } \).
  \item[f-drop] If \( \ottmv{x}  \notin   \text{fvars}( \varphi )  \) and \(\sigma  \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma'  \models  \varphi\), then
    \(\sigma  \ottsym{:}  \Gamma  \ottsym{,}  \Gamma'  \models  \varphi\).
  \end{statements}

  \proof The proof is straightforward by structural induction on \(\ottnt{t}\) or \(\varphi\).
\end{prop}


\begin{prop}[name=Misc.\ theorems]{fol/thm/misc}
  Every following statement holds.
  \begin{statements}
  \item[drop] If \( \Gamma   \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  : \mathord{*} \), then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \ottsym{)}\).
  \item[dup] If \( \ottmv{x'}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x}  \ottsym{\}}  \) and
    \( \Gamma   \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  : \mathord{*} \), then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x'} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \ottsym{(}  \varphi  \wedge  \ottmv{x'}  \ottsym{=}  \ottmv{x}  \ottsym{)}  \wedge  \ottmv{x'}  \ottsym{=}  \ottnt{V}  \ottsym{)}  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{)}\).
  \item[swap] If
    \( \Gamma   \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x'} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x'}  \ottsym{=}  \ottnt{V'}  \ottsym{)}  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  : \mathord{*} \), then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x'} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x'}  \ottsym{=}  \ottnt{V'}  \ottsym{)}  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{)}  \wedge  \ottmv{x'}  \ottsym{=}  \ottnt{V'}  \ottsym{)}\).
  \item[push] If \( \ottmv{x}  \notin   \text{dom}( \Gamma )  \), \( \ottnt{V}  :  \ottnt{T} \), and \( \Gamma   \vdash   \varphi  : \mathord{*} \),
    then \(\Gamma  \models  \varphi  \implies  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \ottsym{(}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{)}  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{)}\).
  \item[not-t] If \( \ottmv{x'}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x}  \ottsym{\}}  \), \(\ottnt{i}  \neq  0\), and
    \( \Gamma   \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{i}  : \mathord{*} \), then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{i}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x'} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottsym{(}  \ottmv{x}  \neq  0  \wedge  \ottmv{x'}  \ottsym{=}  0  \vee  \ottmv{x}  \ottsym{=}  0  \wedge  \ottmv{x'}  \ottsym{=}  1  \ottsym{)}  \ottsym{)}  \wedge  \ottmv{x'}  \ottsym{=}  0  \ottsym{)}\).
  \item[not-f] If \( \ottmv{x'}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x}  \ottsym{\}}  \) and
    \( \Gamma   \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  0  : \mathord{*} \), then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  0  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x'} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottsym{(}  \ottmv{x}  \neq  0  \wedge  \ottmv{x'}  \ottsym{=}  0  \vee  \ottmv{x}  \ottsym{=}  0  \wedge  \ottmv{x'}  \ottsym{=}  1  \ottsym{)}  \ottsym{)}  \wedge  \ottmv{x'}  \ottsym{=}  1  \ottsym{)}\).
  \item[add] If \( \ottmv{x_{{\mathrm{3}}}}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{\}}  \), \( \ottnt{i_{{\mathrm{1}}}}  \ottsym{+}  \ottnt{i_{{\mathrm{2}}}} \ottsym{=} \ottnt{i_{{\mathrm{3}}}} \), and
    \( \Gamma   \vdash   \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{i_{{\mathrm{1}}}}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{i_{{\mathrm{2}}}}  : \mathord{*} \),
    then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{i_{{\mathrm{1}}}}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{i_{{\mathrm{2}}}}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{+}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{3}}}}  \ottsym{=}  \ottnt{i_{{\mathrm{3}}}}  \ottsym{)}\).
  \item[pair] If \( \ottmv{x_{{\mathrm{3}}}}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{\}}  \) and
    \( \Gamma   \vdash   \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  : \mathord{*} \), then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{3}}}}  \ottsym{=}  \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{)}\).
  \item[car] If \(\ottmv{x_{{\mathrm{1}}}}  \neq  \ottmv{x_{{\mathrm{2}}}}\), \( \ottmv{x_{{\mathrm{1}}}}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x}  \ottsym{\}}  \), \( \ottmv{x_{{\mathrm{2}}}}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x}  \ottsym{\}}  \),
    and \( \Gamma   \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  : \mathord{*} \), then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{)}\).
  \item[cdr] If \(\ottmv{x_{{\mathrm{1}}}}  \neq  \ottmv{x_{{\mathrm{2}}}}\), \( \ottmv{x_{{\mathrm{1}}}}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x}  \ottsym{\}}  \), \( \ottmv{x_{{\mathrm{2}}}}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x}  \ottsym{\}}  \),
    and \( \Gamma   \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  : \mathord{*} \), then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}\).
  \item[cons] If \( \ottmv{x_{{\mathrm{3}}}}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{\}}  \) and
    \( \Gamma   \vdash   \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  : \mathord{*} \),
    then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{3}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}\).
  \item[if-t] If \(\ottnt{i}  \neq  0\) and \( \Gamma   \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{i}  : \mathord{*} \),
    then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{i}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \neq  0  \ottsym{)}\).
  \item[if-cons] If \(\ottmv{x_{{\mathrm{1}}}}  \neq  \ottmv{x_{{\mathrm{2}}}}\), \( \ottmv{x_{{\mathrm{1}}}}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x}  \ottsym{\}}  \),
    \( \ottmv{x_{{\mathrm{2}}}}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x}  \ottsym{\}}  \), and
    \( \Gamma   \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  : \mathord{*} \), then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}\).
  \item[iter] If \( \ottmv{x_{{\mathrm{2}}}}  \notin   \text{fvars}( \varphi )  \) and
    \( \Gamma   \vdash   \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  : \mathord{*} \), then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}\).
  \item[strengthen] If \( \Gamma   \vdash   \varphi  : \mathord{*} \) and \(\Gamma  \models  \varphi'\), then
    \(\Gamma  \models  \varphi  \implies  \ottsym{(}  \varphi  \wedge  \varphi'  \ottsym{)}\).
  \item[lambda] If \( \ottmv{x}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{y_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{y_{{\mathrm{2}}}}  \ottsym{\}}  \) and
    \( \Gamma   \vdash   \varphi  \wedge  \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} (  \langle  \mathit{IS}  \rangle  ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}  : \mathord{*} \), then
    \(\Gamma  \models  \ottsym{(}  \varphi  \wedge  \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} (  \langle  \mathit{IS}  \rangle  ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottsym{(}  \varphi  \wedge  \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} ( \ottmv{x} ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}  \ottsym{)}  \wedge  \ottmv{x}  \ottsym{=}   \langle  \mathit{IS}  \rangle   \ottsym{)}\).
  \item[exec] If \( \ottmv{x_{{\mathrm{3}}}}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{\}}  \), \( \ottnt{V_{{\mathrm{2}}}}  :  \ottnt{T_{{\mathrm{2}}}} \), and
    \( \Gamma   \vdash   \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}   \langle  \mathit{IS}  \rangle   \ottsym{)}  \wedge   \ottkw{call} (  \langle  \mathit{IS}  \rangle  ,  \ottnt{V_{{\mathrm{1}}}} ) =  \ottnt{V_{{\mathrm{2}}}}   : \mathord{*} \), then
    \(\Gamma  \models  \ottsym{(}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}   \langle  \mathit{IS}  \rangle   \ottsym{)}  \wedge   \ottkw{call} (  \langle  \mathit{IS}  \rangle  ,  \ottnt{V_{{\mathrm{1}}}} ) =  \ottnt{V_{{\mathrm{2}}}}   \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge   \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottmv{x_{{\mathrm{3}}}}   \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{3}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}\).
  \item[transfer] If \( \ottmv{x_{{\mathrm{4}}}}  \notin    \text{dom}( \Gamma )   \cup  \ottsym{\{}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{3}}}}  \ottsym{\}}  \) and
    \( \Gamma   \vdash   \exists \,  \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{address}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{V}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{i}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{3}}}}  \ottsym{=}  \ottnt{a}  : \mathord{*} \), then
    \(\Gamma  \models  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{address}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{=}  \ottnt{V}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottnt{i}  \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{3}}}}  \ottsym{=}  \ottnt{a}  \ottsym{)}  \implies  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{4}}}} \mathord:\allowbreak \ottkw{operation}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{address}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{4}}}}  \ottsym{=}   \texttt{Transfer}  (  \ottmv{x_{{\mathrm{1}}}} ,  \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{3}}}}  )   \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{4}}}}  \ottsym{=}   \texttt{Transfer}  (  \ottnt{V} ,  \ottnt{i} ,  \ottnt{a}  )   \ottsym{)}\).
  \end{statements}

  \proof Straightforward.

  % So, those
  % can be proved by a standard manner.
\end{prop}

\begin{prop}[name=Lambda encoding]{fol/thm/lambda}
  If
  \begin{gather}
    \ottmv{y_{{\mathrm{1}}}}  \neq  \ottmv{y_{{\mathrm{2}}}} \hyp{neq}\\
      \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*}  \hyp{wf1}\\
      \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*}  \hyp{wf2}\\
      \langle  \mathit{IS}  \rangle   :  \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}  \hyp{typ}\\
    \left(
      \begin{split}
        \text{For any } & \ottnt{V_{{\mathrm{1}}}}, \ottnt{V_{{\mathrm{2}}}}, \sigma, \\
        \text{ if } & \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Downarrow  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ddagger \text{ and } \\
         &\sigma  \ottsym{:}   \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \models  \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ddagger  \ottsym{:}  \ottsym{\{}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright  \ddagger  \mid  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \ottsym{\}} \\
        \text{ then } & \sigma  \ottsym{:}   \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \models  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ddagger  \ottsym{:}  \ottsym{\{}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \ddagger  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}
      \end{split}
    \right) \hyp{OIH}
  \end{gather}
  then
  \(\Gamma  \models  \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} (  \langle  \mathit{IS}  \rangle  ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}\) for any \(\Gamma\).

  \proof By the definition of the semantics of $\mathtt{call}$.
\end{prop}

\begin{prop}[name=Exec encoding]{fol/thm/exec}
  If
  \begin{gather}
    \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Downarrow  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ddagger \hyp{eval}\\
     \ottnt{V_{{\mathrm{1}}}}  :  \ottnt{T_{{\mathrm{1}}}}  \hyp{typ1}\\
     \ottnt{V_{{\mathrm{2}}}}  :  \ottnt{T_{{\mathrm{2}}}}  \hyp{typ2}\\
      \langle  \mathit{IS}  \rangle   :  \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}  \hyp{3}
  \end{gather}
  then
  \(\Gamma  \models   \ottkw{call} (  \langle  \mathit{IS}  \rangle  ,  \ottnt{V_{{\mathrm{1}}}} ) =  \ottnt{V_{{\mathrm{2}}}} \) for any \(\Gamma\).

  \proof By the definition of the semantics of $\mathtt{call}$.
\end{prop}

\endinput

\AI{I think we can be more hand-waving about some of these lemmas, in particular, those about valid formulae.}

\begin{prop}{ftyping/inv}
  Every following statement holds.
  \begin{statements}
  \item[and] If \( \Gamma   \vdash   \varphi_{{\mathrm{1}}}  \wedge  \varphi_{{\mathrm{2}}}  : \mathord{*} \), then \( \Gamma   \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) and \( \Gamma   \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \).
  \item[imply] If \( \Gamma   \vdash   \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}}  : \mathord{*} \), then \( \Gamma   \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) and \( \Gamma   \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \).
  \item[exists] If \( \Gamma   \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  : \mathord{*} \), then \( \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}    \vdash   \varphi  : \mathord{*} \).
  \end{statements}

  \proof Easy.
\end{prop}

\begin{prop}[name=Structural properties for well-sortedness judgment]{ttyping/strut}
  Every following statement holds.
  \begin{statements}
  \item[tclosed] If \(\Gamma  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T}\), then \(  \text{fvars}( \ottnt{t} )   \subseteq   \text{dom}( \Gamma )  \).
  \item[fclosed] If \( \Gamma   \vdash   \varphi  : \mathord{*} \), then \(  \text{fvars}( \varphi )   \subseteq   \text{dom}( \Gamma )  \).
  \item[tperm] If \(\Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}  \Gamma_{{\mathrm{2}}}  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T}\), then
    \(\Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}  \Gamma_{{\mathrm{2}}}  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T}\).
  \item[fperm] If \( \Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}  \Gamma_{{\mathrm{2}}}   \vdash   \varphi  : \mathord{*} \), then
    \( \Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}  \Gamma_{{\mathrm{2}}}   \vdash   \varphi  : \mathord{*} \).
  \item[tweaken] If \(\Gamma_{{\mathrm{1}}}  \ottsym{,}  \Gamma_{{\mathrm{2}}}  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T}\), then \(\Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}  \Gamma_{{\mathrm{2}}}  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T}\).
  \item[fweaken] If \( \Gamma_{{\mathrm{1}}}  \ottsym{,}  \Gamma_{{\mathrm{2}}}   \vdash   \varphi  : \mathord{*} \), then \( \Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma_{{\mathrm{2}}}   \vdash   \varphi  : \mathord{*} \).
  \item[tsubst] If \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\) and \(\Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma_{{\mathrm{2}}}  \vdash  \ottnt{t}  \ottsym{:}  \ottnt{T'}\), then
    \(\texttt{\textcolor{red}{<<no parses (char 12): G1, G2 \mbox{$\mid$}- t.***\{V/x\} : T' >>}}\).
  \item[fsubst] If \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\) and \( \Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma_{{\mathrm{2}}}   \vdash   \varphi  : \mathord{*} \), then
    \(\texttt{\textcolor{red}{<<no parses (char 12): G1, G2 \mbox{$\mid$}- p.***\{V/x\} : * >>}}\).
  \end{statements}

  \proof By straightforward induction on the given well-sortedness
  derivation.  Some proofs depend on former results.
\end{prop}

\begin{prop}{fol/term/subst}
  \(\texttt{\textcolor{red}{<<no parses (char 5): val(t***.\{V/x\}, s) = val(t, s.[V/x]) >>}}\).

  \proof By straightforward induction on \(\ottnt{t}\).
\end{prop}

\begin{prop}{fol/formula/subst}
  \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** p.\{V/x\} >>}}\) iff \(\texttt{\textcolor{red}{<<no parses (char 9): s.[V/x] \mbox{$\mid$}***= p >>}}\).

  \proof By straightforward induction on \(\varphi\) by
  using \propref{fol/term/subst}.
\end{prop}

\begin{prop}{fol/subst}
  If \(\Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma_{{\mathrm{2}}}  \models  \varphi\) and \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\), then \(\texttt{\textcolor{red}{<<no parses (char 14): G1, G2 \mbox{$\mid$}=
  p.***\{V/x\} >>}}\).

  \proof We know \( \Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma_{{\mathrm{2}}}   \vdash   \varphi  : \mathord{*} \) and \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** p >>}}\) for any
  \(\sigma\) such that \(\texttt{\textcolor{red}{<<no parses (char 10): \mbox{$\mid$}= s(x) : ***T >>}}\) for every \(  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \in  \Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma_{{\mathrm{2}}} \) by
  definition.  To show the goal, we show the following two subgoals.
  \begin{goal}
  \item[{\(\texttt{\textcolor{red}{<<no parses (char 12): G1, G2 \mbox{$\mid$}- p.***\{V/x\} : * >>}}\)}] The goal follows by
    \propref{ttyping/strut(fsubst)}.
  \item[{\(\texttt{\textcolor{red}{<<no parses (char 5): s' \mbox{$\mid$}=*** p.\{V/x\} >>}}\) for any \(\sigma'\) such that
      \(\texttt{\textcolor{red}{<<no parses (char 12): \mbox{$\mid$}= s'(x') : ***T >>}}\) for every \(  \ottmv{x'} \mathord:\allowbreak \ottnt{T}   \in  \Gamma_{{\mathrm{1}}}  \ottsym{,}  \Gamma_{{\mathrm{2}}} \)}] We can observe
    that \( \sigma'  [  \ottmv{x}  \mapsto  \ottnt{V}  ] \) satisfies \(\texttt{\textcolor{red}{<<no parses (char 18): \mbox{$\mid$}= s'.[V/x](x') : ***T >>}}\) for every
    \(  \ottmv{x'} \mathord:\allowbreak \ottnt{T}   \in  \Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma_{{\mathrm{2}}} \).  So, \(\texttt{\textcolor{red}{<<no parses (char 10): s'.[V/x] \mbox{$\mid$}***= p >>}}\) follows by the
    assumption.  Then, the subgoal follows by \propref{fol/formula/subst}.
  \end{goal}
\end{prop}

\begin{prop}{fol/weaken}
  If \(\Gamma  \models  \varphi\), then \(\Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \varphi\).
\end{prop}

\begin{prop}{fol/andI}
  If \(\Gamma  \models  \varphi_{{\mathrm{1}}}\) and \(\Gamma  \models  \varphi_{{\mathrm{2}}}\), then \(\Gamma  \models  \varphi_{{\mathrm{1}}}  \wedge  \varphi_{{\mathrm{2}}}\).
\end{prop}

\begin{prop}{fol/forallI}
  If \(\Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \varphi\), then \(\Gamma  \models  \forall \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi\).
\end{prop}

\begin{prop}{fol/imply/refl}
  If \( \Gamma   \vdash   \varphi  : \mathord{*} \), then \(\Gamma  \models  \varphi  \implies  \varphi\).
\end{prop}

\begin{prop}{fol/imply/trans}
  If
  \begin{gather}
    \Gamma  \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}} \hyp{1}\\
    \Gamma  \models  \varphi_{{\mathrm{2}}}  \implies  \varphi_{{\mathrm{3}}} \hyp{2}
  \end{gather}
  then \(\Gamma  \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{3}}}\).

  \proof To show the goal, we show the following two subgoals.
  \begin{goal}
  \item[\( \Gamma   \vdash   \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{3}}}  : \mathord{*} \)] We have \( \Gamma   \vdash   \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}}  : \mathord{*} \) and
    \( \Gamma   \vdash   \varphi_{{\mathrm{2}}}  \implies  \varphi_{{\mathrm{3}}}  : \mathord{*} \) by \propref{def/sem/pred} with \hypref{1} and
    \hypref{2}, respectively.  So, \( \Gamma   \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) and \( \Gamma   \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \)
    follows by \propref{ftyping/inv(imply)}.  From these, the subgoal follows
    by \ruleref{WF-Imply}.

  \item[\(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** p1 ==> p3 >>}}\) for any \(\sigma\) such that \(\texttt{\textcolor{red}{<<no parses (char 10): \mbox{$\mid$}= s(x) : ***T >>}}\)
    for every \(  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \in  \Gamma \)] We have
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** p1 ==> p2 >>}} \hyp{3}\\
      \texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** p2 ==> p3 >>}} \hyp{4}
    \end{gather}
    by \hypref{1} and \hypref{2}, respectively, with \propref{def/sem/pred}.
    To show the subgoal, it is enough to consider the following two cases.
    \begin{match}
    \item[\(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}/***= p1 >>}}\)] The subgoal follows by the definition.
    \item[\(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** p1 >>}}\)] We know \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** p2 >>}}\) by \hypref{3}, and then also
      we know \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** p3 >>}}\) by \hypref{4}.  Now, the subgoal follows by the
      definition.
    \end{match}
  \end{goal}
\end{prop}

\begin{prop}{fol/mp}
  If \(\Gamma  \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}}\) and \(\Gamma  \models  \varphi_{{\mathrm{1}}}\), then \(\Gamma  \models  \varphi_{{\mathrm{2}}}\).
\end{prop}

\begin{prop}{fol/thm/exists=>subst}
  \(\texttt{\textcolor{red}{<<no parses (char 34): \mbox{$\mid$}= (exists x:T. p /\mbox{$\backslash{}$} x = V) ==> p.***\{V/x\} >>}}\).

  \proof To show the goal, we assume \(\sigma\) such that
  \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** exists x:T. p /\mbox{$\backslash{}$} x = V >>}}\), and then show \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** p.\{V/x\} >>}}\).  By
  the assumption, we know, for some \(\ottnt{V'}\),
  \begin{gather}
    \texttt{\textcolor{red}{<<no parses (char 10): s.[V'/x] \mbox{$\mid$}***= p >>}} \hyp{1}\\
    \texttt{\textcolor{red}{<<no parses (char 10): s.[V'/x] \mbox{$\mid$}***= x = V >>}}. \hyp{2}
  \end{gather}
  From \hypref{2} we have \(\ottnt{V'}  \ottsym{=}  \ottnt{V}\).  Now \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** p.\{V/x\} >>}}\) follows by
  applying \propref{fol/formula/subst} to \hypref{1}.
\end{prop}

\begin{prop}{fol/thm/subst=>exists}
  If \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\), then \(\texttt{\textcolor{red}{<<no parses (char 5): \mbox{$\mid$}= p.***\{V/x\} ==> exists x:T. p /\mbox{$\backslash{}$} x = V >>}}\).

  \proof To show the goal, we assume \(\sigma\) such that \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** p.\{V/x\} >>}}\),
  and then show \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** exists x:T. p /\mbox{$\backslash{}$} x = V >>}}\).  We have \(\texttt{\textcolor{red}{<<no parses (char 9): s.[V/x] \mbox{$\mid$}***=
  p >>}}\) by \propref{fol/formula/subst}, and \(\texttt{\textcolor{red}{<<no parses (char 9): s.[V/x] \mbox{$\mid$}***= x = V >>}}\) by
  definition.  So, \(\texttt{\textcolor{red}{<<no parses (char 9): s.[V/x] \mbox{$\mid$}***= p /\mbox{$\backslash{}$} x = V >>}}\); and with the assumption \(\texttt{\textcolor{red}{<<no parses (char 9): \mbox{$\mid$}=
  V : ***T >>}}\), \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** exists x:T. p /\mbox{$\backslash{}$} x = V >>}}\) follows by definition.
\end{prop}

\begin{prop}{fol/thm/valid}
  If \( \Gamma   \vdash   \varphi  : \mathord{*} \) and \(\texttt{\textcolor{red}{<<no parses (char 4): \mbox{$\mid$}= p*** >>}}\), then \(\Gamma  \models  \varphi\).

  \proof Straightforward by \propref{def/sem/pred}.
  \AI{Is \(\texttt{\textcolor{red}{<<no parses (char 4): \mbox{$\mid$}= p*** >>}}\) defined anywhere?}
\end{prop}

\begin{prop}[name=Misc.\ theorems]{fol/thm/misc}
  Every following statement holds.
  \begin{statements}
  \item[drop1] \(\texttt{\textcolor{red}{<<no parses (char 47): \mbox{$\mid$}= (exists x:T. p /\mbox{$\backslash{}$} x1 = V1) ==> exists x:T. p*** >>}}\).
  \item[drop3]
    \(\texttt{\textcolor{red}{<<no parses (char 123): \mbox{$\mid$}= (exists x1:T1. (exists x2:T2. (exists x3:T3. p /\mbox{$\backslash{}$} x3 = V3) /\mbox{$\backslash{}$} x2 =
    V2) /\mbox{$\backslash{}$} x1 = V1) ==> exists x3:T3, x2:T2, x1:T1. p*** >>}}\).
  \item[dup]
    \(\texttt{\textcolor{red}{<<no parses (char 90): \mbox{$\mid$}= (exists x:T. p /\mbox{$\backslash{}$} x = V) ==> exists x:T. (exists y:T. p /\mbox{$\backslash{}$} y = x /\mbox{$\backslash{}$} y
    = V) /\mbox{$\backslash{}$} x = V*** >>}}\).
  \item[swap]
    \(\texttt{\textcolor{red}{<<no parses (char 112): \mbox{$\mid$}= (exists y:T2. (exists x:T1. p /\mbox{$\backslash{}$} x = V1) /\mbox{$\backslash{}$} y = V2) ==> exists
    x:T1. (exists y:T2. p /\mbox{$\backslash{}$} y = V2) /\mbox{$\backslash{}$} x = V1*** >>}}\).
  \item[push] If \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\), then
    \(\texttt{\textcolor{red}{<<no parses (char 42): \mbox{$\mid$}= p ==> exists x:T. (p /\mbox{$\backslash{}$} x = V) /\mbox{$\backslash{}$} x = V*** >>}}\).
  \item[tf] If \(\ottnt{i}  \neq  0\), then
    \(\texttt{\textcolor{red}{<<no parses (char 117): \mbox{$\mid$}= (exists x:int. p /\mbox{$\backslash{}$} x = i) ==> exists y:int. (exists x:int. p /\mbox{$\backslash{}$} (x
    <> 0 /\mbox{$\backslash{}$} y = 0 \mbox{$\backslash{}$}/ x = 0 /\mbox{$\backslash{}$} y = 1)) /\mbox{$\backslash{}$} y = 0*** >>}}\).
  \item[ft]
    \(\texttt{\textcolor{red}{<<no parses (char 117): \mbox{$\mid$}= (exists x:int. p /\mbox{$\backslash{}$} x = 0) ==> exists y:int. (exists x:int. p /\mbox{$\backslash{}$} (x
    <> 0 /\mbox{$\backslash{}$} y = 0 \mbox{$\backslash{}$}/ x = 0 /\mbox{$\backslash{}$} y = 1)) /\mbox{$\backslash{}$} y = 1*** >>}}\).
  \item[add] If \( \ottnt{i_{{\mathrm{1}}}}  \ottsym{+}  \ottnt{i_{{\mathrm{2}}}} \ottsym{=} \ottnt{i_{{\mathrm{3}}}} \), then
    \(\texttt{\textcolor{red}{<<no parses (char 126): \mbox{$\mid$}= (exists y:int. (exists x:int. p /\mbox{$\backslash{}$} x = i1) /\mbox{$\backslash{}$} y = i2) ==> exists
    z:int. (exists x:int, y:int. p /\mbox{$\backslash{}$} x + y = z) /\mbox{$\backslash{}$} z = i3*** >>}}\).
  \item[pair]
    \(\texttt{\textcolor{red}{<<no parses (char 131): \mbox{$\mid$}= (exists y:T2. (exists x:T1. p /\mbox{$\backslash{}$} x = V1) /\mbox{$\backslash{}$} y = V2) ==> exists
    z:T1*T2. (exists x:T1, y:T2. p /\mbox{$\backslash{}$} (x, y) = z) /\mbox{$\backslash{}$} z = (V1, V2)*** >>}}\).
  \item[car]
    \(\texttt{\textcolor{red}{<<no parses (char 114): \mbox{$\mid$}= (exists x:T1*T2. p /\mbox{$\backslash{}$} x = (V1, V2)) ==> exists x1:T1. (exists
    x:T1*T2, x2:T2. p /\mbox{$\backslash{}$} x = (x1, x2)) /\mbox{$\backslash{}$} x1 = V1*** >>}}\).
  \item[cdr]
    \(\texttt{\textcolor{red}{<<no parses (char 114): \mbox{$\mid$}= (exists x:T1*T2. p /\mbox{$\backslash{}$} x = (V1, V2)) ==> exists x2:T2. (exists
    x:T1*T2, x1:T1. p /\mbox{$\backslash{}$} x = (x1, x2)) /\mbox{$\backslash{}$} x2 = V2*** >>}}\).
  \item[cons]
    \(\texttt{\textcolor{red}{<<no parses (char 153): \mbox{$\mid$}= (exists x2:T list. (exists x1:T. p /\mbox{$\backslash{}$} x1 = V1) /\mbox{$\backslash{}$} x2 = V2) ==> exists
    x3:T list. (exists x1:T, x2:T list. p /\mbox{$\backslash{}$} x1 :: x2 = x3) /\mbox{$\backslash{}$} x3 = V1 ::
    V2*** >>}}\).
  \item[ift] If \(\ottnt{i}  \neq  0\), then
    \(\texttt{\textcolor{red}{<<no parses (char 59): \mbox{$\mid$}= (exists x:int. p /\mbox{$\backslash{}$} x = i) ==> exists x:int. p /\mbox{$\backslash{}$} x <> 0*** >>}}\).
  \item[ifconst]
    \(\texttt{\textcolor{red}{<<no parses (char 133): \mbox{$\mid$}= (exists x:T list. p /\mbox{$\backslash{}$} x = V1 :: V2) ==> exists z:T list. (exists
    y:T. (exists x:T list. p /\mbox{$\backslash{}$} y :: z = x) /\mbox{$\backslash{}$} y = V1) /\mbox{$\backslash{}$} z = V2*** >>}}\).
  \item[iter]
    \(\texttt{\textcolor{red}{<<no parses (char 105): \mbox{$\mid$}= (exists x:T list. p /\mbox{$\backslash{}$} V1 :: V2 = x) ==> exists y:T. (exists x:T
    list. p /\mbox{$\backslash{}$} y :: V2 = x) /\mbox{$\backslash{}$} y = V1*** >>}}\).
  \item[transfer]
    \(\texttt{\textcolor{red}{<<no parses (char 130): \mbox{$\mid$}= (exists x3:address. (exists x2:int. (exists x1:T. p /\mbox{$\backslash{}$} x1 = V) /\mbox{$\backslash{}$} x2
    = i) /\mbox{$\backslash{}$} x3 = a) ==> exists x1:T, x2:int, x3:address. p*** >>}}\).
  \item[exsitsandforall]
    \(\texttt{\textcolor{red}{<<no parses (char 86): \mbox{$\mid$}= ((exists x:T. p1 /\mbox{$\backslash{}$} x = V) /\mbox{$\backslash{}$} forall x:T. p2) ==> exists x:T. p1 /\mbox{$\backslash{}$}
    p2 /\mbox{$\backslash{}$} x = V*** >>}}\).
  \item[existsswap]
    \(\texttt{\textcolor{red}{<<no parses (char 75): \mbox{$\mid$}= (exists x1:T1. exists x2:T2. p) <==> (exists x2:T2. exists
    x1:T2. p)*** >>}}\)
  \end{statements}

  \proof Straightforward.
  
  \AI{``The statements are standard properties in first-order logic.'' Well, standard first-order logic doesn't make any commitment on specific datatypes.}
  % So, those
  % can be proved by a standard manner.
\end{prop}

\begin{prop}{fol/thm/lambda}
  If $\mathit{IS}$ satisfies
  \begin{multline}
    \text{for any } \ottnt{V_{{\mathrm{1}}}}, \ottnt{V_{{\mathrm{2}}}} \text{ if }
    \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Downarrow  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ddagger \text{ and }
    \texttt{\textcolor{red}{<<no parses (char 15): y1':T1 \mbox{$\mid$}= V1 :.*** \_ : \{y1:T1 :. \_ \mbox{$\mid$} y1' = y1 /\mbox{$\backslash{}$} p1\} >>}},\\ \text{ then }
    \texttt{\textcolor{red}{<<no parses (char 15): y1':T1 \mbox{$\mid$}= V2 :.*** \_ : \{y2:T2 :. \_ \mbox{$\mid$} p2\} >>}}, \hyp{OIH}
  \end{multline}
  then
  \(\texttt{\textcolor{red}{<<no parses (char 79): \mbox{$\mid$}= forall y1':T1, y1:T1, y2:T2. y1' = y1 /\mbox{$\backslash{}$} p1 /\mbox{$\backslash{}$} call(<IS>, y1') = y2 ==>
  p2*** >>}}\).

  \proof \AI{By definition of the semantics of call?}
\end{prop}

\begin{prop}{fol/thm/exec}
  If
  \begin{gather}
    \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Downarrow  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ddagger \hyp{eval}
  \end{gather}
  then
  \(\texttt{\textcolor{red}{<<no parses (char 22): \mbox{$\mid$}= call(<IS>, V1) = V2*** >>}}\).

  \proof \AI{By definition of the semantics of call?}
\end{prop}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper.otex"
%%% End:


==> proofs/semty.tex <==
\subsection{Properties for semantics of refinement stack typse}

\begin{prop}{semty/conservative}
  If \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \Phi\), then \( \ottnt{S}  :   \lfloor  \Phi  \rfloor  \).

  \proof The proof is done by induction on the given derivation.
  \begin{match}
  \item[\ruleref{Sem-Bottom}] We have
    \begin{gather}
       \ottnt{S} \ottsym{=} \ddagger  \hyp{1}\\
       \Phi \ottsym{=} \ottsym{\{}  \ddagger  \mid  \varphi  \ottsym{\}}  \hyp{2}
    \end{gather}
    for some \(\varphi\).  The goal \( \ddagger  :  \ddagger \) is derived by
    \ruleref{ST-Bottom}.

  \item[\ruleref{Sem-Push}] We have
    \begin{gather}
       \ottnt{S} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S'}  \hyp{1}\\
       \Phi \ottsym{=} \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}}  \hyp{2}\\
       \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{3}
    \end{gather}
    for some \(\ottnt{V}\), \(\ottnt{S'}\), \(\ottmv{x}\), \(\ottnt{T}\), \(\Upsilon\), and
    \(\varphi\).  By IH of \hypref{3}, we have
    \begin{gather}
       \ottnt{S'}  :   \lfloor  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}}  \rfloor   \hyp{4}.
    \end{gather}
    We know \( \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \) by \hypref{3}.  So, by definition, we have
    \begin{gather}
       \ottnt{V}  :  \ottnt{T}  \hyp{5}.
    \end{gather}
    Now we can derive the goal \( \ottnt{V}  \triangleright  \ottnt{S'}  :  \ottnt{T}  \triangleright   \lfloor  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}}  \rfloor  \) by
    \ruleref{ST-Push}, \hypref{4}, and \hypref{5}.  \qedhere
  \end{match}
\end{prop}

\begin{prop}{semty/wf}
  If \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}}\), then \(\sigma  \ottsym{:}  \Gamma\) and \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \varphi  : \mathord{*} \).

  \proof The proof is straightforward by induction on the given derivation.
\end{prop}

\begin{prop}{semty/inv}
  Every following statement holds.
  \begin{statements}
  \item[bottom] If \(\sigma  \ottsym{:}  \Gamma  \models  \ddagger  \ottsym{:}  \Phi\), then \( \Phi \ottsym{=} \ottsym{\{}  \ddagger  \mid  \varphi  \ottsym{\}} \) and
    \(\sigma  \ottsym{:}  \Gamma  \models  \varphi\) for some \(\varphi\).
  \item[push] If \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{V}  \triangleright  \ottnt{S}  \ottsym{:}  \Phi\), then \( \Phi \ottsym{=} \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \)
    and \( \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}}\) for some \(\ottmv{x}\), \(\ottnt{T}\),
    \(\Upsilon\), and \(\varphi\).
  \end{statements}

  \proof Easy by definition.
\end{prop}

\begin{prop}{semty/env/perm}
  If \(\sigma  \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}  \Gamma'  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}}\), then
  \(\sigma  \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma'  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}}\).

  \proof The proof is straightforward by induction on the given derivation.  In
  the base case we use \propref{fol/strut(f-perm)}.
\end{prop}

\begin{prop}{semty/logic}
  The following statements are equivalent:
  \begin{statements}
  \item[exists=>subst] \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}\);
  \item[subst=>exists] \( \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}}\); and
  \item[push] \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{V}  \triangleright  \ottnt{S}  \ottsym{:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}}\).
  \end{statements}

  \proof\noindent
  \begin{itemize}
  \item \((1) \Rightarrow (2)\).  The proof is done by induction on the given
    derivation.
    \begin{match}
    \item[\ruleref{Sem-Bottom}] We have
      \begin{gather}
         \ottnt{S} \ottsym{=} \ddagger  \hyp{1}\\
         \Upsilon \ottsym{=} \ddagger  \hyp{2}\\
        \sigma  \ottsym{:}  \Gamma  \models  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V} \hyp{3}.
      \end{gather}
      By definition of \hypref{3}, we have
      \begin{gather}
         \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \varphi \hyp{4}.
      \end{gather}
      So the goal \( \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ddagger  \ottsym{:}  \ottsym{\{}  \ddagger  \mid  \varphi  \ottsym{\}}\) can be derived by
      \ruleref{Sem-Bottom} and \hypref{4}.

    \item[\ruleref{Sem-Push}] We have
      \begin{gather}
         \ottnt{S} \ottsym{=} \ottnt{V'}  \triangleright  \ottnt{S'}  \hyp{1}\\
         \Upsilon \ottsym{=}  \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \triangleright  \Upsilon'  \hyp{2}\\
         \sigma  [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}} \hyp{4}
      \end{gather}
      for some \(\ottnt{V'}\), \(\ottnt{S'}\), \(\ottmv{x'}\), \(\ottnt{T'}\), and \(\Upsilon'\).
      By IH of \hypref{4}, we have
      \begin{gather}
          \sigma  [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \varphi  \ottsym{\}} \hyp{4.1}.
      \end{gather}
      We know \(\ottmv{x}  \neq  \ottmv{x'}\) by the constraint on typing environments.  So, we
      have
      \begin{gather}
           \sigma  [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   [  \ottmv{x}  \mapsto  \ottnt{V}  ]  \ottsym{=}   \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   \hyp{4.3}.
      \end{gather}
      By \propref{semty/env/perm}, \hypref{4.1}, and \hypref{4.3}, we have
      \begin{gather}
          \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \varphi  \ottsym{\}} \hyp{6}.
      \end{gather}
      So the goal \( \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{V'}  \triangleright  \ottnt{S'}  \ottsym{:}  \ottsym{\{}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \triangleright  \Upsilon'  \mid  \varphi  \ottsym{\}}\) can be
      derived by \ruleref{Sem-Push} and \hypref{6}. \qedhere
    \end{match}

  \item \((2) \Rightarrow (1)\).  The proof is done by structural induction on
    \(\ottnt{S}\).
    \begin{match}
    \item[\( \ottnt{S} \ottsym{=} \ddagger \)] By \propref{semty/inv(bottom)} and the premise, we have
      \begin{gather}
         \Upsilon \ottsym{=} \ddagger  \hyp{2}\\
         \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \varphi \hyp{3}
      \end{gather}
      By \propref{def/sem/formula} and \hypref{3}, we have
      \begin{gather}
        \sigma  \ottsym{:}  \Gamma  \models  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V} \hyp{4}.
      \end{gather}
      So the goal \(\sigma  \ottsym{:}  \Gamma  \models  \ddagger  \ottsym{:}  \ottsym{\{}  \ddagger  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}\) can be derived
      by \ruleref{Sem-Bottom} and \hypref{4}.

    \item[\( \ottnt{S} \ottsym{=} \ottnt{V'}  \triangleright  \ottnt{S'} \) for some \(\ottnt{V'}\) and \(\ottnt{S'}\)] By
      \propref{semty/inv(push)} and the premise, we have
      \begin{gather}
         \Upsilon \ottsym{=}  \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \triangleright  \Upsilon'  \hyp{2}\\
          \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \varphi  \ottsym{\}} \hyp{4}
      \end{gather}
      for some \(\ottmv{x'}\), \(\ottnt{T'}\), and \(\Upsilon'\).  We know
      \( \ottmv{x'} \neq \ottmv{x} \) by the constraint on typing environments.  Then, we have
      \(   \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]  \ottsym{=}   \sigma  [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   [  \ottmv{x}  \mapsto  \ottnt{V}  ]  \), and so, by
      \propref{semty/env/perm} and \hypref{4},
      \begin{gather}
          \sigma  [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \varphi  \ottsym{\}} \hyp{5}.
      \end{gather}
      Now we have
      \begin{gather}
         \sigma  [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}} \hyp{6}
      \end{gather}
      by applying IH of \hypref{5}.  So the goal
      \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{V'}  \triangleright  \ottnt{S'}  \ottsym{:}  \ottsym{\{}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \triangleright  \Upsilon'  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}\) can be
      derived by \ruleref{Sem-Push} and \hypref{6}.  \qedhere
    \end{match}

  \item \((2) \Rightarrow (3)\).  This just follows from \ruleref{Sem-Push}.

  \item \((3) \Rightarrow (2)\).  Easy by \propref{semty/inv(push)}.  \qed
  \end{itemize}
\end{prop}

\begin{comment}

\begin{prop}{semty/logic/exists=>subst}
  If \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}\), then
  \( \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}}\).

  \proof The proof is done by induction on the given derivation.
  \begin{match}
  \item[\ruleref{Sem-Bottom}] We have the following hypothesis.
    \begin{gather}
       \ottnt{S} \ottsym{=} \ddagger  \hyp{1}\\
       \Upsilon \ottsym{=} \ddagger  \hyp{2}\\
      \sigma  \ottsym{:}  \Gamma  \models  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V} \hyp{3}
    \end{gather}
    By definition of \hypref{3}, we have
    \begin{gather}
       \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \varphi \hyp{4}.
    \end{gather}
    So the goal \( \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ddagger  \ottsym{:}  \ottsym{\{}  \ddagger  \mid  \varphi  \ottsym{\}}\) can be derived by
    \ruleref{Sem-Bottom} and \hypref{4}.

  \item[\ruleref{Sem-Push}] We have the following hypothesis for some
    \(\ottnt{V'}\), \(\ottnt{S'}\), \(\ottmv{x'}\), \(\ottnt{T'}\), and \(\Upsilon'\).
    \begin{gather}
       \ottnt{S} \ottsym{=} \ottnt{V'}  \triangleright  \ottnt{S'}  \hyp{1}\\
       \Upsilon \ottsym{=}  \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \triangleright  \Upsilon'  \hyp{2}\\
       \sigma  [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}} \hyp{4}
    \end{gather}
    By IH of \hypref{4}, we have
    \begin{gather}
        \sigma  [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \varphi  \ottsym{\}} \hyp{4.1}.
    \end{gather}
    We know \(\ottmv{x}  \neq  \ottmv{x'}\) by the constraint on typing environments.  So, we
    have
    \begin{gather}
         \sigma  [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   [  \ottmv{x}  \mapsto  \ottnt{V}  ]  \ottsym{=}   \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   \hyp{4.3}.
    \end{gather}
    By \propref{semty/env/perm}, \hypref{4.1}, and \hypref{4.3}, we have
    \begin{gather}
        \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \varphi  \ottsym{\}} \hyp{6}.
    \end{gather}
    So the goal \( \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{V'}  \triangleright  \ottnt{S'}  \ottsym{:}  \ottsym{\{}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \triangleright  \Upsilon'  \mid  \varphi  \ottsym{\}}\) can be
    derived by \ruleref{Sem-Push} and \hypref{6}. \qedhere
  \end{match}
\end{prop}

\begin{prop}{semty/logic/subst=>exists}
  If
  \begin{gather}
     \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{semty}
  \end{gather}
  then \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}\).

  \proof The proof is done by structural induction on \(\ottnt{S}\).
  \begin{match}
  \item[\( \ottnt{S} \ottsym{=} \ddagger \)] We have the following hypothesis by
    \propref{semty/inv(bottom)} and \hypref{semty}.
    \begin{gather}
       \Upsilon \ottsym{=} \ddagger  \hyp{2}\\
       \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \varphi \hyp{3}
    \end{gather}
    By \propref{def/sem/formula} and \hypref{3}, we have
    \begin{gather}
      \sigma  \ottsym{:}  \Gamma  \models  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V} \hyp{4}.
    \end{gather}
    So the goal \(\sigma  \ottsym{:}  \Gamma  \models  \ddagger  \ottsym{:}  \ottsym{\{}  \ddagger  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}\) can be derived
    by \ruleref{Sem-Bottom} and \hypref{4}.

  \item[\( \ottnt{S} \ottsym{=} \ottnt{V'}  \triangleright  \ottnt{S'} \) for some \(\ottnt{V'}\) and \(\ottnt{S'}\)] By
    \propref{semty/inv(push)} and \hypref{semty}, we have the following
    hypothesis for some \(\ottmv{x'}\), \(\ottnt{T'}\), and \(\Upsilon'\).
    \begin{gather}
       \Upsilon \ottsym{=}  \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \triangleright  \Upsilon'  \hyp{2}\\
        \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \varphi  \ottsym{\}} \hyp{4}
    \end{gather}
    We know \( \ottmv{x'} \neq \ottmv{x} \) by the constraint on typing environments.  Then, we have
    \(   \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]  \ottsym{=}   \sigma  [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   [  \ottmv{x}  \mapsto  \ottnt{V}  ]  \), and so, by
    \propref{semty/env/perm} and \hypref{4},
    \begin{gather}
        \sigma  [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \varphi  \ottsym{\}} \hyp{5}.
    \end{gather}
    Now we have
    \begin{gather}
       \sigma  [  \ottmv{x'}  \mapsto  \ottnt{V'}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}} \hyp{6}
    \end{gather}
    by applying IH of \hypref{5}.  So the goal
    \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{V'}  \triangleright  \ottnt{S'}  \ottsym{:}  \ottsym{\{}   \ottmv{x'} \mathord:\allowbreak \ottnt{T'}   \triangleright  \Upsilon'  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}\) can be
    derived by \ruleref{Sem-Push} and \hypref{6}.  \qedhere
  \end{match}
\end{prop}

\end{comment}

\begin{prop}{semty/logic/imply}
  If
  \begin{gather}
    \sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{semty}\\
    \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \models  \varphi  \implies  \varphi' \hyp{imply}
  \end{gather}
  then \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi'  \ottsym{\}}\).
  
  \proof The proof is done by induction on the given derivation of
  \hypref{semty}. 
  \begin{match}
  \item[\ruleref{Sem-Bottom}] We have
    \begin{gather}
       \ottnt{S} \ottsym{=} \ddagger  \hyp{1}\\
       \Upsilon \ottsym{=} \ddagger  \hyp{2}\\
      \sigma  \ottsym{:}  \Gamma  \models  \varphi \hyp{3}.
    \end{gather}
    By definition of \hypref{imply}, we have
    \begin{gather}
      \sigma  \ottsym{:}  \Gamma  \models  \varphi  \implies  \varphi' \hyp{6}.
    \end{gather}
    Now we have
    \begin{gather}
      \sigma  \ottsym{:}  \Gamma  \models  \varphi' \hyp{7}
    \end{gather}
    by \hypref{3} and \hypref{6}.
    Finally the goal can be derived by \ruleref{Sem-Bottom} and \hypref{7}.

  \item[\ruleref{Sem-Push}] We have
    \begin{gather}
       \ottnt{S} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S'}  \hyp{1}\\
       \Upsilon \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon'  \hyp{2}\\
       \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \varphi  \ottsym{\}} \hyp{3}
    \end{gather}
    for some \(\ottnt{V}\), \(\ottnt{S'}\), \(\ottmv{x}\) and \(\Upsilon\).  By applying IH
    of \hypref{3} to \hypref{imply}, we have
    \begin{gather}
       \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon'  \mid  \varphi'  \ottsym{\}} \hyp{5}.
    \end{gather}
    Now the goal can be derived by \ruleref{Sem-Push} and \hypref{5}.  \qedhere
  \end{match}
\end{prop}

\endinput

\begin{prop}{semty/logical/push}
  If \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}\), then
  \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{V}  \triangleright  \ottnt{S}  \ottsym{:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}}\).

  \proof By \propref{semty/logic/exists=>subst}, we have \( \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}}\).  So the goal can be derived by \ruleref{Sem-Push}.
\end{prop}


\begin{prop}{semty/logical/inv}
  If \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{V}  \triangleright  \ottnt{S}  \ottsym{:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}}\), then
  \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}\).

  \proof We have \( \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}}\) by
  \propref{semty/inv(push)}.  To this end,
  \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}\) is obtained by
  \propref{semty/logic/subst=>exists}.
\end{prop}

\endinput

\begin{prop}{semty/wf}
  If \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} p\} >>}}\), then \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \varphi  : \mathord{*} \).

  \proof The proof is done by induction on the given derivation.
  \AI{I think we could just say ``By straightfortward induction''.}
  \begin{match}
  \item[\ruleref{Sem-Bottom}] We have the following hypothesis.
    \begin{gather}
      \Gamma  \models  \varphi \hyp{1}\\
       \Upsilon \ottsym{=} \ddagger  \hyp{2}
    \end{gather}
    So, the goal follows by \propref{def/sem/pred}.
    
  \item[\ruleref{Sem-Push}] We have the following hypothesis.
    \begin{gather}
       \ottnt{S} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S'}  \hyp{1}\\
       \Upsilon \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon'  \hyp{2}\\
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}} \hyp{3}\\
      \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S' : ***\{xTs' \mbox{$\mid$} exists x:T. p /\mbox{$\backslash{}$} x = V\} >>}} \hyp{4}
    \end{gather}
    \( \Gamma  \ottsym{,}   \widehat{ \Upsilon' }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  : \mathord{*} \) by IH of \hypref{4}.
    Then, the goal \( \Gamma  \ottsym{,}   \widehat{ \Upsilon' }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}    \vdash   \varphi  : \mathord{*} \) follows by
    \propref{ftyping/inv(exists)}, \propref{ftyping/inv(and)}.
  \end{match}
\end{prop}

\begin{prop}{semty/inv}
  Every following statement holds.
  \AI{We don't even have to state.}
  \begin{statements}
  \item[bottom] If \(\texttt{\textcolor{red}{<<no parses (char 7): G \mbox{$\mid$}= \_ ***: \{\_ \mbox{$\mid$} p\} >>}}\), then \(\Gamma  \models  \varphi\).
  \item[push] If \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** S : \{x:T :. xTs \mbox{$\mid$} p\} >>}}\), then \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\)
    and \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T. p /\mbox{$\backslash{}$} x = V\} >>}}\).
  \end{statements}

  \proof Trivial.
\end{prop}

\begin{prop}{semty/exists=>subst}
  If \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T. p /\mbox{$\backslash{}$} x = V\} >>}}\), then \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$}
    p.\{V/x\}\} >>}}\).
  \AI{We don't even have to state.}

  \proof We have \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  : \mathord{*} \) by
  \propref{semty/wf}.  Then, \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}    \vdash   \varphi  : \mathord{*} \) and
  \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\) by \propref{ftyping/inv(exists)}, \propref{ftyping/inv(and)}
  \YN{TODO: we need to know variables are monomorphic}.  So, we have
  \(\texttt{\textcolor{red}{<<no parses (char 48): G \mbox{$\mid$}- \{xTs \mbox{$\mid$} exists x:T. p /\mbox{$\backslash{}$} x = V\} <: \{xTs \mbox{$\mid$} p.***\{V/x\}\} >>}}\) by
  \propref{subty/exists=>subst}.  Consequently, the goal follows by
  \propref{subty/sound}.
\end{prop}

\begin{prop}{semty/strengthen}
  Every following statement holds.
  \AI{We don't even have to state them, either.  If we'd like to state anything, why not stating a more general property like ``If $\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} phi1\} >>}}$ and $\Gamma  \ottsym{,}   \widehat{ \Upsilon }   \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}}$, then $\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} phi2\} >>}}$''?}
  
  \begin{statements}
  \item[drop] If \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T. p /\mbox{$\backslash{}$} x = V\} >>}}\), then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T. p\} >>}}\).
  \item[dup] If \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T. p /\mbox{$\backslash{}$} x = V\} >>}}\), then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T. (exists y:T. p /\mbox{$\backslash{}$} y = x /\mbox{$\backslash{}$} y = V) /\mbox{$\backslash{}$} x =
      V\} >>}}\).
  \item[swap] If
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists y:T2. (exists x:T1. p /\mbox{$\backslash{}$} x = V1) /\mbox{$\backslash{}$} y = V2\} >>}}\),
    then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T1. (exists y:T2. p /\mbox{$\backslash{}$} y = V2) /\mbox{$\backslash{}$} x = V1\} >>}}\).
  \item[push] If \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\) and \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} p\} >>}}\), then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T. (p /\mbox{$\backslash{}$} x = V) /\mbox{$\backslash{}$} x = V\} >>}}\).
  \item[tf] If \(\ottnt{i}  \neq  0\) and
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x = i\} >>}}\), then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists y:int. (exists x:int. p /\mbox{$\backslash{}$} (x <> 0 /\mbox{$\backslash{}$} y = 0 \mbox{$\backslash{}$}/ x
      = 0 /\mbox{$\backslash{}$} y = 1)) /\mbox{$\backslash{}$} y = 0\} >>}}\).
  \item[ft] If \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x = 0\} >>}}\), then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists y:int. (exists x:int. p /\mbox{$\backslash{}$} (x <> 0 /\mbox{$\backslash{}$} y = 0 \mbox{$\backslash{}$}/ x
      = 0 /\mbox{$\backslash{}$} y = 1)) /\mbox{$\backslash{}$} y = 1\} >>}}\).
  \item[add] If \( \ottnt{i_{{\mathrm{1}}}}  \ottsym{+}  \ottnt{i_{{\mathrm{2}}}} \ottsym{=} \ottnt{i_{{\mathrm{3}}}} \) and
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists y:int. (exists x:int. p /\mbox{$\backslash{}$} x = i1) /\mbox{$\backslash{}$} y =
      i2\} >>}}\), then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists z:int. (exists x:int, y:int. p /\mbox{$\backslash{}$} x + y = z) /\mbox{$\backslash{}$} z
      = i3\} >>}}\).
  \item[pair] If
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists y:T2. (exists x:T1. p /\mbox{$\backslash{}$} x = V1) /\mbox{$\backslash{}$} y = V2\} >>}}\),
    then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists z:T1*T2. (exists x:T1, y:T2. p /\mbox{$\backslash{}$} (x, y) = z) /\mbox{$\backslash{}$}
      z = (V1, V2)\} >>}}\).
  \item[car] If \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T1*T2. p /\mbox{$\backslash{}$} x = (V1, V2)\} >>}}\), then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x1:T1. (exists x:T1*T2, x2:T2. p /\mbox{$\backslash{}$} x = (x1, x2))
      /\mbox{$\backslash{}$} x1 = V1\} >>}}\).
  \item[cdr] If \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T1*T2. p /\mbox{$\backslash{}$} x = (V1, V2)\} >>}}\), then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x2:T2. (exists x:T1*T2, x1:T1. p /\mbox{$\backslash{}$} x = (x1, x2))
      /\mbox{$\backslash{}$} x2 = V2\} >>}}\).
  \item[cons] If
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x2:T list. (exists x1:T. p /\mbox{$\backslash{}$} x1 = V1) /\mbox{$\backslash{}$} x2 =
      V2\} >>}}\), then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x3:T list. (exists x1:T, x2:T list. p /\mbox{$\backslash{}$} x1 :: x2
      = x3) /\mbox{$\backslash{}$} x3 = V1 :: V2\} >>}}\).
  \item[ift] If \(\ottnt{i}  \neq  0\) and
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x = i\} >>}}\), then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x <> 0\} >>}}\).
  \item[ifconst] If \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T list. p /\mbox{$\backslash{}$} x = V1 :: V2\} >>}}\),
    then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists z:T list. (exists y:T. (exists x:T list. p /\mbox{$\backslash{}$} y
      :: z = x) /\mbox{$\backslash{}$} y = V1) /\mbox{$\backslash{}$} z = V2\} >>}}\).
  \item[iter] If \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T list. p /\mbox{$\backslash{}$} V1 :: V2 = x\} >>}}\),
    then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists y:T. (exists x:T list. p /\mbox{$\backslash{}$} y :: V2 = x) /\mbox{$\backslash{}$} y =
      V1\} >>}}\).
  \item[transfertokens] If
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x1:T1. (exists x2:T2. (exists x3:T3. p /\mbox{$\backslash{}$} x3 =
      V3) /\mbox{$\backslash{}$} x2 = V2) /\mbox{$\backslash{}$} x1 = V1\} >>}}\), then
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x3:T3, x2:T2, x1:T1. p\} >>}}\).
  \item[existsandforall] If \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} (exists x:T. p1 /\mbox{$\backslash{}$} x = V) /\mbox{$\backslash{}$}
      forall x:T. p2\} >>}}\), then \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T. p1 /\mbox{$\backslash{}$} p2
  /\mbox{$\backslash{}$} x = V\} >>}}\).
  \end{statements}

  \proof Every statement can be proven by using lemmas in
  \propref{fol/thm/misc}, \propref{fol/thm/valid}, \propref{subty/sound}.  We
  show the proof of the first statement.  We have
  \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  : \mathord{*} \) by \propref{semty/wf}.  From
  that, we can have \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  : \mathord{*} \).  Hence,
  \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{)}  \implies  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  : \mathord{*} \) by
  \ruleref{WF-Imply}.  Then, by \propref{fol/thm/valid},
  \propref{fol/thm/misc(drop1)}, we have
  \(\Gamma  \ottsym{,}   \widehat{ \Upsilon }   \models  \ottsym{(}  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{)}  \implies  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi\).  So,
  \(\Gamma  \vdash  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}  \ottsym{<:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \ottsym{\}}\) by
  \propref{def/subty}.  Now the goal follows by \propref{subty/sound}.
\end{prop}

\begin{prop}{semty/append/thm}
  If
  \begin{gather}
    \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} p1\} >>}} \hyp{semty}\\
    \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \models  \varphi_{{\mathrm{2}}} \hyp{thm}
  \end{gather}
  then \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} p1 /\mbox{$\backslash{}$} p2\} >>}}\).

  \proof The proof is done by induction on the given derivation of
  \hypref{semty}.
  \AI{I think we could just say ``By straightfortward induction''.}
  \begin{match}
  \item[\ruleref{Sem-Bottom}] We have the following hypothesis.
    \begin{gather}
       \ottnt{S} \ottsym{=} \ddagger  \hyp{1}\\
       \Upsilon \ottsym{=} \ddagger  \hyp{2}\\
      \Gamma  \models  \varphi_{{\mathrm{1}}} \hyp{3}
    \end{gather}
    So, \(\Gamma  \models  \varphi_{{\mathrm{1}}}  \wedge  \varphi_{{\mathrm{2}}}\) by applying \propref{fol/andI} to \hypref{thm},
    \hypref{3}.  Then, the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{\(\Gamma  \models  \varphi_{{\mathrm{1}}}  \wedge  \varphi_{{\mathrm{2}}}\)}%
      \RightLabel{\ruleref{Sem-Bottom}}%
      \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 7): G \mbox{$\mid$}= \_ ***: \{\_ \mbox{$\mid$} p1 /\mbox{$\backslash{}$} p2\} >>}}\)}%
    \end{prooftree}
    
  \item[\ruleref{Sem-Push}] We have the following hypothesis.
    \begin{gather}
       \ottnt{S} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S'}  \hyp{1}\\
       \Upsilon \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon'  \hyp{2}\\
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}} \hyp{3}\\
      \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S' : ***\{xTs' \mbox{$\mid$} exists x:T. p1 /\mbox{$\backslash{}$} x = V\} >>}} \hyp{4}
    \end{gather}
    We have \(\Gamma  \ottsym{,}   \widehat{ \Upsilon' }   \models  \forall \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi\) by \propref{fol/forallI},
    \hypref{thm}, \hypref{2}.  So, by IH, \hypref{4}, we have
    \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S' : ***\{xTs' \mbox{$\mid$} (exists x:T. p1 /\mbox{$\backslash{}$} x = V) /\mbox{$\backslash{}$} forall x:T. p2\} >>}}\).
    Then, by \propref{semty/strengthen(existsandforall)}, we have
    \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S' : ***\{xTs' \mbox{$\mid$} exists x:T. p1 /\mbox{$\backslash{}$} p2 /\mbox{$\backslash{}$} x = V\} >>}}\).  Consequently, the
    goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 6): \mbox{$\mid$}=V : ***T >>}}\) by \hypref{3}}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S' : ***\{xTs' \mbox{$\mid$} exists x:T. p1 /\mbox{$\backslash{}$} p2 /\mbox{$\backslash{}$} x = V\} >>}}\)}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** S' : \{x:T :. xTs' \mbox{$\mid$} p1 /\mbox{$\backslash{}$} p2\} >>}}\)}%
    \end{prooftree}
  \end{match}
\end{prop}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper.otex"
%%% End:


==> proofs/subty.tex <==
\subsection{Properties for subtyping}


\begin{prop}{subty/conservative}
  If \(\Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}\), then \(  \lfloor  \Phi_{{\mathrm{1}}}  \rfloor  \ottsym{=}  \lfloor  \Phi_{{\mathrm{2}}}  \rfloor  \).

  \proof The proof is straightforward by structural induction on the type
  binding stack of \(\Phi_{{\mathrm{1}}}\).
\end{prop}


\begin{prop}{subty/wf}
  If \(\Gamma  \vdash  \ottsym{\{}  \Upsilon  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}}  \ottsym{<:}  \ottsym{\{}  \Upsilon  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}\), then \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \)
  and \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \).

  \proof By definition, we have \(\Gamma  \ottsym{,}   \widehat{ \Upsilon }   \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}}\), and so,
  \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}}  : \mathord{*} \).  Now the goal follows from
  \propref{fol/wf/inv(imply)}.
\end{prop}


\begin{prop}[name=Soundness of subtyping]{subty/sound}
  If
  \begin{gather}
    \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{subty}\\
    \sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \Phi_{{\mathrm{1}}} \hyp{semty}
  \end{gather}
  then \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{S}  \ottsym{:}  \Phi_{{\mathrm{2}}}\).

  \proof By \propref{def/subty} of \hypref{subty}, we have
  \begin{gather}
     \Phi_{{\mathrm{1}}} \ottsym{=} \ottsym{\{}  \Upsilon  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}}  \hyp{1}\\
     \Phi_{{\mathrm{2}}} \ottsym{=} \ottsym{\{}  \Upsilon  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \hyp{2}\\
    \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}} \hyp{3}
  \end{gather}
  for some \(\Upsilon\), \(\varphi_{{\mathrm{1}}}\), and \(\varphi_{{\mathrm{2}}}\).
  So, the goal follows by \propref{semty/logic/imply}, \hypref{semty}, and \hypref{3}.
  \begin{comment}
  \proof The proof is done by induction on the given derivation of
  \hypref{semty}.
  \begin{match}
  \item[\ruleref{Sem-Bottom}] We have the following hypothesis for some \(\varphi_{{\mathrm{1}}}\).
    \begin{gather}
       \ottnt{S} \ottsym{=} \ddagger  \hyp{1}\\
       \Phi_{{\mathrm{1}}} \ottsym{=} \ottsym{\{}  \ddagger  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}}  \hyp{2}\\
      \sigma  \ottsym{:}  \Gamma  \models  \varphi_{{\mathrm{1}}} \hyp{2.5}
    \end{gather}
    So, by \propref{def/subty} of \hypref{subty}, we have
    \begin{gather}
       \Phi_{{\mathrm{2}}} \ottsym{=} \ottsym{\{}  \ddagger  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \hyp{3}\\
      \Gamma  \ottsym{,}   \widehat{ \ddagger }   \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}} \hyp{4}
    \end{gather}
    for some \(\varphi_{{\mathrm{2}}}\).  By \propref{def/sem/formula} of \hypref{4}, we have
    \begin{gather}
      \sigma  \ottsym{:}  \Gamma  \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}} \hyp{5}.
    \end{gather}
    Now we have
    \begin{gather}
      \sigma  \ottsym{:}  \Gamma  \models  \varphi_{{\mathrm{2}}} \hyp{6}
    \end{gather}
    by \propref{def/sem/formula} of \hypref{5} and \hypref{2.5}.  Finally, the
    goal \(\sigma  \ottsym{:}  \Gamma  \models  \ddagger  \ottsym{:}  \ottsym{\{}  \ddagger  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}\) can be derived by \ruleref{Sem-Bottom} and
    \hypref{6}.

  \item[\ruleref{Sem-Push}] We have the following hypothesis for some
    \(\ottnt{V}\), \(\ottnt{S'}\), \(\ottmv{x}\), \(\ottnt{T}\), \(\Upsilon\), and \(\varphi_{{\mathrm{1}}}\).
    \begin{gather}
       \ottnt{S} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S'}  \hyp{1}\\
       \Phi_{{\mathrm{1}}} \ottsym{=} \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}}  \hyp{2}\\
       \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \hyp{4}
    \end{gather}
    By \propref{def/subty} of \hypref{subty}, we have
    \begin{gather}
       \Phi_{{\mathrm{2}}} \ottsym{=} \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \hyp{5}\\
      \Gamma  \ottsym{,}   \widehat{  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon }   \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}} \hyp{6}
    \end{gather}
    for some \(\varphi_{{\mathrm{2}}}\).  So, by \propref{def/subty}, \hypref{6}, we have
    \begin{gather}
      \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \vdash  \ottsym{\{}  \Upsilon  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}}  \ottsym{<:}  \ottsym{\{}  \Upsilon  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}} \hyp{7}.
    \end{gather}
    Now applying IH of \hypref{4} to \hypref{7}, we have
    \begin{gather}
       \sigma  [  \ottmv{x}  \mapsto  \ottnt{V}  ]   \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \ottnt{S'}  \ottsym{:}  \ottsym{\{}  \Upsilon  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}} \hyp{9}.
    \end{gather}
    So, the goal \(\sigma  \ottsym{:}  \Gamma  \models  \ottnt{V}  \triangleright  \ottnt{S'}  \ottsym{:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}\) can be derived by
    \ruleref{Sem-Push} and \hypref{9}.  \qedhere
  \end{match}
\end{comment}
\end{prop}


\endinput

\begin{prop}[name=Well-sortedness of predicates in subtyping]{subty/wf}
  If \(\Gamma  \vdash  \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}}  \ottsym{<:}  \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}\), then
  \( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{1}}} }    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) and \( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \).

  \proof \( \Upsilon_{{\mathrm{1}}} \ottsym{=} \Upsilon_{{\mathrm{2}}} \) and \(\Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{1}}} }   \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}}\) by
  definition.  So, \( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{1}}} }    \vdash   \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}}  : \mathord{*} \), and then the goal can
  be obtained by \AI{inversion}.
\end{prop}

\begin{prop}[name=Reflexivity of subtyping]{subty/refl}
  If \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \varphi  : \mathord{*} \), then \(\Gamma  \vdash  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}}  \ottsym{<:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}}\).

  \proof \(\Gamma  \ottsym{,}   \widehat{ \Upsilon }   \models  \varphi  \implies  \varphi\) by \propref{fol/imply/refl}.  Thus, the
  goal follows by \propref{def/subty}.
\end{prop}

\begin{prop}[name=Transitivity of subtyping]{subty/trans}
  If
  \begin{gather}
    \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{1}\\
    \Gamma  \vdash  \Phi_{{\mathrm{2}}}  \ottsym{<:}  \Phi_{{\mathrm{3}}} \hyp{2}
  \end{gather}
  then \(\Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \Phi_{{\mathrm{3}}}\).

  \proof We have \( \Phi_{{\mathrm{1}}} \ottsym{=} \ottsym{\{}  \Upsilon  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \), \( \Phi_{{\mathrm{2}}} \ottsym{=} \ottsym{\{}  \Upsilon  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}} \),
  \(\Gamma  \ottsym{,}   \widehat{ \Upsilon }   \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}}\) by \propref{def/subty} of \hypref{1}.  Then,
  \( \Phi_{{\mathrm{3}}} \ottsym{=} \ottsym{\{}  \Upsilon  \mid  \varphi_{{\mathrm{3}}}  \ottsym{\}} \), \(\Gamma  \ottsym{,}   \widehat{ \Upsilon }   \models  \varphi_{{\mathrm{2}}}  \implies  \varphi_{{\mathrm{3}}}\) also by
  \propref{def/subty} of \hypref{2}.  Now \(\Gamma  \ottsym{,}   \widehat{ \Upsilon }   \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{3}}}\) by
  \propref{fol/imply/trans}.  As a result, the goal follows by
  \propref{def/subty}.
\end{prop}

\begin{prop}[name=Substitution for subtyping]{subty/subst}
  If
  \begin{gather}
    \Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma_{{\mathrm{2}}}  \vdash  \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}}  \ottsym{<:}  \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}} \hyp{subty} \\
    \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}} \hyp{vtyping}
  \end{gather}
  then \(\texttt{\textcolor{red}{<<no parses (char 21): G1, G2 \mbox{$\mid$}- \{xTs1 \mbox{$\mid$} p1.***\{V/x\}\} <: \{xTs2 \mbox{$\mid$} p2.\{V/x\}\} >>}}\).

  \proof We have the following by the definition of \hypref{subty}.
  \begin{gather}
     \Upsilon_{{\mathrm{1}}} \ottsym{=} \Upsilon_{{\mathrm{2}}}  \hyp{1}\\
    \Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma_{{\mathrm{2}}}  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{1}}} }   \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}} \hyp{2}
  \end{gather}
  So, \(\texttt{\textcolor{red}{<<no parses (char 24): G1, G2, rev(xTs1) \mbox{$\mid$}= p1.***\{V/x\} ==> p2.\{V/x\} >>}}\) follows by applying
  \propref{fol/subst} to \hypref{vtyping} and \hypref{2}.  Now the goal follows
  by \propref{def/subty}.
\end{prop}

\begin{prop}{subty/exists=>subst}
  If \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}    \vdash   \varphi  : \mathord{*} \) and \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\), then
  \(\texttt{\textcolor{red}{<<no parses (char 48): G \mbox{$\mid$}- \{xTs \mbox{$\mid$} exists x:T. p /\mbox{$\backslash{}$} x = V\} <: \{xTs \mbox{$\mid$} p.***\{V/x\}\} >>}}\).

  \proof By \propref{def/subty}, it is enough to show
  \begin{gather*}
    \texttt{\textcolor{red}{<<no parses (char 46): G, rev(xTs) \mbox{$\mid$}= (exists x:T. p /\mbox{$\backslash{}$} x = V) ==> p.***\{V/x\} >>}}.
  \end{gather*}
  To prove the above by \propref{fol/thm/exists=>subst},
  \propref{fol/thm/valid}, what we need to show is
  \begin{gather*}
    \texttt{\textcolor{red}{<<no parses (char 46): G, rev(xTs) \mbox{$\mid$}- (exists x:T. p /\mbox{$\backslash{}$} x = V) ==> p.***\{V/x\} : * >>}}.
  \end{gather*}
  The above can be derived with given assumptions and  \propref{ttyping/strut(fsubst)}.
\end{prop}

\begin{prop}{subty/subst=>exists}
  If \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}    \vdash   \varphi  : \mathord{*} \) and \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\), then
  \(\texttt{\textcolor{red}{<<no parses (char 14): G \mbox{$\mid$}- \{xTs \mbox{$\mid$} p.***\{V/x\}\} <: \{xTs \mbox{$\mid$} exists x:T. p /\mbox{$\backslash{}$} x = V\} >>}}\).

  \proof By \propref{def/subty}, it is enough to show
  \begin{gather*}
    \texttt{\textcolor{red}{<<no parses (char 17): G, rev(xTs) \mbox{$\mid$}= p.***\{V/x\} ==> exists x:T. p /\mbox{$\backslash{}$} x = V >>}}.
  \end{gather*}
  To prove the above by \propref{fol/thm/subst=>exists},
  \propref{fol/thm/valid}, what we need to show is
  \begin{gather*}
    \texttt{\textcolor{red}{<<no parses (char 17): G, rev(xTs) \mbox{$\mid$}- p.***\{V/x\} ==> exists x:T. p /\mbox{$\backslash{}$} x = V : * >>}}.
  \end{gather*}
  The above can be derived with given assumptions and \propref{ttyping/strut(fsubst)}.
\end{prop}

\begin{prop}[name=Soundness of subtyping]{subty/sound}
  If
  \begin{gather}
    \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{subty}\\
    \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***P1 >>}} \hyp{semty}
  \end{gather}
  then \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***P2 >>}}\).

  \proof The proof is done by induction on the given derivation of
  \hypref{semty}.
  \begin{match}
  \item[\ruleref{Sem-Bottom}] We have
    \begin{gather}
       \ottnt{S} \ottsym{=} \ddagger  \hyp{1}\\
       \Phi_{{\mathrm{1}}} \ottsym{=} \ottsym{\{}  \ddagger  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}}  \hyp{2}\\
      \Gamma  \models  \varphi_{{\mathrm{1}}} \hyp{3}
    \end{gather}
    for some $\varphi_{{\mathrm{1}}}$.
    Thus, by \propref{def/subty} and \hypref{subty}, we have
    \begin{gather}
       \Phi_{{\mathrm{2}}} \ottsym{=} \ottsym{\{}  \ddagger  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \hyp{4}\\
      \Gamma  \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}} \hyp{5}
    \end{gather}
    for some $\varphi_{{\mathrm{2}}}$.
    By \propref{fol/mp}, \hypref{3}, \hypref{5}, we have
    \(\Gamma  \models  \varphi_{{\mathrm{2}}}\), from which the goal is derived by \ruleref{Sem-Bottom}.

  \item[\ruleref{Sem-Push}] We have
    \begin{gather}
       \ottnt{S} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S'}  \hyp{1}\\
       \Phi_{{\mathrm{1}}} \ottsym{=} \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}}  \hyp{2}\\
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}} \hyp{3}\\
      \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S' : ***\{xTs \mbox{$\mid$} exists x:T. p1 /\mbox{$\backslash{}$} x = V\} >>}} \hyp{4}
    \end{gather}
    for some $\ottnt{V}, \ottnt{S'}, \ottnt{T}, \Upsilon$ and $\varphi_{{\mathrm{1}}}$.
    Thus, by \propref{def/subty} and \hypref{subty}, we have
    \begin{gather}
       \Phi_{{\mathrm{2}}} \ottsym{=} \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \hyp{5}\\
      \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \models  \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}} \hyp{6}
    \end{gather}
    for some $\varphi_{{\mathrm{2}}}$.
    We have \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}    \vdash   \varphi_{{\mathrm{1}}}  \implies  \varphi_{{\mathrm{2}}}  : \mathord{*} \) by \propref{def/sem/pred}
    and \hypref{6}, and so, applying \propref{ftyping/inv(imply)}, we have
    \begin{gather}
       \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*}  \hyp{7}\\
       \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}    \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*}  \ . \hyp{8}
    \end{gather}
    Therefore, applying \propref{subty/exists=>subst} and
    \propref{subty/subst=>exists} to \hypref{3}, \hypref{7} and \hypref{3},
    \hypref{8}, we have
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 50): G \mbox{$\mid$}- \{xTs \mbox{$\mid$} exists x:T. p1 /\mbox{$\backslash{}$} x = V\} <: \{xTs \mbox{$\mid$} p1.***\{V/x\}\} >>}} \hyp{10}\\
      \texttt{\textcolor{red}{<<no parses (char 15): G \mbox{$\mid$}- \{xTs \mbox{$\mid$} p2.***\{V/x\}\} <: \{xTs \mbox{$\mid$} exists x:T. p2 /\mbox{$\backslash{}$} x = V\} >>}} \ . \hyp{11}
    \end{gather}
    Applying \propref{fol/subst} to \hypref{3}, \hypref{6}, we have
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 18): G, rev(xTs) \mbox{$\mid$}= p1.***\{V/x\} ==> p2.\{V/x\} >>}}. \hyp{9}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 15): G \mbox{$\mid$}- \{xTs \mbox{$\mid$} p1.***\{V/x\}\} <: \{xTs \mbox{$\mid$} p2.\{V/x\}\} >>}}\) by
    \propref{def/subty}.  Now,
    \(\Gamma  \vdash  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}  \ottsym{<:}  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi_{{\mathrm{2}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}\) by \propref{subty/trans}.  Finally, we can derive the goal as
    follows.
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\) by \hypref{3}}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S' : ***\{xTs \mbox{$\mid$} exists x:T. p2 /\mbox{$\backslash{}$} x = V\} >>}}\) by IH}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** S' : \{x:T :. xTs \mbox{$\mid$} p2\} >>}}\)}%
    \end{prooftree}
  \end{match}
\end{prop}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper.otex"
%%% End:


==> proofs/tmp.tex <==
\begin{itemize}
\item If \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** S : \{xTs \mbox{$\mid$} exists x:T. p /\mbox{$\backslash{}$} x = V\} >>}}\), then
  \(\texttt{\textcolor{red}{<<no parses (char 9): s.[V/x] \mbox{$\mid$}***= S : \{xTs \mbox{$\mid$} p\} >>}}\).
\item If \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\) and \(\texttt{\textcolor{red}{<<no parses (char 9): s.[V/x] \mbox{$\mid$}***= S : \{xTs \mbox{$\mid$} p\} >>}}\), then
  \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** S : \{xTs \mbox{$\mid$} exists x:T. p /\mbox{$\backslash{}$} x = V\} >>}}\).
\item If \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** S : \{xTs \mbox{$\mid$} p\} >>}}\) and \(\texttt{\textcolor{red}{<<no parses (char 11): \mbox{$\mid$}= p ==> p'*** >>}}\), then
  \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** S : \{xTs \mbox{$\mid$} p'\} >>}}\).

\item If \(\texttt{\textcolor{red}{<<no parses (char 5): \mbox{$\mid$}= p'*** >>}}\), then \(\texttt{\textcolor{red}{<<no parses (char 18): \mbox{$\mid$}= p ==> (p /\mbox{$\backslash{}$} p')*** >>}}\).
\item \(\texttt{\textcolor{red}{<<no parses (char 47): \mbox{$\mid$}= (exists x:T. p /\mbox{$\backslash{}$} x = V) ==> (exists x:T. p)*** >>}}\).
\item
  \(\texttt{\textcolor{red}{<<no parses (char 95): \mbox{$\mid$}= (exists x:T. p /\mbox{$\backslash{}$} x = V) ==> (exists x:T. (exists x':T. (p /\mbox{$\backslash{}$} x' = x)
  /\mbox{$\backslash{}$} x' = V) /\mbox{$\backslash{}$} x = V)*** >>}}\).
\item
  \(\texttt{\textcolor{red}{<<no parses (char 111): \mbox{$\mid$}= (exists x:T. (exists x':T. p /\mbox{$\backslash{}$} x' = V') /\mbox{$\backslash{}$} x = V) ==> (exists
  x':T'. (exists x:T. p /\mbox{$\backslash{}$} x = V) /\mbox{$\backslash{}$} x' = V')*** >>}}\).
\item If \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\), then
  \(\texttt{\textcolor{red}{<<no parses (char 44): \mbox{$\mid$}= p ==> (exists x:T. (p /\mbox{$\backslash{}$} x = V) /\mbox{$\backslash{}$} x = V)*** >>}}\).
\item If \(\ottnt{i}  \neq  0\), then
  \(\texttt{\textcolor{red}{<<no parses (char 76): \mbox{$\mid$}= (exists x:int. p /\mbox{$\backslash{}$} x = i) ==> (exists x':int. (exists x:int. p /\mbox{$\backslash{}$} (x
  !***= 0 /\mbox{$\backslash{}$} x' = 0 \mbox{$\backslash{}$}/ x = 0 /\mbox{$\backslash{}$} x' = 1)) /\mbox{$\backslash{}$} x' = 0) >>}}\).
\item
  \(\texttt{\textcolor{red}{<<no parses (char 76): \mbox{$\mid$}= (exists x:int. p /\mbox{$\backslash{}$} x = 0) ==> (exists x':int. (exists x:int. p /\mbox{$\backslash{}$} (x
  !***= 0 /\mbox{$\backslash{}$} x' = 0 \mbox{$\backslash{}$}/ x = 0 /\mbox{$\backslash{}$} x' = 1)) /\mbox{$\backslash{}$} x' = 1) >>}}\).
\item If \( \ottnt{i_{{\mathrm{1}}}}  \ottsym{+}  \ottnt{i_{{\mathrm{2}}}} \ottsym{=} \ottnt{i_{{\mathrm{3}}}} \), then \(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= i3 : ***int >>}}\).
\item If \( \ottnt{i_{{\mathrm{1}}}}  \ottsym{+}  \ottnt{i_{{\mathrm{2}}}} \ottsym{=} \ottnt{i_{{\mathrm{3}}}} \), then
  \(\texttt{\textcolor{red}{<<no parses (char 137): \mbox{$\mid$}= (exists x2:int. (exists x1:int. p /\mbox{$\backslash{}$} x1 = i1) /\mbox{$\backslash{}$} x2 = i2) ==> (exists
  x3:int. (exists x1:int, x2:int. p /\mbox{$\backslash{}$} x1 + x2 = x3) /\mbox{$\backslash{}$} x3 = i3)*** >>}}\).
\item
  \(\texttt{\textcolor{red}{<<no parses (char 142): \mbox{$\mid$}= (exists x2:T2. (exists x1:T1. p /\mbox{$\backslash{}$} x1 = V1) /\mbox{$\backslash{}$} x2 = V2) ==> (exists
  x3:T1*T2. (exists x1:T1, x2:T2. p /\mbox{$\backslash{}$} (x1, x2) = x3) /\mbox{$\backslash{}$} x3 = (V1, V2))*** >>}}\).
\item
  \(\texttt{\textcolor{red}{<<no parses (char 114): \mbox{$\mid$}= (exists x:T1*T2. p /\mbox{$\backslash{}$} x = (V1, V2)) ==> (exists x1:T1. (exists x:T1*T2,
  x2:T2. p /\mbox{$\backslash{}$} x = (x1, x2)) /\mbox{$\backslash{}$} x1 = V1)*** >>}}\).
\item
  \(\texttt{\textcolor{red}{<<no parses (char 114): \mbox{$\mid$}= (exists x:T1*T2. p /\mbox{$\backslash{}$} x = (V1, V2)) ==> (exists x2:T2. (exists x:T1*T2,
  x2:T2. p /\mbox{$\backslash{}$} x = (x1, x2)) /\mbox{$\backslash{}$} x2 = V2)*** >>}}\).
\item If \(\ottnt{i}  \neq  0\), then
  \(\texttt{\textcolor{red}{<<no parses (char 61): \mbox{$\mid$}= (exists x:int. p /\mbox{$\backslash{}$} x = i) ==> (exists x:int. p /\mbox{$\backslash{}$} x <> 0)*** >>}}\).
\item
  \(\texttt{\textcolor{red}{<<no parses (char 137): \mbox{$\mid$}= (exists x:T list. p /\mbox{$\backslash{}$} x = V1::V2) ==> (exists x2:T list. (exists
  x1:T. (exists x:T list. p /\mbox{$\backslash{}$} x1 :: x2 = x) /\mbox{$\backslash{}$} x1 = V1) /\mbox{$\backslash{}$} x2 = V2)*** >>}}\).
\item If \( \ottmv{x_{{\mathrm{2}}}}  \notin   \text{fvars}( \varphi )  \), then
  \(\texttt{\textcolor{red}{<<no parses (char 101): \mbox{$\mid$}= (exists x2:T list. (exists x:T list. p /\mbox{$\backslash{}$} x2 = x) /\mbox{$\backslash{}$} x2 = V2) ==>
  (exists x:T list. p /\mbox{$\backslash{}$} x = V2)*** >>}}\).
\item If \(\texttt{\textcolor{red}{<<no parses (char 10): \mbox{$\mid$}= <IS> : ***T1->T2 >>}}\), then
  \(\texttt{\textcolor{red}{<<no parses (char 202): \mbox{$\mid$}= (p /\mbox{$\backslash{}$} forall y1':T1, y1:T1, y2:T2. y1' = y1 /\mbox{$\backslash{}$} p1 /\mbox{$\backslash{}$} call(<IS>, y1') =
  y2 ==> p2) ==> (exists x:T1->T2. (p /\mbox{$\backslash{}$} forall y1':T1, y1:T1, y2:T2. y1' = y1
  /\mbox{$\backslash{}$} p1 /\mbox{$\backslash{}$} call(x, y1') = y2 ==> p2) /\mbox{$\backslash{}$} x = <IS>)*** >>}}\)
\item If \(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T2 >>}}\), then
  \(\texttt{\textcolor{red}{<<no parses (char 174): \mbox{$\mid$}= ((exists x2:T1->T2. (exists x1:T1. p /\mbox{$\backslash{}$} x1 = V1) /\mbox{$\backslash{}$} x2 = <IS>) /\mbox{$\backslash{}$}
  call(<IS>, V1) = V2) ==> (exists x3:T2. (exists x1:T1, x2:T1->T2. p /\mbox{$\backslash{}$}
  call(x2, x1) = x3) /\mbox{$\backslash{}$} x3 = V2)*** >>}}\).
\item
  \(\texttt{\textcolor{red}{<<no parses (char 216): \mbox{$\mid$}= (exists x3:address. (exists x2:int. (exists x1:T. p /\mbox{$\backslash{}$} x1 = V) /\mbox{$\backslash{}$} x2 =
  i) /\mbox{$\backslash{}$} x3 = a) ==> (exists x4:operation. (exists x1:T, x2:int, x3:address. p /\mbox{$\backslash{}$}
  x4 = transaction(x1, x2, x3)) /\mbox{$\backslash{}$} x4 = transaction(V, i, a))*** >>}}\).
\end{itemize}

\begin{rules}
  \infun{
    \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** p >>}}\)
  }{
    \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** \_ : \{\_ \mbox{$\mid$} p\} >>}}\)
  }
  \infbi{
    \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\)
  }{
    \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** S : \{xTs \mbox{$\mid$} exists x:T. p /\mbox{$\backslash{}$} x = V\} >>}}\)
  }{
    \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** V :. S : \{x:T :. xTs \mbox{$\mid$} p\} >>}}\)
  }
\end{rules}


\begin{prop}{typing/sound/iter'}
  If
  \begin{gather}
    \text{For any } \ottnt{S'_{{\mathrm{1}}}}, \ottnt{S'_{{\mathrm{2}}}}, \sigma', \text{ if } \ottnt{S'_{{\mathrm{1}}}}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S'_{{\mathrm{2}}}},
    \sigma'  \ottsym{:}  \Gamma  \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list} , \text{
      and } \texttt{\textcolor{red}{<<no parses (char 5): s' \mbox{$\mid$}=*** S1' : \{x1:T :. xTs \mbox{$\mid$} exists x:T list. p /\mbox{$\backslash{}$} x1 :: x2 = x\} >>}},
    \text{ then } \texttt{\textcolor{red}{<<no parses (char 5): s' \mbox{$\mid$}=*** S2' : \{xTs \mbox{$\mid$} exists x:T list. p /\mbox{$\backslash{}$} x2 = x\} >>}}
    \hyp{OIH}\\
    \ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{ITER} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{eval}\\
    \texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** S1 : \{x:T list :. xTs \mbox{$\mid$} p\} >>}} \hyp{semty}
  \end{gather}
  then \(\texttt{\textcolor{red}{<<no parses (char 4): s \mbox{$\mid$}=*** S2 : \{xTs \mbox{$\mid$} exists x:T list. p /\mbox{$\backslash{}$} x = []\} >>}}\).

  \proof The proof is done by induction on the given derivation of
  \hypref{eval}.
  \begin{match}
  \item[\ruleref{E-IterNil}]
    We have the following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{[}  \ottsym{]}  \triangleright  \ottnt{S_{{\mathrm{2}}}}  \hyp{1}
    \end{gather}
    So the goal follows by \propref{semty/inv(push)}, \hypref{semty},
    \hypref{1}.

  \item[\ruleref{E-IterCons}]
    We have the following hypothesis.
  \end{match}
\end{prop}
  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper.otex"
%%% End:


==> proofs/typing.tex <==
\section{Soundness of the refinement type system}

\begin{prop}{typing/conservative}
  The following two statements hold.
  \begin{statements}
  \item If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \mathit{IS} \; \Phi_{{\mathrm{2}}} \), then \( \lfloor  \Phi_{{\mathrm{1}}}  \rfloor   \vdash  \mathit{IS}  \Rightarrow   \lfloor  \Phi_{{\mathrm{2}}}  \rfloor \).
  \item If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottnt{I} \; \Phi_{{\mathrm{2}}} \), then \( \lfloor  \Phi_{{\mathrm{1}}}  \rfloor   \vdash  \ottnt{I}  \Rightarrow   \lfloor  \Phi_{{\mathrm{2}}}  \rfloor \).
  \end{statements}

  \proof The proof is straightforward by mutual induction on the given derivations.
  When the last step is derived by \ruleref{RT-Sub}, we use
  \propref{subty/conservative}.
\end{prop}


\begin{prop}{typing/wf}
  The following two statements hold.
  \begin{statements}
  \item If \( \Gamma \vdash \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \; \mathit{IS} \; \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}} \) and \( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{1}}} }    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \), then \( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \).
  \item If \( \Gamma \vdash \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \; \ottnt{I} \; \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}} \) and \( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{1}}} }    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \), then \( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \).
  \end{statements}

  \proof The proof is routine by mutual induction on the given refinement typing
  derivations.  We use \propref{fol/wf/strut} and \propref{subty/wf}.
\end{prop}


\endinput


\begin{prop}{typing/wf}
  If
  \begin{gather}
     \Gamma \vdash \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \; \ottnt{I} \; \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \hyp{typing}\\
     \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{1}}} }    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*}  \hyp{ftyping}
  \end{gather}
  then \( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \).

  \proof The proof is done by induction on the given derivation of
  \hypref{typing}.  \AI{Could we just say ``By straightfortward induction''?
    It's routine, isn't it?}
  \begin{match}
  \item[\ruleref{RT-Nop}] We know \( \Upsilon_{{\mathrm{1}}} \ottsym{=} \Upsilon_{{\mathrm{2}}} \) and \( \varphi_{{\mathrm{1}}} \ottsym{=} \varphi_{{\mathrm{2}}} \).  So,
    the goal equivalent to \hypref{ftyping}.
    
  \item[\ruleref{RT-Seq}] We have the following hypothesis.
    \begin{gather}
       \Gamma \vdash \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \; \ottnt{I_{{\mathrm{1}}}} \; \ottsym{\{}  \Upsilon'  \mid  \varphi'  \ottsym{\}}  \hyp{2}\\
       \Gamma \vdash \ottsym{\{}  \Upsilon'  \mid  \varphi'  \ottsym{\}} \; \ottsym{\{}  \ottnt{I_{{\mathrm{2}}}}  \ottsym{;} \, ... \, \ottsym{;}  \ottnt{I_{\ottmv{n}}}  \ottsym{\}} \; \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \hyp{3}
    \end{gather}
    So, \( \Gamma  \ottsym{,}   \widehat{ \Upsilon' }    \vdash   \varphi'  : \mathord{*} \) follows by IH of \hypref{2}, and thus,
    the goal \( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \) follows by IH of \hypref{3}.
    
  \item[\ruleref{RT-Dip}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon'_{{\mathrm{1}}}  \hyp{2}\\
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon'_{{\mathrm{2}}}  \hyp{3}\\
       \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}  \vdash \ottsym{\{}  \Upsilon'_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \; \mathit{IS} \; \ottsym{\{}  \Upsilon'_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \hyp{4}
    \end{gather}
    Applying \propref{ttyping/strut(fperm)} to \hypref{ftyping} with \hypref{2},
    we have \( \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \widehat{ \Upsilon'_{{\mathrm{1}}} }    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \).  So,
    \( \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \widehat{ \Upsilon'_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \) follows by IH of \hypref{4}.  Now the
    goal \( \Gamma  \ottsym{,}   \widehat{ \Upsilon'_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}    \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \) by \propref{ttyping/strut(fperm)}.
    
  \item[\ruleref{RT-Drop}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon_{{\mathrm{2}}}  \hyp{1}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \hyp{2}
    \end{gather}
    So, the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) by \hypref{ftyping}}%
      \RightLabel{\ruleref{WF-Exists}}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi_{{\mathrm{1}}}  : \mathord{*} \)}%
    \end{prooftree}
    
  \item[\ruleref{RT-Dup}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \hyp{1}\\
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x'} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon_{{\mathrm{1}}}  \hyp{2}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x'}  \ottsym{=}  \ottmv{x}  \hyp{3}
    \end{gather}
    So, the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) by
        \propref{ttyping/strut(fweaken)}, \hypref{ftyping}}%
      \AxiomC{\(( \ottmv{x'} \mathord:\allowbreak \ottnt{T}  \in \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} } )\)}%
      \RightLabel{\ruleref{WT-Var}}%
      \UnaryInfC{\(\Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \vdash  \ottmv{x'}  \ottsym{:}  \ottnt{T}\)}%
      \AxiomC{\(( \ottmv{x} \mathord:\allowbreak \ottnt{T}  \in \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} } )\)}%
      \RightLabel{\ruleref{WT-Var}}%
      \UnaryInfC{\(\Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \vdash  \ottmv{x}  \ottsym{:}  \ottnt{T}\)}%
      \RightLabel{\ruleref{WF-Equal}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \ottmv{x'}  \ottsym{=}  \ottmv{x}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x'}  \ottsym{=}  \ottmv{x}  : \mathord{*} \)}%
    \end{prooftree}
    
  \item[\ruleref{RT-Swap}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \hyp{1}\\
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \hyp{2}\\
       \varphi_{{\mathrm{1}}} \ottsym{=} \varphi_{{\mathrm{2}}}  \hyp{3}
    \end{gather}
    So, the goal follows by applying \propref{ttyping/strut(fperm)} to
    \hypref{ftyping}.
    
  \item[\ruleref{RT-Push}] We have the following hypothesis.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}} \hyp{1}\\
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon_{{\mathrm{1}}}  \hyp{2}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \hyp{3}
    \end{gather}
    So, the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) by
        \propref{ttyping/strut(fweaken)}, \hypref{ftyping}}%
      \AxiomC{(By routine)} \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \ottmv{x}  \ottsym{=}  \ottnt{V}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  : \mathord{*} \)}%
    \end{prooftree}
    
  \item[\ruleref{RT-Not}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \hyp{1}\\
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x'} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \hyp{2}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottsym{(}  \ottmv{x}  \neq  0  \wedge  \ottmv{x'}  \ottsym{=}  0  \vee  \ottmv{x}  \ottsym{=}  0  \wedge  \ottmv{x'}  \ottsym{=}  1  \ottsym{)}  \hyp{3}
    \end{gather}
    By applying \propref{ttyping/strut(fweaken)} and
    \propref{ttyping/strut(fperm)} to \hypref{ftyping}, we have
    \begin{gather}
       \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*}  \hyp{4}
    \end{gather}
    Now the goal can be derived as follows.
    % \begin{prooftree}
    %   \AxiomC{\(( \ottmv{x} \mathord:\allowbreak \ottkw{int}  \in \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int} )\)}%
    %   \RightLabel{\ruleref{WT-Var}}%
    %   \UnaryInfC{\(\Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \vdash  \ottmv{x}  \ottsym{:}  \ottkw{int}\)}%
    %   \AxiomC{}%
    %   \RightLabel{\ruleref{RTV-Int}}%
    %   \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= 0 : ***int >>}}\)}%
    %   \RightLabel{\ruleref{WT-Val}}%
    %   \UnaryInfC{\(\Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \vdash  0  \ottsym{:}  \ottkw{int}\)}%
    %   \RightLabel{\ruleref{WF-Equal}}%
    %   \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \ottmv{x}  \ottsym{=}  0  : \mathord{*} \)}%
    %   \RightLabel{\ruleref{WF-Not}}%
    %   \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \ottmv{x}  \neq  0  : \mathord{*} \)}%
    %   \AxiomC{\(( \ottmv{x'} \mathord:\allowbreak \ottkw{int}  \in \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int} )\)}%
    %   \RightLabel{\ruleref{WT-Var}}%
    %   \UnaryInfC{\(\Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \vdash  \ottmv{x'}  \ottsym{:}  \ottkw{int}\)}%
    %   \AxiomC{}%
    %   \RightLabel{\ruleref{RTV-Int}}%
    %   \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= 0 : ***int >>}}\)}%
    %   \RightLabel{\ruleref{WT-Val}}%
    %   \UnaryInfC{\(\Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \vdash  0  \ottsym{:}  \ottkw{int}\)}%
    %   \RightLabel{\ruleref{WF-Equal}}%
    %   \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \ottmv{x'}  \ottsym{=}  0  : \mathord{*} \)}%
    %   \RightLabel{\ruleref{WF-And}}%
    %   \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \ottmv{x}  \neq  0  \wedge  \ottmv{x'}  \ottsym{=}  0  : \mathord{*} \)}%
    % \end{prooftree}
    % \begin{prooftree}
    %   \AxiomC{\(( \ottmv{x} \mathord:\allowbreak \ottkw{int}  \in \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int} )\)}%
    %   \RightLabel{\ruleref{WT-Var}}%
    %   \UnaryInfC{\(\Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \vdash  \ottmv{x}  \ottsym{:}  \ottkw{int}\)}%
    %   \AxiomC{}%
    %   \RightLabel{\ruleref{RTV-Int}}%
    %   \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= 0 : ***int >>}}\)}%
    %   \RightLabel{\ruleref{WT-Val}}%
    %   \UnaryInfC{\(\Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \vdash  0  \ottsym{:}  \ottkw{int}\)}%
    %   \RightLabel{\ruleref{WF-Equal}}%
    %   \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \ottmv{x}  \ottsym{=}  0  : \mathord{*} \)}%
    %   \AxiomC{\(( \ottmv{x'} \mathord:\allowbreak \ottkw{int}  \in \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int} )\)}%
    %   \RightLabel{\ruleref{WT-Var}}%
    %   \UnaryInfC{\(\Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \vdash  \ottmv{x'}  \ottsym{:}  \ottkw{int}\)}%
    %   \AxiomC{}%
    %   \RightLabel{\ruleref{RTV-Int}}%
    %   \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= 1 : ***int >>}}\)}%
    %   \RightLabel{\ruleref{WT-Val}}%
    %   \UnaryInfC{\(\Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \vdash  1  \ottsym{:}  \ottkw{int}\)}%
    %   \RightLabel{\ruleref{WF-Equal}}%
    %   \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \ottmv{x'}  \ottsym{=}  1  : \mathord{*} \)}%
    %   \RightLabel{\ruleref{WF-And}}%
    %   \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \ottmv{x}  \ottsym{=}  0  \wedge  \ottmv{x'}  \ottsym{=}  1  : \mathord{*} \)}%
    % \end{prooftree}
    \begin{prooftree}
      \AxiomC{\hypref{4}}%
      \AxiomC{(By routine)}
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \ottmv{x}  \neq  0  \wedge  \ottmv{x'}  \ottsym{=}  0  \vee  \ottmv{x}  \ottsym{=}  0  \wedge  \ottmv{x'}  \ottsym{=}  1  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottsym{(}  \ottmv{x}  \neq  0  \wedge  \ottmv{x'}  \ottsym{=}  0  \vee  \ottmv{x}  \ottsym{=}  0  \wedge  \ottmv{x'}  \ottsym{=}  1  \ottsym{)}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-Exists}}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottsym{(}  \ottmv{x}  \neq  0  \wedge  \ottmv{x'}  \ottsym{=}  0  \vee  \ottmv{x}  \ottsym{=}  0  \wedge  \ottmv{x'}  \ottsym{=}  1  \ottsym{)}  : \mathord{*} \)}%
    \end{prooftree}
    
  \item[\ruleref{RT-Add}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottkw{int}   \triangleright   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \hyp{1}\\
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \hyp{2}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{+}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  \hyp{3}
    \end{gather}
    By applying \propref{ttyping/strut(fweaken)} and
    \propref{ttyping/strut(fperm)} to \hypref{ftyping}, we have
    \begin{gather}
       \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} . \hyp{4}
    \end{gather}
    Now the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{\hypref{4}}%
      \AxiomC{(By routine)}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}    \vdash   \ottmv{x_{{\mathrm{1}}}}  \ottsym{+}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{+}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-Exists} twice}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x_{{\mathrm{1}}}}  \ottsym{+}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  : \mathord{*} \)}%
    \end{prooftree}
    
  \item[\ruleref{RT-Pair}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \hyp{1}\\
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \hyp{2}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  \hyp{3}
    \end{gather}
    So, the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{By \propref{ttyping/strut(fweaken)},
        \propref{ttyping/strut(fperm)}, \hypref{ftyping}}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \)}%
      \AxiomC{(By routine)}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-Exists} twice}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  : \mathord{*} \)}%
    \end{prooftree}

  \item[\ruleref{RT-CAR}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \hyp{1}\\
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright  \Upsilon  \hyp{2}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  \hyp{3}
    \end{gather}
    So, the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{By \propref{ttyping/strut(fweaken)},
        \propref{ttyping/strut(fperm)}, \hypref{ftyping}}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \)}%
      \AxiomC{(By routine)}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-Exists} twice}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  : \mathord{*} \)}%
    \end{prooftree}
    
  \item[\ruleref{RT-CDR}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \hyp{1}\\
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \hyp{2}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  \hyp{3}
    \end{gather}
    So, the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{By \propref{ttyping/strut(fweaken)},
        \propref{ttyping/strut(fperm)}, \hypref{ftyping}}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \)}%
      \AxiomC{(By routine)}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}    \vdash   \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-Exists} twice}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  : \mathord{*} \)}%
    \end{prooftree}
    
  \item[\ruleref{RT-Nil}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon_{{\mathrm{1}}}  \hyp{1}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  \hyp{2}
    \end{gather}
    So, the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) by
        \propref{ttyping/strut(fweaken)}, \hypref{ftyping}}%
      \AxiomC{(By routine)}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  : \mathord{*} \)}%
    \end{prooftree}
    
  \item[\ruleref{RT-Cons}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \triangleright   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \hyp{1}\\
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \hyp{2}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  \hyp{3}
    \end{gather}
    So, the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{By \propref{ttyping/strut(fweaken)},
        \propref{ttyping/strut(fperm)}, \hypref{ftyping}}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \)}%
      \AxiomC{(By routine)}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}    \vdash   \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-Exists} twice}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  : \mathord{*} \)}%
    \end{prooftree}
    
  \item[\ruleref{RT-If}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \hyp{1}\\
       \Gamma \vdash \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  0  \ottsym{\}} \; \mathit{IS}_{{\mathrm{2}}} \; \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \hyp{2}
    \end{gather}
    We can derive \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  0  : \mathord{*} \) as
    follows.
    \begin{prooftree}
      \AxiomC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) by \hypref{ftyping}}%
      \AxiomC{(By routine)}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \ottmv{x}  \ottsym{=}  0  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  0  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-Exists}}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  0  : \mathord{*} \)}%
    \end{prooftree}
    So, the goal follows by IH of \hypref{2}.
    
  \item[\ruleref{RT-Loop}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon_{{\mathrm{2}}}  \hyp{1}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  0  \hyp{2}
    \end{gather}
    So, the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) by \hypref{ftyping}}%
      \AxiomC{(By routine)}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \ottmv{x}  \ottsym{=}  0  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottkw{int}    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  0  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-Exists}}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  0  : \mathord{*} \)}%
    \end{prooftree}
    
  \item[\ruleref{RT-IfCons}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \hyp{1}\\
       \Gamma \vdash \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  \ottsym{\}} \; \mathit{IS}_{{\mathrm{2}}} \; \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \hyp{2}
    \end{gather}
    We can derive \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  : \mathord{*} \) as
    follows.
    \begin{prooftree}
      \AxiomC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) by \hypref{ftyping}}%
      \AxiomC{(By routine)}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}    \vdash   \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-Exists}}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  : \mathord{*} \)}%
    \end{prooftree}
    So, the goal follows by IH of \hypref{2}.

  \item[\ruleref{RT-Iter}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon_{{\mathrm{2}}}  \hyp{1}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  \hyp{2}
    \end{gather}
    So, the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) by \hypref{ftyping}}%
      \AxiomC{(By routine)}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}    \vdash   \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-Exists}}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  : \mathord{*} \)}%
    \end{prooftree}
    
  \item[\ruleref{RT-Lambda}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon_{{\mathrm{1}}}  \hyp{1}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \varphi_{{\mathrm{1}}}  \wedge  \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{11}}}  \wedge   \ottkw{call} ( \ottmv{x} ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{12}}}  \hyp{2}\\
        \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}    \vdash   \varphi_{{\mathrm{11}}}  : \mathord{*}  \hyp{3}\\
        \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \vdash \ottsym{\{}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright  \ddagger  \mid  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{11}}}  \ottsym{\}} \; \mathit{IS} \; \ottsym{\{}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \ddagger  \mid  \varphi_{{\mathrm{12}}}  \ottsym{\}}  \hyp{4}
    \end{gather}
    We can have the following derivation.
    \begin{prooftree}
      \AxiomC{(By routine)}%
      \UnaryInfC{\(  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}    \vdash   \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  : \mathord{*} \)}%
      \AxiomC{\(  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}    \vdash   \varphi_{{\mathrm{11}}}  : \mathord{*} \) by \hypref{3}}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\(  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}    \vdash   \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{11}}}  : \mathord{*} \)}%
    \end{prooftree}
    So, \(  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \varphi_{{\mathrm{12}}}  : \mathord{*} \) by IH.  Then, we have the following
    hypothesis by \propref{ttyping/strut(fweaken)}.
    \begin{gather*}
        \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \varphi_{{\mathrm{12}}}  : \mathord{*}  \\
        \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{11}}}  : \mathord{*} 
    \end{gather*}
    Now we can derive
    \begin{gather*}
        \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}    \vdash   \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{11}}}  \wedge   \ottkw{call} ( \ottmv{x} ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{12}}}  : \mathord{*} .
    \end{gather*}
    Again by \propref{ttyping/strut(fweaken)}, we have
    \begin{gather*}
       \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*}  \\
       \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}    \vdash   \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{11}}}  \wedge   \ottkw{call} ( \ottmv{x} ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{12}}}  : \mathord{*} .
    \end{gather*}
    The goal can be derived from the above.
  
  \item[\ruleref{RT-Exec}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \hyp{1}\\
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \hyp{2}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottmv{x_{{\mathrm{3}}}}   \hyp{3}
    \end{gather}
    So, the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{By \propref{ttyping/strut(fweaken)},
        \propref{ttyping/strut(fperm)}, \hypref{ftyping}}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \)}%
      \AxiomC{(By routine)}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}    \vdash    \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottmv{x_{{\mathrm{3}}}}   : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}    \vdash   \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottmv{x_{{\mathrm{3}}}}   : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-Exists} twice}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottmv{x_{{\mathrm{3}}}}   : \mathord{*} \)}%
    \end{prooftree}
    
  \item[\ruleref{RT-TransferTokens}] We have the following hypothesis.
    \begin{gather}
       \Upsilon_{{\mathrm{1}}} \ottsym{=}  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \triangleright   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \triangleright   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{address}   \triangleright  \Upsilon  \hyp{1}\\
       \Upsilon_{{\mathrm{2}}} \ottsym{=}  \ottmv{x_{{\mathrm{4}}}} \mathord:\allowbreak \ottkw{operation}   \triangleright  \Upsilon  \hyp{2}\\
       \varphi_{{\mathrm{2}}} \ottsym{=} \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{address}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x_{{\mathrm{4}}}}  \ottsym{=}   \texttt{Transfer}  (  \ottmv{x_{{\mathrm{1}}}} ,  \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{3}}}}  )   \hyp{3}
    \end{gather}
    So, the goal can be derived as follows.
    \begin{prooftree}
      \AxiomC{(By routine)}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{address}    \vdash   \ottmv{x_{{\mathrm{4}}}}  \ottsym{=}   \texttt{Transfer}  (  \ottmv{x_{{\mathrm{1}}}} ,  \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{3}}}}  )   : \mathord{*}  \quad (\ast)\)}%
    \end{prooftree}
    \begin{prooftree}
      \AxiomC{By \propref{ttyping/strut(fweaken)},
        \propref{ttyping/strut(fperm)}, \hypref{ftyping}}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{address}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \)}%
      \AxiomC{$(\ast)$}%
      \RightLabel{\ruleref{WF-And}}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{address}    \vdash   \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x_{{\mathrm{4}}}}  \ottsym{=}   \texttt{Transfer}  (  \ottmv{x_{{\mathrm{1}}}} ,  \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{3}}}}  )   : \mathord{*} \)}%
      \RightLabel{\ruleref{WF-Exists} three times}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{address}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x_{{\mathrm{4}}}}  \ottsym{=}   \texttt{Transfer}  (  \ottmv{x_{{\mathrm{1}}}} ,  \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{3}}}}  )   : \mathord{*} \)}%
    \end{prooftree}
    
  \item[\ruleref{RT-Sub}] We have the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi'_{{\mathrm{2}}}  \ottsym{<:}  \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}} \hyp{2}
    \end{gather}
    So, the goal follows by \propref{subty/wf}.
  \end{match}
\end{prop}


\endinput


\begin{prop}[name=Inversion of typing]{typing/inv}
  Let \(\Gamma\) be a typing environment.
  Suppose \( \Phi_{{\mathrm{1}}} \ottsym{=} \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \) such that \( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{1}}} }    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \).
  Every following statement holds.
  \AI{We might want to introduce well-formedness for $\Phi$.}
  \AI{Do we need inversion, even when we prove the main theorem by induction on type derivations?}
  \begin{statements}
  \item[nop] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottsym{\{}  \ottsym{\}} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \Phi \\
      \Gamma  \vdash  \Phi  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}
    \AI{Add ``for some $\Phi$.'' (and delete the period above). Similarly for the other items.}

  \item[seq] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottsym{\{}  \ottnt{I_{{\mathrm{1}}}}  \ottsym{;}  \ottnt{I_{{\mathrm{2}}}}  \ottsym{;} \, ... \, \ottsym{;}  \ottnt{I_{\ottmv{n}}}  \ottsym{\}} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \Phi'_{{\mathrm{1}}} \\
       \Gamma \vdash \Phi'_{{\mathrm{1}}} \; \ottnt{I_{{\mathrm{1}}}} \; \Phi  \\
       \Gamma \vdash \Phi \; \ottsym{\{}  \ottnt{I_{{\mathrm{2}}}}  \ottsym{;} \, ... \, \ottsym{;}  \ottnt{I_{\ottmv{n}}}  \ottsym{\}} \; \Phi'_{{\mathrm{2}}}  \\
      \Gamma  \vdash  \Phi'_{{\mathrm{2}}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}

  \item[dip] \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{DIP} \, \mathit{IS} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \\
       \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}  \vdash \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \; \mathit{IS} \; \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}

  \item[drop] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{DROP} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}

  \item[dup] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{DUP} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{y} \mathord:\allowbreak \ottnt{T}   \triangleright   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi  \wedge  \ottmv{y}  \ottsym{=}  \ottmv{x}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}

  \item[swap] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{SWAP} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright   \ottmv{y} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{y} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}

  \item[push] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{PUSH} \, \ottnt{T} \, \ottnt{V} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \\
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}.
    \end{gather*}

  \item[not] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{NOT} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{y} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottsym{(}  \ottmv{x}  \neq  0  \wedge  \ottmv{y}  \ottsym{=}  0  \vee  \ottmv{x}  \ottsym{=}  0  \wedge  \ottmv{y}  \ottsym{=}  1  \ottsym{)}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}

  \item[add] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{ADD} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright   \ottmv{y} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{z} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{y} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{+}  \ottmv{y}  \ottsym{=}  \ottmv{z}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}

  \item[pair] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{PAIR} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright   \ottmv{y} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{z} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge  \ottsym{(}  \ottmv{x}  \ottsym{,}  \ottmv{y}  \ottsym{)}  \ottsym{=}  \ottmv{z}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}

  \item[car] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{CAR} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}

  \item[cdr] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{CDR} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}

  \item[nil] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{NIL} \, \ottnt{T} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}

  \item[cons] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{CONS} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \triangleright   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}

  \item[if] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{IF} \, \mathit{IS}_{{\mathrm{1}}} \, \mathit{IS}_{{\mathrm{2}}} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \texttt{\textcolor{red}{<<no parses (char 6): G \mbox{$\mid$}= \{***xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x <> 0\} IS1 P2 >>}} \\
      \texttt{\textcolor{red}{<<no parses (char 6): G \mbox{$\mid$}= \{***xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x = 0\} IS2 P2 >>}}.
    \end{gather*}

  \item[loop] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{LOOP} \, \mathit{IS} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  0  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \\
       \Gamma \vdash \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \neq  0  \ottsym{\}} \; \mathit{IS} \; \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} .
    \end{gather*}

  \item[ifcons] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \texttt{IF\symbol{95}CONS} \, \mathit{IS}_{{\mathrm{1}}} \, \mathit{IS}_{{\mathrm{2}}} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
       \Gamma \vdash \ottsym{\{}   \ottmv{y} \mathord:\allowbreak \ottnt{T}   \triangleright   \ottmv{z} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{y}  ::  \ottmv{z}  \ottsym{=}  \ottmv{x}  \ottsym{\}} \; \mathit{IS}_{{\mathrm{1}}} \; \Phi_{{\mathrm{2}}}  \\
       \Gamma \vdash \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  \ottsym{\}} \; \mathit{IS}_{{\mathrm{2}}} \; \Phi_{{\mathrm{2}}} .
    \end{gather*}

  \item[iter] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{ITER} \, \mathit{IS} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \\
       \Gamma  \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}  \vdash \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{\}} \; \mathit{IS} \; \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{\}} .
    \end{gather*}

  \item[lambda] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{LAMBDA} \, \ottnt{T_{{\mathrm{1}}}} \, \ottnt{T_{{\mathrm{2}}}} \, \mathit{IS} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \texttt{\textcolor{red}{<<no parses (char 10): \mbox{$\mid$}= <IS> : ***T1->T2 >>}}\\
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}}\\
        \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \\
      \texttt{\textcolor{red}{<<no parses (char 11): y1':T1 \mbox{$\mid$}= \{***y1:T1 :. \_ \mbox{$\mid$} y1' = y1 /\mbox{$\backslash{}$} p1\} IS \{y2:T2 :. \_ \mbox{$\mid$} p2\} >>}}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \varphi  \wedge  \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} ( \ottmv{x} ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}
    \end{gather*}

  \item[exec] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottkw{EXEC} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge   \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottmv{x_{{\mathrm{3}}}}   \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}

  \item[transfertokens] If \( \Gamma \vdash \Phi_{{\mathrm{1}}} \; \texttt{TRANSFER\symbol{95}TOKENS} \, \ottnt{T} \; \Phi_{{\mathrm{2}}} \), then
    \begin{gather*}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \triangleright   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \triangleright   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{address}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x_{{\mathrm{4}}}} \mathord:\allowbreak \ottkw{operation}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{address}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{4}}}}  \ottsym{=}   \texttt{Transfer}  (  \ottmv{x_{{\mathrm{1}}}} ,  \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{3}}}}  )   \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}.
    \end{gather*}
  \end{statements}

  \proof Every statement can be proven by induction on the given derivation,
  using \propref{subty/refl}, \propref{typing/wf} in a base case and
  \propref{subty/trans} in an inductive case.  To show the first goal of
  \propref{typing/inv(lambda)}, we use \propref{typing/conservative}.
\end{prop}

\subsubsection{Substitution lemma}

\begin{prop}{typing/subst}
  If \( \Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma_{{\mathrm{2}}} \vdash \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \; \ottnt{I} \; \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}} \) and \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\), then
  \(\texttt{\textcolor{red}{<<no parses (char 21): G1, G2 \mbox{$\mid$}- \{xTs1 \mbox{$\mid$} p1.***\{V/x\}\} I \{xTs2 \mbox{$\mid$} p2.\{V/x\}\} >>}}\).

  \proof By straightforward induction on the given derivation of
  \( \Gamma_{{\mathrm{1}}}  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}  \Gamma_{{\mathrm{2}}} \vdash \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \; \ottnt{I} \; \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}} \) with
  \propref{subty/subst}.
\end{prop}

\begin{prop}{typing/subst=>exists}
  If
  \begin{gather}
     \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}  \vdash \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \; \ottnt{I} \; \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \hyp{1}\\
     \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{1}}} }    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*}  \hyp{2}\\
    \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}} \hyp{3}
  \end{gather}
  then
  \( \Gamma \vdash \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}} \; \ottnt{I} \; \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi_{{\mathrm{2}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}} \).

  \proof Applying \propref{typing/subst} to \hypref{1}, \hypref{3}, we have the
  following hypothesis.
  \begin{gather}
    \texttt{\textcolor{red}{<<no parses (char 16): G \mbox{$\mid$}- \{xTs1 \mbox{$\mid$} p1.***\{V/x\}\} I \{xTs2 \mbox{$\mid$} p2.\{V/x\}\} >>}} \hyp{3}
  \end{gather}
  We have \( \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \) by applying \propref{typing/wf} to
  \hypref{1}, \hypref{2}.  So, we have the following hypothesis by applying
  \propref{subty/exists=>subst} and \propref{subty/subst=>exists}, respectively.
  \begin{gather}
    \texttt{\textcolor{red}{<<no parses (char 52): G \mbox{$\mid$}- \{xTs1 \mbox{$\mid$} exists x:T. p1 /\mbox{$\backslash{}$} x = V\} <: \{xTs1 \mbox{$\mid$} p1.***\{V/x\}\} >>}} \hyp{4}\\
    \texttt{\textcolor{red}{<<no parses (char 16): G \mbox{$\mid$}- \{xTs2 \mbox{$\mid$} p2.***\{V/x\}\} <: \{xTs2 \mbox{$\mid$} exists x:T. p2 /\mbox{$\backslash{}$} x = V\} >>}} \hyp{5}
  \end{gather}
  Now the goal follows by \ruleref{RT-Sub} with \hypref{3}, \hypref{4}, \hypref{5}.
\end{prop}

\subsubsection{Soundness}

\begin{prop}{typing/sound/loop} Suppose $\mathit{IS}$ satisfies
  \begin{gather}
    \text{for any } \ottnt{S_{{\mathrm{1}}}}, \ottnt{S_{{\mathrm{2}}}} \text{ if } \ottnt{S_{{\mathrm{1}}}}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \text{ and }
    \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x <> 0\} >>}} \text{ then } \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 :
***    \{x:int :. xTs \mbox{$\mid$} p\} >>}}. \hyp{OIH}
  \end{gather}
  If
  \begin{gather}
    \ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{LOOP} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{eval}\\
    \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***\{x:int :. xTs \mbox{$\mid$} p\} >>}} \hyp{semty}
  \end{gather}
  then \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x = 0\} >>}}\).

  \proof The proof is done by induction on the given derivation of
  \hypref{eval}.
  \begin{match}
  \item[\ruleref{E-LoopT}] We have the following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{i}  \triangleright  \ottnt{S}  \hyp{h1}\\
      \ottnt{i}  \neq  0 \hyp{h2}\\
      \ottnt{S}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S'} \hyp{h3}\\
      \ottnt{S'}  \vdash  \ottkw{LOOP} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{h4}
    \end{gather}
    By applying \propref{semty/inv(push)}, we have the following hypothesis.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= i : ***int >>}} \hyp{h5}\\
      \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x = i\} >>}} \hyp{h6}
    \end{gather}
    Then, we have \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x <> 0\} >>}}\) by
    \propref{semty/strengthen(ift)}, \hypref{h2}, \hypref{h6}.  Applying
    \hypref{OIH} to \hypref{h3}, \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S' : ***\{x:int :. xTs \mbox{$\mid$} p\} >>}}\).  Now the
    goal follows by IH.

  \item[\ruleref{E-LoopF}] We have the following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} 0  \triangleright  \ottnt{S_{{\mathrm{2}}}}  \hyp{h1}
    \end{gather}
    So the goal \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x = 0\} >>}}\) follows by
    applying \propref{semty/inv(push)} on \hypref{semty}.
  \end{match}
\end{prop}

\begin{prop}{typing/sound/iter}
  Suppose \AI{Do we need $ \ottmv{x_{{\mathrm{1}}}}  \notin   \text{fvars}( \varphi )  $, too?}
  \begin{gather}
     \ottmv{x_{{\mathrm{2}}}}  \notin   \text{fvars}( \varphi )   \hyp{fv} \\
     \Gamma  \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}  \vdash \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{\}} \; \mathit{IS} \; \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{\}}  \hyp{type} \\
    \text{For any } \Gamma, \Phi_{{\mathrm{1}}}, \Phi_{{\mathrm{2}}}, \ottnt{S_{{\mathrm{1}}}}, \ottnt{S_{{\mathrm{2}}}}, \text{ if }  \Gamma \vdash \Phi_{{\mathrm{1}}} \; \mathit{IS} \; \Phi_{{\mathrm{2}}} , \ottnt{S_{{\mathrm{1}}}}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}, \text{ and } \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***P1 >>}}, \text{ then }
    \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***P2 >>}} \hyp{OIH}
  \end{gather}
  For any \(\ottnt{S_{{\mathrm{1}}}}, \ottnt{S_{{\mathrm{2}}}}\), if
  \begin{gather}
    \ottnt{S_{{\mathrm{1}}}}  \vdash  \ottkw{ITER} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{eval}\\
    \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***\{x:T list :. xTs \mbox{$\mid$} p\} >>}} \hyp{semty}
  \end{gather}
  then \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***\{xTs \mbox{$\mid$} exists x:T list. p /\mbox{$\backslash{}$} x = []\} >>}}\).

  \proof The proof is done by induction on the given derivation of
  \hypref{eval}.
  \begin{match}
  \item[\ruleref{E-IterNil}] We have the following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{[}  \ottsym{]}  \triangleright  \ottnt{S_{{\mathrm{2}}}}  \hyp{h1}
    \end{gather}
    So, the goal follows by applying \propref{semty/inv(push)} to
    \hypref{semty}.

  \item[\ruleref{E-IterCons}] We have the following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{h1}\\
      \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{S}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S'} \hyp{h2}\\
      \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S'}  \vdash  \ottkw{ITER} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{h3}
    \end{gather}
    So, applying \propref{semty/inv(push)} to \hypref{semty}, we have the
    following hypothesis.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 14): \mbox{$\mid$}= V1 :: V2 : ***T list >>}} \hyp{h4}\\
      \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T list. p /\mbox{$\backslash{}$} x = V1 :: V2\} >>}} \hyp{h5}
    \end{gather}
    Applying \propref{vtyping/inv(cons)} to \hypref{h4}, we also have
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T >>}} \hyp{h6}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T list >>}} \hyp{h7}.
    \end{gather}
    So, by \propref{typing/subst}, \hypref{fv}, \hypref{type}, \hypref{h7},
    we have
    \begin{gather}
       \Gamma \vdash \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{\}} \; \mathit{IS} \; \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottnt{V_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{\}} . \hyp{h8}
    \end{gather}
    We can have the following derivation.
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T >>}}\) by \hypref{h6}}%
      \AxiomC{By applying \propref{semty/strengthen(iter)} to \hypref{h5}}%
      \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x1:T. (exists x:T list. p /\mbox{$\backslash{}$} x1 :: V2 =
          x) /\mbox{$\backslash{}$} x1 = V1\} >>}}\)}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V1 :.*** S : \{x1:T :. xTs \mbox{$\mid$} exists x:T list. p /\mbox{$\backslash{}$} x1 ::
          V2 = x\} >>}}\)}
    \end{prooftree}
    Now applying \hypref{OIH} with conclusion above, \hypref{h8}, and
    \hypref{h2}, we have \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S' : ***\{xTs \mbox{$\mid$} exists x:T list. p /\mbox{$\backslash{}$} V2 = x\} >>}}\);
    and then, we can have the following derivation.
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T list >>}}\)}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S' : ***\{xTs \mbox{$\mid$} exists x:T list. p /\mbox{$\backslash{}$} V2 = x\} >>}}\)}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V2 :.*** S' : \{x:T list :. xTs \mbox{$\mid$} p\} >>}}\)}
    \end{prooftree}
    Now, the goal follows by IH.
  \end{match}
\end{prop}

\begin{prop}[name=Soundness, type=theorem]{typing/sound}
  If
  \begin{gather}
     \Gamma \vdash \Phi_{{\mathrm{1}}} \; \ottnt{I} \; \Phi_{{\mathrm{2}}}  \hyp{type} \\
    \ottnt{S_{{\mathrm{1}}}}  \vdash  \ottnt{I}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{eval} \\
    \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***P1 >>}} \hyp{semty}
  \end{gather}
  then \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***P2 >>}}\).
  \AI{We prove also the ``instruction sequence version'' by mutual induction.
  I think we are mainly interested in that version.}

  \proof First of all, we know \( \Phi_{{\mathrm{1}}} \ottsym{=} \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \) such that
  \( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{1}}} }    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*} \) by \propref{semty/wf}, \hypref{semty}; and
  thus, \( \Phi_{{\mathrm{2}}} \ottsym{=} \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}} \) such that \( \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{2}}} }    \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*} \) by
  \propref{typing/wf}.  The proof is done by structural induction on \(\ottnt{I}\).
  \begin{match}
  \item[\( \ottnt{I} \ottsym{=} \ottsym{\{}  \ottsym{\}} \)] \AI{$ \mathit{IS} \ottsym{=} \ottsym{\{}  \ottsym{\}} $?} By applying \propref{typing/inv(nop)} to \hypref{type},
    we have the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \Phi \hyp{h1}\\
      \Gamma  \vdash  \Phi  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{h2}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***P2 >>}}\) by \propref{subty/sound}, \hypref{semty},
    \hypref{h1}, \hypref{h2}.  It is the goal because \( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{S_{{\mathrm{2}}}} \) by
    applying \propref{eval/inv(nop)} to \hypref{eval}.

  \item[\( \ottnt{I} \ottsym{=} \ottsym{\{}  \ottnt{I_{{\mathrm{1}}}}  \ottsym{;}  \ottnt{I_{{\mathrm{2}}}}  \ottsym{;} \, ... \, \ottsym{;}  \ottnt{I_{\ottmv{n}}}  \ottsym{\}} \)] \AI{$ \mathit{IS} \ottsym{=} \ottsym{\{}  \ottnt{I_{{\mathrm{1}}}}  \ottsym{;}  \ottnt{I_{{\mathrm{2}}}}  \ottsym{;} \, ... \, \ottsym{;}  \ottnt{I_{\ottmv{n}}}  \ottsym{\}} $?} By applying \propref{typing/inv(seq)} to
    \hypref{type}, we have the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \Phi'_{{\mathrm{1}}} \hyp{h1}\\
       \Gamma \vdash \Phi'_{{\mathrm{1}}} \; \ottnt{I_{{\mathrm{1}}}} \; \Phi  \hyp{h2}\\
       \Gamma \vdash \Phi \; \ottsym{\{}  \ottnt{I_{{\mathrm{2}}}}  \ottsym{;} \, ... \, \ottsym{;}  \ottnt{I_{\ottmv{n}}}  \ottsym{\}} \; \Phi'_{{\mathrm{2}}}  \hyp{h3}\\
      \Gamma  \vdash  \Phi'_{{\mathrm{2}}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{h4}
    \end{gather}
    By applying \propref{eval/inv(seq)} to \hypref{eval}, we have the following
    hypothesis.
    \begin{gather}
      \ottnt{S_{{\mathrm{1}}}}  \vdash  \ottnt{I_{{\mathrm{1}}}}  \Downarrow  \ottnt{S} \hyp{h5}\\
      \ottnt{S}  \vdash  \ottsym{\{}  \ottnt{I_{{\mathrm{2}}}}  \ottsym{;} \, ... \, \ottsym{;}  \ottnt{I_{\ottmv{n}}}  \ottsym{\}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{h6}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***P1' >>}}\) by \propref{subty/sound} to \hypref{semty},
    \hypref{h1}; \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***P >>}}\) by IH; \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***P2' >>}}\) by IH; and
    then; the goal \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***P2 >>}}\) by \propref{subty/sound}, \hypref{h4}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{DIP} \, \mathit{IS} \)] By applying \propref{typing/inv(dip)} to
    \hypref{type}, we have the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \hyp{h1}\\
       \Gamma  \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}  \vdash \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \varphi_{{\mathrm{1}}}  \ottsym{\}} \; \mathit{IS} \; \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \hyp{h2}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon_{{\mathrm{2}}}  \mid  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{h3}
    \end{gather}
    By applying \propref{eval/inv(dip)} to \hypref{eval}, we have the following
    hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S'_{{\mathrm{1}}}}  \hyp{h4}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S'_{{\mathrm{2}}}}  \hyp{h5}\\
      \ottnt{S'_{{\mathrm{1}}}}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S'_{{\mathrm{2}}}} \hyp{h6}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** S1' : \{x:T :. xTs1 \mbox{$\mid$} p1\} >>}}\) by \propref{subty/sound}; and
    then, we have the following hypothesis by \propref{semty/inv(push)}.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}} \hyp{h7}\\
      \texttt{\textcolor{red}{<<no parses (char 11): G \mbox{$\mid$}= S1' : ***\{xTs1 \mbox{$\mid$} exists x:T. p1 /\mbox{$\backslash{}$} x = V\} >>}} \hyp{h8}
    \end{gather}
    We also have the following hypothesis by \propref{semty/wf}.
    \begin{gather}
       \Gamma  \ottsym{,}   \widehat{ \Upsilon_{{\mathrm{1}}} }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*}  \hyp{9}
    \end{gather}
    We have
    \( \Gamma \vdash \ottsym{\{}  \Upsilon_{{\mathrm{1}}}  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi_{{\mathrm{1}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}} \; \mathit{IS} \; \ottsym{\{}  \Upsilon_{{\mathrm{2}}}  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi_{{\mathrm{2}}}  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}} \) by \propref{typing/subst=>exists}, \hypref{h2}, \hypref{h7},
    \hypref{9}.  Now, we can have the following derivation.
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\) by \hypref{h7}}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 11): G \mbox{$\mid$}= S2' : ***\{xTs2 \mbox{$\mid$} exists x:T. p2 /\mbox{$\backslash{}$} x = V\} >>}}\) by IH,
        \hypref{h6}, \hypref{h8}}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** S2' : \{x:T :. xTs2 \mbox{$\mid$} p2\} >>}}\)}%
    \end{prooftree}
    Finally, the goal \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** S2' : P2 >>}}\) follows by
    \propref{subty/sound}, \hypref{h3}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{DROP} \)] By applying \propref{typing/inv(drop)}, we have the
    following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{h1}\\
      \Gamma  \vdash  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T}   \ottsym{.}  \varphi  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{h2}
    \end{gather}
    By applying \propref{eval/inv(drop)}, we have the following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S_{{\mathrm{2}}}}  \hyp{h3}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** S2 : \{x:T :. xTs \mbox{$\mid$} p\} >>}}\) by \propref{subty/sound}; and
    then, \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\) and \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***\{xTs \mbox{$\mid$} exists x:T. p /\mbox{$\backslash{}$} x = V\} >>}}\)
    by \propref{semty/inv(push)}.  We have
    \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***\{xTs \mbox{$\mid$} exists x:T. p\} >>}}\) by \propref{semty/strengthen(drop)}.
    Therefore, the goal \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***P2 >>}}\) follows by \propref{subty/sound}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{DUP} \)] By applying \propref{typing/inv(dup)}, we have the
    following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{h1}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{y} \mathord:\allowbreak \ottnt{T}   \triangleright   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi  \wedge  \ottmv{y}  \ottsym{=}  \ottmv{x}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{h2}
    \end{gather}
    By applying \propref{eval/inv(dup)}, we have the following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S}  \hyp{h3}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{V}  \triangleright  \ottnt{S}  \hyp{h4}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** S : \{x:T :. xTs \mbox{$\mid$} p\} >>}}\) by \propref{subty/sound}; and
    then, \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\) and \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T. p /\mbox{$\backslash{}$} x = V\} >>}}\)
    by \propref{semty/inv(push)}.  Now we can derive
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** V :. S : \{y:T :. x:T :. xTs \mbox{$\mid$} p /\mbox{$\backslash{}$} y = x\} >>}}\) as follows.
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\)}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\)}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T. (exists y:T. p /\mbox{$\backslash{}$} y = x /\mbox{$\backslash{}$} y = V)
          /\mbox{$\backslash{}$} x = V\} >>}}\) by \propref{semty/strengthen(dup)}}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** S : \{x:T :. xTs \mbox{$\mid$} exists y:T. p /\mbox{$\backslash{}$} y = x /\mbox{$\backslash{}$} y =
          V\} >>}}\)}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** V :. S : \{y:T :. x:T :. xTs \mbox{$\mid$} p /\mbox{$\backslash{}$} y = x\} >>}}\)}
    \end{prooftree}
    Finally, the goal follows by \propref{subty/sound}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{SWAP} \)] By applying \propref{typing/inv(swap)}, we have the
    following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright   \ottmv{y} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{h1}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{y} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{h2}
    \end{gather}
    By applying \propref{eval/inv(swap)}, we have the following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{h3}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{S}  \hyp{h4}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V1 :.*** V2 :. S : \{x:T1 :. y:T2 :. xTs \mbox{$\mid$} p\} >>}}\) by
    \propref{subty/sound}; and then we have the following hypothesis by applying
    \propref{semty/inv(push)} twice.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T1 >>}} \hyp{h4}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T2 >>}} \hyp{h5}\\
      \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists y:T2. (exists x:T1. p /\mbox{$\backslash{}$} x = V1) /\mbox{$\backslash{}$} y = V2\} >>}}
      \hyp{h6}
    \end{gather}
    Now we can derive \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V2 :.*** V1 :. S : \{y:T2 :. x:T1 :. xTs \mbox{$\mid$} p\} >>}}\) as
    follows.
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T2 >>}}\)}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T1 >>}}\)}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T1. (exists y:T2. p /\mbox{$\backslash{}$} y = V2) /\mbox{$\backslash{}$} x =
          V1\} >>}}\) by \propref{semty/strengthen(swap)}}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V1 :.*** S : \{x:T1 :. xTs \mbox{$\mid$} exists y:T2. p /\mbox{$\backslash{}$} y =
          V2\} >>}}\)}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V2 :.*** V1 :. S : \{y:T2 :. x:T1 :. xTs \mbox{$\mid$} p\} >>}}\)}
    \end{prooftree}
    Finally, the goal follows by \propref{subty/sound}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{PUSH} \, \ottnt{T} \, \ottnt{V} \)] By applying \propref{typing/inv(push)}, we have
    the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{h1}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottnt{V}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{h2}\\
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}} \hyp{h3}
    \end{gather}
    By applying \propref{eval/inv(push)}, we have the following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S_{{\mathrm{1}}}}  \hyp{h3}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***\{xTs \mbox{$\mid$} p\} >>}}\) by \propref{subty/sound}; and then, we can
    derive \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** S1 : \{x:T :. xTs \mbox{$\mid$} p /\mbox{$\backslash{}$} x = V\} >>}}\) as follows.
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}}\)}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***\{xTs \mbox{$\mid$} exists x:T. (p /\mbox{$\backslash{}$} x = V) /\mbox{$\backslash{}$} x = V\} >>}}\) by
        \propref{semty/strengthen(push)}}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** S1 : \{x:T :. xTs \mbox{$\mid$} p /\mbox{$\backslash{}$} x = V\} >>}}\)}
    \end{prooftree}
    Finally, the goal follows by \propref{subty/sound}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{NOT} \)] By applying \propref{typing/inv(not)}, we have the
    following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{h1}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{y} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottsym{(}  \ottmv{x}  \neq  0  \wedge  \ottmv{y}  \ottsym{=}  0  \vee  \ottmv{x}  \ottsym{=}  0  \wedge  \ottmv{y}  \ottsym{=}  1  \ottsym{)}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{h2}
    \end{gather}
    By applying \propref{eval/inv(not)}, we have two cases.
    \begin{match}
    \item[\( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{i}  \triangleright  \ottnt{S} ,  \ottnt{S_{{\mathrm{2}}}} \ottsym{=} 0  \triangleright  \ottnt{S} \), where \(\ottnt{i}  \neq  0\)] We have
      \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= i :.*** S : \{x:int :. xTs \mbox{$\mid$} p\} >>}}\) by \propref{subty/sound}.  Then,
      \(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= i : ***int >>}}\) and \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x = i\} >>}}\)
      by \propref{semty/inv(push)}.  Now we can derive
      \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= 0 :.*** S : \{y:int :. xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} (x <> 0 /\mbox{$\backslash{}$} y = 0 \mbox{$\backslash{}$}/ x
        = 0 /\mbox{$\backslash{}$} y = 1)\} >>}}\) as follows.
      \begin{prooftree}
        \AxiomC{}%
        \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= 0 : ***int >>}}\)}
        \AxiomC{By \propref{semty/strengthen(tf)}}%
        \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists y:int. (exists x:int. p /\mbox{$\backslash{}$} (x <> 0 /\mbox{$\backslash{}$}
            y = 0 \mbox{$\backslash{}$}/ x = 0 /\mbox{$\backslash{}$} y = 1)) /\mbox{$\backslash{}$} y = 0\} >>}}\)}%
        \RightLabel{\ruleref{Sem-Push}}%
        \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= 0 :.*** S : \{y:int :. xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} (x <> 0
            /\mbox{$\backslash{}$} y = 0 \mbox{$\backslash{}$}/ x = 0 /\mbox{$\backslash{}$} y = 1)\} >>}}\)}
      \end{prooftree}
      Finally, the goal follows by \propref{subty/sound}.

    \item[\( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} 0  \triangleright  \ottnt{S} ,  \ottnt{S_{{\mathrm{2}}}} \ottsym{=} 1  \triangleright  \ottnt{S} \)] We have
      \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= 0 :.*** S : \{x:int :. xTs \mbox{$\mid$} p\} >>}}\) by \propref{subty/sound}.  So,
      \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x = 0\} >>}}\) by
      \propref{semty/inv(push)}.  Now we can derive
      \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= 1 :.*** S : \{y:int :. xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} (x <> 0 /\mbox{$\backslash{}$} y = 0 \mbox{$\backslash{}$}/ x
        = 0 /\mbox{$\backslash{}$} y = 1)\} >>}}\) as follows.
      \begin{prooftree}
        \AxiomC{}%
        \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= 1 : ***int >>}}\)}
        \AxiomC{By \propref{semty/strengthen(ft)}}%
        \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists y:int. (exists x:int. p /\mbox{$\backslash{}$} (x <> 0 /\mbox{$\backslash{}$}
            y = 0 \mbox{$\backslash{}$}/ x = 0 /\mbox{$\backslash{}$} y = 1)) /\mbox{$\backslash{}$} y = 1\} >>}}\)}%
        \RightLabel{\ruleref{Sem-Push}}%
        \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= 1 :.*** S : \{y:int :. xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} (x <> 0
            /\mbox{$\backslash{}$} y = 0 \mbox{$\backslash{}$}/ x = 0 /\mbox{$\backslash{}$} y = 1)\} >>}}\)}
      \end{prooftree}
      Finally, the goal follows by \propref{subty/sound}.
    \end{match}

  \item[\( \ottnt{I} \ottsym{=} \ottkw{ADD} \)] By applying \propref{typing/inv(add)}, we have the
    following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright   \ottmv{y} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{h1}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{z} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{y} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{+}  \ottmv{y}  \ottsym{=}  \ottmv{z}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}
      \hyp{h2}
    \end{gather}
    By applying \propref{eval/inv(add)}, we have the following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{i_{{\mathrm{1}}}}  \triangleright  \ottnt{i_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{h1}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{i_{{\mathrm{3}}}}  \triangleright  \ottnt{S}  \hyp{h2}\\
       \ottnt{i_{{\mathrm{1}}}}  \ottsym{+}  \ottnt{i_{{\mathrm{2}}}} \ottsym{=} \ottnt{i_{{\mathrm{3}}}}  \hyp{h3}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= i1 :.*** i2 :. S : \{x:int :. y:int :. xTs \mbox{$\mid$} p\} >>}}\) by
    \propref{subty/sound}.  Then, by applying \propref{semty/inv(push)} twice,
    we have the following hypothesis.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= i1 : ***int >>}} \hyp{h4}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= i2 : ***int >>}} \hyp{h5}\\
      \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists y:int. (exists x:int. p /\mbox{$\backslash{}$} x = i1) /\mbox{$\backslash{}$} y = i2\} >>}}
      \hyp{h6}
    \end{gather}
    Now we can derive
    \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= i3 :.*** S : \{z:int :. xTs \mbox{$\mid$} exists x:int, y:int. p /\mbox{$\backslash{}$} x + y = z\} >>}}\)
    as follows.  \YN{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= i3 : ***int >>}}\) from where?}
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= i3 : ***int >>}}\)}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists z:int. (exists x:int, y:int. p /\mbox{$\backslash{}$} x + y
          = z) /\mbox{$\backslash{}$} z = i3\} >>}}\) by \propref{semty/strengthen(add)}}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= i3 :.*** S : \{z:int :. xTs \mbox{$\mid$} exists x:int, y:int. p /\mbox{$\backslash{}$} x
          + y = z\} >>}}\)}
    \end{prooftree}
    Finally, the goal follows by \propref{subty/sound}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{PAIR} \)] By applying \propref{typing/inv(pair)}, we have the
    following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright   \ottmv{y} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{h1}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{z} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge  \ottsym{(}  \ottmv{x}  \ottsym{,}  \ottmv{y}  \ottsym{)}  \ottsym{=}  \ottmv{z}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}
      \hyp{h2}
    \end{gather}
    By applying \propref{eval/inv(pair)}, we have the following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{h3}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \triangleright  \ottnt{S}  \hyp{h4}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V1 :.*** V2 :. S : \{x:T1 :. y:T2 :. xTs \mbox{$\mid$} p\} >>}}\) by
    \propref{subty/sound}.  Then, by applying \propref{semty/inv(push)} twice,
    we have the following hypothesis.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T1 >>}} \hyp{h5}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T2 >>}} \hyp{h6}\\
      \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists y:T2. (exists x:T1. p /\mbox{$\backslash{}$} x = V1) /\mbox{$\backslash{}$} y = V2\} >>}}
      \hyp{h7}
    \end{gather}
    So, we can also derive
    \(\texttt{\textcolor{red}{<<no parses (char 16): G \mbox{$\mid$}= (V1, V2) :.*** S : \{z:T1*T2 :. xTs \mbox{$\mid$} exists x:T1, y:T2. p /\mbox{$\backslash{}$} (x, y) =
      z\} >>}}\) as follows.
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T1 >>}}\)}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T2 >>}}\)}%
%      \RightLabel{\ruleref{RTV-Pair}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 14): \mbox{$\mid$}= (V1, V2) : ***T1 * T2 >>}}\)}%
      \AxiomC{By applying \propref{semty/strengthen(pair)} to \hypref{h7}}%
      \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists z:T1*T2. (exists x:T1, y:T2. p /\mbox{$\backslash{}$} (x,
          y) = z) /\mbox{$\backslash{}$} z = (V1, V2)\} >>}}\)}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 16): G \mbox{$\mid$}= (V1, V2) :.*** S : \{z:T1*T2 :. xTs \mbox{$\mid$} exists x:T1,
          y:T2. p /\mbox{$\backslash{}$} (x, y) = z\} >>}}\)}
    \end{prooftree}
    Finally the goal follows by \propref{subty/sound}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{CAR} \)] By applying \propref{typing/inv(car)} on \hypref{type},
    we have the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{1}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}
      \hyp{2}
    \end{gather}
    By applying \propref{eval/inv(car)} on \hypref{eval}, we have the following
    hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \triangleright  \ottnt{S}  \hyp{3}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{S}  \hyp{4}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 16): G \mbox{$\mid$}= (V1, V2) :.*** S : \{x:T1*T2 :. xTs \mbox{$\mid$} p\} >>}}\) by
    \propref{subty/sound}, \hypref{1}, \hypref{3}, \hypref{semty}.  Then, by
    \propref{semty/inv(push)} and \propref{vtyping/inv(pair)}, we have the
    following hypothesis.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T1 >>}} \hyp{5}\\
      \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T1*T2. p /\mbox{$\backslash{}$} x = (V1, V2)\} >>}} \hyp{6}
    \end{gather}
    Now we can have the following derivation.
    \begin{prooftree}
      \AxiomC{\hypref{5}}%
      \AxiomC{By applying \propref{semty/strengthen(car)} to \hypref{6}}%
      \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x1:T1. (exists x:T1*T2, x2:T2. p /\mbox{$\backslash{}$} x =
          (x1, x2)) /\mbox{$\backslash{}$} x1 = V1\} >>}}\)}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V1 :.*** S : \{x1:T1 :. xTs \mbox{$\mid$} exists x:T1*T2, x2:T2. p /\mbox{$\backslash{}$}
          x = (x1, x2)\} >>}}\)}%
    \end{prooftree}
    Then the goal follows by the conclusion above and \propref{subty/sound},
    \hypref{2}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{CDR} \)] By applying \propref{typing/inv(cdr)} on \hypref{type},
    we have the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{1}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{(}  \ottmv{x_{{\mathrm{1}}}}  \ottsym{,}  \ottmv{x_{{\mathrm{2}}}}  \ottsym{)}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}}
      \hyp{2}
    \end{gather}
    By applying \propref{eval/inv(cdr)} on \hypref{eval}, we have the following
    hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \triangleright  \ottnt{S}  \hyp{3}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{4}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 16): G \mbox{$\mid$}= (V1, V2) :.*** S : \{x:T1*T2 :. xTs \mbox{$\mid$} p\} >>}}\) by
    \propref{subty/sound}, \hypref{semty}, \hypref{1}, \hypref{3}.  Then, by
    \propref{semty/inv(push)} and \propref{vtyping/inv(pair)}, we have the
    following hypothesis.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T2 >>}} \hyp{5}\\
      \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T1*T2. p /\mbox{$\backslash{}$} x = (V1, V2)\} >>}} \hyp{6}
    \end{gather}
    Now we can have the following derivation.
    \begin{prooftree}
      \AxiomC{\hypref{5}}%
      \AxiomC{By applying \propref{semty/strengthen(cdr)} to \hypref{6}}%
      \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x2:T2. (exists x:T1*T2, x1:T1. p /\mbox{$\backslash{}$} x =
          (x1, x2)) /\mbox{$\backslash{}$} x2 = V2\} >>}}\)}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V2 :.*** S : \{x2:T2 :. xTs \mbox{$\mid$} exists x:T1*T2, x1:T1. p /\mbox{$\backslash{}$}
          x = (x1, x2)\} >>}}\)}
    \end{prooftree}
    Finally, the goal follows by the conclusion above and \propref{subty/sound},
    \hypref{2}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{NIL} \, \ottnt{T} \)] By applying \propref{typing/inv(nil)} on
    \hypref{type}, we have the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{1}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{2}
    \end{gather}
    By applying \propref{eval/inv(nil)} on \hypref{eval}, we haec the following
    hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottsym{[}  \ottsym{]}  \triangleright  \ottnt{S_{{\mathrm{1}}}}  \hyp{3}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***\{xTs \mbox{$\mid$} p\} >>}}\) by \propref{subty/sound}, \hypref{semty},
    \hypref{1}.  \(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= [] : ***T list >>}}\) by \ruleref{RTV-Nil}.  Then, we can have
    the following derivation.
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= [] : ***T list >>}}\)}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***\{xTs \mbox{$\mid$} exists x:T list. (p /\mbox{$\backslash{}$} x = []) /\mbox{$\backslash{}$} x = []\} >>}}\)
        by \propref{semty/strengthen(push)}}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= [] :.*** S1 : \{x:T list :. xTs \mbox{$\mid$} p /\mbox{$\backslash{}$} x = []\} >>}}\)}
    \end{prooftree}
    Finally, the goal follows by the conclusion above, \propref{subty/sound},
    and \hypref{2}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{CONS} \)] By applying \propref{typing/inv(cons)} to
    \hypref{type}, we have the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \triangleright   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{1}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x_{{\mathrm{3}}}}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{2}
    \end{gather}
    By applying \propref{eval/inv(cons)} to \hypref{eval}, we have the following
    hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{4}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{5}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V1 :.*** V2 :. S : \{x1:T :. x2:T list :. xTs \mbox{$\mid$} p\} >>}}\) by
    \propref{subty/sound}, \hypref{semty}, \hypref{1}, \hypref{4}.  Then,
    applying \propref{semty/inv(push)} twice, we have the following hypothesis.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T >>}} \hyp{6}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T list >>}} \hyp{7}\\
      \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x2:T list. (exists x1:T. p /\mbox{$\backslash{}$} x1 = V1) /\mbox{$\backslash{}$} x2 =
        V2\} >>}} \hyp{8}
    \end{gather}
    Now we can have the following derivation.
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T >>}}\) by \hypref{6}}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T list >>}}\) by \hypref{7}}%
      \RightLabel{\ruleref{RTV-Cons}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 12): \mbox{$\mid$}= V1::V2 : ***T list >>}}\)}%
    \end{prooftree}
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 12): \mbox{$\mid$}= V1::V2 : ***T list >>}}\)}%
      \AxiomC{By applying
        \propref{semty/strengthen(cons)} to \hypref{8}}%
      \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x3:T list. (exists x1:T, x2:T list. p
          /\mbox{$\backslash{}$} x1 :: x2 = x3) /\mbox{$\backslash{}$} x3 = V1::V2\} >>}}\)}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 14): G \mbox{$\mid$}= V1::V2 :.*** S : \{xTs \mbox{$\mid$} exists x1:T, x2:T list. p /\mbox{$\backslash{}$} x1
          :: x2 = x3\} >>}}\)}
    \end{prooftree}
    Finally, the goal follows by the conclusion above, \propref{subty/sound},
    and \hypref{2}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{IF} \, \mathit{IS}_{{\mathrm{1}}} \, \mathit{IS}_{{\mathrm{2}}} \)] By applying \propref{typing/inv(if)}, we have
    the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{h1}\\
      \texttt{\textcolor{red}{<<no parses (char 6): G \mbox{$\mid$}= \{***xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x <> 0\} IS1 P2 >>}} \hyp{h2}\\
      \texttt{\textcolor{red}{<<no parses (char 6): G \mbox{$\mid$}= \{***xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x = 0\} IS2 P2 >>}} \hyp{h3}
    \end{gather}
    By applying \propref{eval/inv(if)}, we have two cases.
    \begin{match}
    \item[\( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{i}  \triangleright  \ottnt{S} , \ottnt{S}  \vdash  \mathit{IS}_{{\mathrm{1}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\), where \(\ottnt{i}  \neq  0\)] We have
      \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= i :.*** S : \{x:int :. xTs \mbox{$\mid$} p\} >>}}\) by \propref{subty/sound}.  So, by
      applying \propref{semty/inv(push)}, we have the following hypothesis.
      \begin{gather}
        \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= i : ***int >>}} \hyp{h4}\\
        \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x = i\} >>}} \hyp{h5}
      \end{gather}
      Now we have \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x <> 0\} >>}}\) by
      \propref{semty/strengthen(ift)}; and so, the goal follows by IH.

    \item[\( \ottnt{S_{{\mathrm{1}}}} \ottsym{=} 0  \triangleright  \ottnt{S} , \ottnt{S}  \vdash  \mathit{IS}_{{\mathrm{2}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}\)] We have
      \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= 0 :.*** S : \{x:int :. xTs \mbox{$\mid$} p\} >>}}\) by \propref{subty/sound}.  So,
      applying \propref{semty/inv(push)}, we have the following hypothesis.
      \begin{gather}
        \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x = 0\} >>}} \hyp{h6}
      \end{gather}
      Now the goal follows by the IH.
    \end{match}
    
  \item[\( \ottnt{I} \ottsym{=} \ottkw{LOOP} \, \mathit{IS} \)] By applying \propref{typing/inv(loop)}, we have the
    following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{h1}\\
      \Gamma  \vdash  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  0  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{h2}\\
       \Gamma \vdash \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottkw{int}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \neq  0  \ottsym{\}} \; \mathit{IS} \; \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottkw{int}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}}  \hyp{h3}
    \end{gather}
    We have the following induction hypothesis.
    \begin{gather}
      \text{For any } S1, S2 \text{ if } \ottnt{S_{{\mathrm{1}}}}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \text{ and } \texttt{\textcolor{red}{<<no parses (char 16): G \mbox{$\mid$}=
      S1 : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x <> 0\} >>}} \text{ then } \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***\{x:int
        :. xTs \mbox{$\mid$} p\} >>}}. \hyp{OIH}
    \end{gather}
    We also have \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***\{x:int :. xTs \mbox{$\mid$} p\} >>}}\) by \propref{subty/sound}.
    So, we can use \propref{typing/sound/loop}; and we have
    \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***\{xTs \mbox{$\mid$} exists x:int. p /\mbox{$\backslash{}$} x = 0\} >>}}\).  The goal follows by
    \propref{subty/sound}.

  \item[\( \ottnt{I} \ottsym{=} \texttt{IF\symbol{95}CONS} \, \mathit{IS}_{{\mathrm{1}}} \, \mathit{IS}_{{\mathrm{2}}} \)] Applying \propref{typing/inv(ifcons)}, we
    have the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{h1}\\
       \Gamma \vdash \ottsym{\{}   \ottmv{y} \mathord:\allowbreak \ottnt{T}   \triangleright   \ottmv{z} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{y}  ::  \ottmv{z}  \ottsym{=}  \ottmv{x}  \ottsym{\}} \; \mathit{IS}_{{\mathrm{1}}} \; \Phi_{{\mathrm{2}}}  \hyp{h2}\\
       \Gamma \vdash \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  \ottsym{\}} \; \mathit{IS}_{{\mathrm{2}}} \; \Phi_{{\mathrm{2}}}  \hyp{h3}
    \end{gather}
    Applying \propref{eval/inv(ifcons)}, we have two cases.
    \begin{match}
    \item
      \begin{gather}
         \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{h4}\\
        \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \vdash  \mathit{IS}_{{\mathrm{1}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{h5}
      \end{gather}
      We have \(\texttt{\textcolor{red}{<<no parses (char 16): G \mbox{$\mid$}= V1 :: V2 :.*** S : \{x:T list :. xTs \mbox{$\mid$} p\} >>}}\) by
      \propref{subty/sound}.  Then, applying \propref{semty/inv(push)} and
      \propref{vtyping/inv(cons)}, we have the following hypothesis.
      \begin{gather}
        \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T >>}} \hyp{h6}\\
        \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T list >>}} \hyp{h7}\\
        \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T list. p /\mbox{$\backslash{}$} x = V1 :: V2\} >>}} \hyp{h8}
      \end{gather}
      \begin{prooftree}
        \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T list >>}}\)}%
        \AxiomC{By applying
          \propref{semty/strengthen(ifconst)} to \hypref{h8}}%
        \UnaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists z:T list. (exists y:T. (exists x:T
            list. p /\mbox{$\backslash{}$} y :: z = x) /\mbox{$\backslash{}$} y = V1) /\mbox{$\backslash{}$} z = V2\} >>}}\)}%
        \RightLabel{\ruleref{Sem-Push}}%
        \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V2 :.*** S : \{z:T list :. xTs \mbox{$\mid$} exists y:T. (exists
            x:T list. p /\mbox{$\backslash{}$} y :: z = x) /\mbox{$\backslash{}$} y = V1\} >>}} \quad (\ast)\)}%
      \end{prooftree}
      \begin{prooftree}
        \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T >>}}\)}%
        \AxiomC{\((\ast)\)}%
        \RightLabel{\ruleref{Sem-Push}}%
        \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V1 :.*** V2 :. S : \{y:T :. z:T list :. xTs \mbox{$\mid$} exists
            x:T list. p /\mbox{$\backslash{}$} y :: z = x\} >>}}\)}%
      \end{prooftree}
      Now the goal follows by IH.

    \item
      \begin{gather}
         \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{[}  \ottsym{]}  \triangleright  \ottnt{S}  \hyp{h9}\\
        \ottnt{S}  \vdash  \mathit{IS}_{{\mathrm{2}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{h10}
      \end{gather}
      We have \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= [] :.*** S : \{x:T list :. xTs \mbox{$\mid$} p\} >>}}\) by
      \propref{subty/sound}.  Then, applying \propref{semty/inv(push)}, we have
      \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x:T list. p /\mbox{$\backslash{}$} x = []\} >>}}\).  Now the goal
      follows by IH.
    \end{match}

  \item[\( \ottnt{I} \ottsym{=} \ottkw{ITER} \, \mathit{IS} \)] We have the following induction hypothesis.
    \begin{gather}
      \text{For any } \Gamma, \Phi_{{\mathrm{1}}}, \Phi_{{\mathrm{2}}}, \ottnt{S_{{\mathrm{1}}}}, \ottnt{S_{{\mathrm{2}}}}, \text{ if }  \Gamma \vdash \Phi_{{\mathrm{1}}} \; \mathit{IS} \; \Phi_{{\mathrm{2}}} , \ottnt{S_{{\mathrm{1}}}}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}}, \text{ and } \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***P1 >>}}, \text{ then
      } \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***P2 >>}}. \hyp{OIH}
    \end{gather}
    By applying \propref{typing/inv(iter)}, we have the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{h1}\\
      \Gamma  \vdash  \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x}  \ottsym{=}  \ottsym{[}  \ottsym{]}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{h2}\\
       \Gamma  \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}  \vdash \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{1}}}}  ::  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{\}} \; \mathit{IS} \; \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{2}}}}  \ottsym{=}  \ottmv{x}  \ottsym{\}}  \hyp{h3}
    \end{gather}
    So, \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}    \vdash   \varphi  : \mathord{*} \) by applying \propref{subty/wf} to
    \hypref{h1}; and then \(  \text{fvars}( \varphi )   \subseteq   \text{dom}( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}  )  \) by
    \propref{ttyping/strut(fclosed)}.  Since, w.l.o.g., we can assume
    \( \ottmv{x_{{\mathrm{2}}}}  \notin   \text{dom}( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T} \, \ottkw{list}  )  \), we know
    \begin{gather}
       \ottmv{x_{{\mathrm{2}}}}  \notin   \text{fvars}( \varphi )  . \hyp{4}
    \end{gather}
    We also have the following hypothesis by \propref{subty/sound},
    \hypref{semty}, \hypref{h1}.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***\{x:T list :. xTs \mbox{$\mid$} p\} >>}} \hyp{5}
    \end{gather}
    Now applying \propref{typing/sound/iter} to \hypref{eval}, \hypref{OIH},
    \hypref{h3}, \hypref{4}, \hypref{5}, we have
    \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S2 : ***\{xTs \mbox{$\mid$} exists x:T list. p /\mbox{$\backslash{}$} x = []\} >>}}\).  Then, the goal
    follows by \propref{subty/sound}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{LAMBDA} \, \ottnt{T_{{\mathrm{1}}}} \, \ottnt{T_{{\mathrm{2}}}} \, \mathit{IS} \)] By applying \propref{typing/inv(lambda)} to
    \hypref{type}, we have the following hypothesis.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 10): \mbox{$\mid$}= <IS> : ***T1->T2 >>}} \hyp{0}\\
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{1}\\
        \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}    \vdash   \varphi_{{\mathrm{1}}}  : \mathord{*}  \hyp{1.1}\\
      \texttt{\textcolor{red}{<<no parses (char 11): y1':T1 \mbox{$\mid$}= \{***y1:T1 :. \_ \mbox{$\mid$} y1' = y1 /\mbox{$\backslash{}$} p1\} IS \{y2:T2 :. \_ \mbox{$\mid$} p2\} >>}} \hyp{2}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \varphi  \wedge  \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} ( \ottmv{x} ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}  \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{3}
    \end{gather}
    By applying \propref{eval/inv(lambda)} to \hypref{eval}, we have the
    following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=}  \langle  \mathit{IS}  \rangle   \triangleright  \ottnt{S_{{\mathrm{1}}}}  \hyp{4}
    \end{gather}
    So, applying \propref{subty/sound}, \hypref{semty}, \hypref{1}, we have
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***\{xTs \mbox{$\mid$} p\} >>}}. \hyp{7}
    \end{gather}
    From the above, we have the following hypothesis by \propref{semty/wf}.
    \begin{gather}
       \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \varphi  : \mathord{*}  \hyp{7.1}
    \end{gather}
    We can derive \(  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}    \vdash   \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  : \mathord{*} \) by using
    \hypref{1.1}.  So, we have the following hypothesis by \propref{typing/wf},
    \hypref{2}.
    \begin{gather}
        \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \varphi_{{\mathrm{2}}}  : \mathord{*}  \hyp{7.2}
    \end{gather}
    Now, we know
    \(\texttt{\textcolor{red}{<<no parses (char 7): fv(p) /***\mbox{$\backslash{}$} fv(p1) /\mbox{$\backslash{}$} fv(p2) sub dom(G, rev(xTs)) /\mbox{$\backslash{}$} \{y1', y1, y2\} >>}}\) by
    \propref{ttyping/strut(fclosed)}, \hypref{1.1}, \hypref{7.1}, \hypref{7.2}.  Since, we
    can assume \(\texttt{\textcolor{red}{<<no parses (char 24): x nin dom(G, rev(xTs)) /***\mbox{$\backslash{}$} \{y1', y1, y2\} >>}}\), w.l.o.g, we can
    have the following assumption.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 13): x nin fv(p) /***\mbox{$\backslash{}$} fv(p1) /\mbox{$\backslash{}$} fv(p2) >>}} \hyp{A1}
    \end{gather}
    We have the following hypothesis by applying \propref{subty/wf} to
    \hypref{3}.
    \begin{gather}
       \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}    \vdash   \varphi  \wedge  \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} ( \ottmv{x} ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}  : \mathord{*}  \hyp{10}
    \end{gather}
    Then, applying \propref{ftyping/inv(and)} to \hypref{10}, we have the following
    hypothesis.
    \begin{gather}
       \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}    \vdash   \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} ( \ottmv{x} ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}  : \mathord{*}  \hyp{wfp2}
    \end{gather}
    Under the assumption \hypref{A1},
    \(\texttt{\textcolor{red}{<<no parses (char 78): (forall y1':T1, y1:T1, y2:T2. y1' = y1 /\mbox{$\backslash{}$} p1 /\mbox{$\backslash{}$} call(x, y1') = y2 ==>
    p2).***\{<IS>/x\} >>}}\) equals to
    \(\forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} (  \langle  \mathit{IS}  \rangle  ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}\).  So, by \propref{ttyping/strut(fsubst)}, \hypref{0}, \hypref{wfp2}, we have
    the following hypothesis.
    \begin{gather}
       \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} (  \langle  \mathit{IS}  \rangle  ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}  : \mathord{*}  \hyp{wfp2'}
    \end{gather}
    We have the following hypothesis by applying IH to
    \hypref{2}.
    \begin{multline}
      \text{For any } \ottnt{V_{{\mathrm{1}}}}, \ottnt{V_{{\mathrm{2}}}} \text{ if } \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Downarrow  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ddagger
      \text{ and } \texttt{\textcolor{red}{<<no parses (char 15): y1':T1 \mbox{$\mid$}= V1 :.*** \_ : \{y1:T1 :. \_ \mbox{$\mid$} y1' = y1 /\mbox{$\backslash{}$} p1\} >>}},\\ \text{
        then } \texttt{\textcolor{red}{<<no parses (char 15): y1':T1 \mbox{$\mid$}= V2 :.*** \_ : \{y2:T2 :. \_ \mbox{$\mid$} p2\} >>}} \hyp{5}
    \end{multline}
    So, applying \propref{fol/thm/lambda} to \hypref{5}, and then
    \propref{fol/thm/valid} with \hypref{wfp2'}, we have
    \begin{gather}
      \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \models  \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} (  \langle  \mathit{IS}  \rangle  ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}. \hyp{6}
    \end{gather}
    Now, we have
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***\{xTs \mbox{$\mid$} p /\mbox{$\backslash{}$} forall y1':T1, y1:T1, y2:T2. y1' = y1 /\mbox{$\backslash{}$} p1 /\mbox{$\backslash{}$}
        call(<IS>, y1') = y2 ==> p2\} >>}} \hyp{8}
    \end{gather}
    by \propref{semty/append/thm}, \hypref{7}, \hypref{6}.  Under the assumption
    \hypref{A1},
    \(\varphi  \wedge  \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} (  \langle  \mathit{IS}  \rangle  ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}\) equals to
    \(\texttt{\textcolor{red}{<<no parses (char 83): (p /\mbox{$\backslash{}$} forall y1':T1, y1:T1, y2:T2. y1' = y1 /\mbox{$\backslash{}$} p1 /\mbox{$\backslash{}$} call(x, y1') = y2
    ==> p2).***\{<IS>/x\} >>}}\).  So, applying \propref{subty/subst=>exists} to
    \hypref{0}, \hypref{10}, we have
    \begin{gather}
      \begin{aligned}
        &\Gamma  \vdash  \ottsym{\{}  \Upsilon  \mid  \varphi  \wedge  \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} (  \langle  \mathit{IS}  \rangle  ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}  \ottsym{\}}\\
        \ottsym{<:}\;& \ottsym{\{}  \Upsilon  \mid  \exists \,  \ottmv{x} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottsym{(}  \varphi  \wedge  \forall \,  \ottmv{y'_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{y_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottmv{y'_{{\mathrm{1}}}}  \ottsym{=}  \ottmv{y_{{\mathrm{1}}}}  \wedge  \varphi_{{\mathrm{1}}}  \wedge   \ottkw{call} ( \ottmv{x} ,  \ottmv{y'_{{\mathrm{1}}}} ) =  \ottmv{y_{{\mathrm{2}}}}   \implies  \varphi_{{\mathrm{2}}}  \ottsym{)}  \wedge  \ottmv{x}  \ottsym{=}   \langle  \mathit{IS}  \rangle   \ottsym{\}}.
      \end{aligned}
      \hyp{10}
    \end{gather}
    Applying \propref{subty/sound} to \hypref{8}, \hypref{10}, we have
    \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= S1 : ***\{xTs \mbox{$\mid$} exists x:T1->T2. (p /\mbox{$\backslash{}$} forall y1':T1, y1:T1, y2:T2. y1'
      = y1 /\mbox{$\backslash{}$} p1 /\mbox{$\backslash{}$} call(x, y1') = y2 ==> p2) /\mbox{$\backslash{}$} x = <IS>\} >>}}\), from which we
    can derive
    \(\texttt{\textcolor{red}{<<no parses (char 12): G \mbox{$\mid$}= <IS> :.*** S1 : \{x:T1->T2 :. xTs \mbox{$\mid$} p /\mbox{$\backslash{}$} forall y1':T1, y1:T1,
      y2:T2. y1' = y1 /\mbox{$\backslash{}$} p1 /\mbox{$\backslash{}$} call(x, y1') = y2 ==> p2\} >>}}\) by \hypref{0} and
    \ruleref{Sem-Push}.
    Finally, the goal follows by the conclusion above, \propref{subty/sound},
    and \hypref{3}.

  \item[\( \ottnt{I} \ottsym{=} \ottkw{EXEC} \)] By applying \propref{typing/inv(exec)} to
    \hypref{type}, we have the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \triangleright   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{1}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge   \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottmv{x_{{\mathrm{3}}}}   \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{2}
    \end{gather}
    By applying \propref{eval/inv(exec)} to \hypref{eval}, we have the following
    hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright   \langle  \mathit{IS}  \rangle   \triangleright  \ottnt{S}  \hyp{3}\\
      \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Downarrow  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ddagger \hyp{4}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{5}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V1 :.*** <IS> :. S : \{x1:T1 :. x2:T1->T2 :. xTs \mbox{$\mid$} p\} >>}}\) by
    \propref{subty/sound}, \hypref{semty}, \hypref{1}, \hypref{3}.  Then,
    applying \propref{semty/inv(push)} twice, we have the following hypothesis.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T1 >>}} \hyp{5}\\
      \texttt{\textcolor{red}{<<no parses (char 10): \mbox{$\mid$}= <IS> : ***T1->T2 >>}} \hyp{6}\\
      \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x2:T1->T2. (exists x1:T1. p /\mbox{$\backslash{}$} x1 = V1) /\mbox{$\backslash{}$} x2 =
        <IS>\} >>}} \hyp{7}
    \end{gather}
    Applying \propref{vtyping/inv(fun)} to \hypref{6}, we have
    \(\ottnt{T_{{\mathrm{1}}}}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Rightarrow  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \ddagger\).  So, by \propref{styping/sound}, \hypref{4},
    \hypref{5}, we have
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T2 >>}}. \hyp{10}
    \end{gather}
    Applying \propref{semty/exists=>subst} to \hypref{7} twice, we have
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} p.\{<IS>/x2\}.\{V1/x1\}\} >>}}. \hyp{7'}
    \end{gather}
    Applying \propref{subty/wf} to \hypref{2}, we have
    \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge   \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottmv{x_{{\mathrm{3}}}}   : \mathord{*} \).  So, by \propref{ftyping/inv(exists)}, \propref{ftyping/inv(and)}, we
    have \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}    \vdash    \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottmv{x_{{\mathrm{3}}}}   : \mathord{*} \).
    Furthermore, by \propref{ttyping/strut(fsubst)}, \hypref{5}, \hypref{6},
    \hypref{10}, we have \( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash    \ottkw{call} (  \langle  \mathit{IS}  \rangle  ,  \ottnt{V_{{\mathrm{1}}}} ) =  \ottnt{V_{{\mathrm{2}}}}   : \mathord{*} \).  Then,
    applying \propref{fol/thm/exec} to \hypref{4} and by
    \propref{fol/thm/valid}, we have
    \begin{gather}
      \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \models   \ottkw{call} (  \langle  \mathit{IS}  \rangle  ,  \ottnt{V_{{\mathrm{1}}}} ) =  \ottnt{V_{{\mathrm{2}}}} . \hyp{8}
    \end{gather}
    Applying \propref{semty/append/thm} to \hypref{7'}, \hypref{8}, we have
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} (p /\mbox{$\backslash{}$} call(x2, x1) = V2).\{<IS>/x2\}.\{V1/x1\}\} >>}}. \hyp{9}
    \end{gather}
    We have the following hypothesis by \propref{fol/thm/subst=>exists},
    \propref{fol/thm/misc(drop1)}, \propref{fol/thm/misc(existsswap)}.
    \begin{itemize}
      \setlength{\leftmargin}{0pt}
      \setlength{\labelsep}{0.5em}
      \setlength{\itemsep}{0pt}
    \item
      \(\texttt{\textcolor{red}{<<no parses (char 28): \mbox{$\mid$}= (p /\mbox{$\backslash{}$} call(x2, x1) = V2).***\{<IS>/x2\}.\{V1/x1\} ==> exists x1:T1. (p /\mbox{$\backslash{}$}
      call(x2, x1) = V2).\{<IS>/x2\} /\mbox{$\backslash{}$} x1 = V1 >>}}\)
    \item
      \(\texttt{\textcolor{red}{<<no parses (char 43): \mbox{$\mid$}= (exists x1:T1. (p /\mbox{$\backslash{}$} call(x2, x1) = V2).***\{<IS>/x2\} /\mbox{$\backslash{}$} x1 = V1) ==>
      exists x1:T1. (p /\mbox{$\backslash{}$} call(x2, x1) = V2).\{<IS>/x2\} >>}}\)
    \item
      \(\texttt{\textcolor{red}{<<no parses (char 42): \mbox{$\mid$}= (exists x1:T1. p /\mbox{$\backslash{}$} call(x2, x1) = V2).***\{<IS>/x2\} ==> exists
      x2:T1->T2. (exists x1:T1. p /\mbox{$\backslash{}$} call(x2, x1) = V2) /\mbox{$\backslash{}$} x2 = <IS> >>}}\)
    \item
      \(\texttt{\textcolor{red}{<<no parses (char 141): \mbox{$\mid$}= (exists x2:T1->T2. (exists x1:T1. p /\mbox{$\backslash{}$} call(x2, x1) = V2) /\mbox{$\backslash{}$} x2 =
      <IS>) ==> exists x2:T1->T2. (exists x1:T1. p /\mbox{$\backslash{}$} call(x2, x1) = V2)*** >>}}\)
    \item
      \(\texttt{\textcolor{red}{<<no parses (char 117): \mbox{$\mid$}= exists x2:T1->T2. (exists x1:T1. p /\mbox{$\backslash{}$} call(x2, x1) = V2) ==> exists
      x1:T1, x2:T1->T2. p /\mbox{$\backslash{}$} call(x2, x1) = V2*** >>}}\)
    \item
      \(\texttt{\textcolor{red}{<<no parses (char 53): \mbox{$\mid$}= (exists x1:T1, x2:T1->T2. p /\mbox{$\backslash{}$} call(x2, x1) = x3).***\{V2/x3\} ==>
      exists x3:T2. (exists x1:T1, x2:T1->T2. p /\mbox{$\backslash{}$} call(x2, x1) = x3) /\mbox{$\backslash{}$} x3 =
      V2 >>}}\)
    \end{itemize}
    We can assume \(\ottmv{x_{{\mathrm{1}}}}  \neq  \ottmv{x_{{\mathrm{2}}}}\) and
    \( \ottmv{x_{{\mathrm{3}}}}  \notin   \text{dom}( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}  )  \), w.l.o.g.  Since, we know
    \(  \text{fvars}( \varphi )   \subseteq   \text{dom}( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}  )  \) by
    \propref{ttyping/strut(fclosed)}, \propref{subty/wf}, \hypref{1},
    \( \ottmv{x_{{\mathrm{3}}}}  \notin   \text{fvars}( \varphi )  \).  Now we know that
    \(\texttt{\textcolor{red}{<<no parses (char 39): exists x1:T1. (p /\mbox{$\backslash{}$} call(x2, x1) = V2).***\{<IS>/x2\} >>}}\) equals to
    \(\texttt{\textcolor{red}{<<no parses (char 39): (exists x1:T1. p /\mbox{$\backslash{}$} call(x2, x1) = V2).***\{<IS>/x2\} >>}}\) and
    \(\exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge   \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottnt{V_{{\mathrm{2}}}} \) equals to
    \(\texttt{\textcolor{red}{<<no parses (char 50): (exists x1:T1, x2:T1->T2. p /\mbox{$\backslash{}$} call(x2, x1) = x3).***\{V2/x3\} >>}}\).
    Consequently, we have
    \begin{multline}
       \models  \texttt{\textcolor{red}{<<no parses (char 25): (p /\mbox{$\backslash{}$} call(x2, x1) = V2).***\{<IS>/x2\}.\{V1/x1\} >>}}  \implies  \\ \exists \,  \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge   \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottmv{x_{{\mathrm{3}}}}   \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{3}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}} \hyp{imply}
    \end{multline}
    We have the following derivations.
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 40): G, rev(xTs) \mbox{$\mid$}- (p /\mbox{$\backslash{}$} call(x2, x1) = V2).***\{<IS>/x2\}.\{V1/x1\} :
        * >>}}\) by \propref{semty/wf}, \hypref{9}}%
    \end{prooftree}
    \begin{prooftree}
      \AxiomC{By applying \propref{subty/wf} to \hypref{2}}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge   \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottmv{x_{{\mathrm{3}}}}   : \mathord{*} \)}%
      \AxiomC{(By routine using \hypref{10})}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \ottmv{x_{{\mathrm{3}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  : \mathord{*} \)}%
      \BinaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon }   \ottsym{,}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}    \vdash   \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge   \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottmv{x_{{\mathrm{3}}}}   \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{3}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  : \mathord{*} \)}%
      \UnaryInfC{\( \Gamma  \ottsym{,}   \widehat{ \Upsilon }    \vdash   \exists \,  \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \ottsym{(}  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}   \ottsym{.}  \varphi  \wedge   \ottkw{call} ( \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{1}}}} ) =  \ottmv{x_{{\mathrm{3}}}}   \ottsym{)}  \wedge  \ottmv{x_{{\mathrm{3}}}}  \ottsym{=}  \ottnt{V_{{\mathrm{2}}}}  : \mathord{*} \)}%
    \end{prooftree}
    So,
    \(\texttt{\textcolor{red}{<<no parses (char 40): G, rev(xTs) \mbox{$\mid$}- (p /\mbox{$\backslash{}$} call(x2, x1) = V2).***\{<IS>/x2\}.\{V1/x1\} ==> exists
    x3:T2. (exists x1:T1, x2:T1->T2. p /\mbox{$\backslash{}$} call(x2, x1) = x3) /\mbox{$\backslash{}$} x3 = V2 : * >>}}\)
    by \ruleref{WF-Imply}.  Then,
    \(\texttt{\textcolor{red}{<<no parses (char 37): G \mbox{$\mid$}- \{xTs \mbox{$\mid$} (p /\mbox{$\backslash{}$} call(x2, x1) = V2).***\{<IS>/x2\}.\{V1/x1\}\} <: \{xTs \mbox{$\mid$} exists
      x3:T2. (exists x1:T1, x2:T1->T2. p /\mbox{$\backslash{}$} call(x2, x1) = x3) /\mbox{$\backslash{}$} x3 = V2\} >>}}\)
    follows by \propref{def/subty}, \propref{fol/thm/valid}, \hypref{imply}.
    Now we have
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x3:T2. (exists x1:T1, x2:T1->T2. p /\mbox{$\backslash{}$} call(x2,
      x1) = x3) /\mbox{$\backslash{}$} x3 = V2\} >>}}\) by \propref{subty/sound}, \hypref{9}.
    Therefore, we can have the following derivation.
    \begin{prooftree}
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T2 >>}}\)}%
      \AxiomC{\(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x3:T2. (exists x1:T1, x2:T1->T2. p /\mbox{$\backslash{}$}
          call(x2, x1) = x3) /\mbox{$\backslash{}$} x3 = V2\} >>}}\)}%
      \RightLabel{\ruleref{Sem-Push}}%
      \BinaryInfC{\(\texttt{\textcolor{red}{<<no parses (char 10): G \mbox{$\mid$}= V2 :.*** S : \{x3:T2 :. xTs \mbox{$\mid$} exists x1:T1, x2:T1->T2. p
          /\mbox{$\backslash{}$} call(x2, x1) = x3\} >>}}\)}
    \end{prooftree}
    Finally, the goal follows by the conclusion above, \propref{subty/sound},
    \hypref{2}.

  \item[\( \ottnt{I} \ottsym{=} \texttt{TRANSFER\symbol{95}TOKENS} \, \ottnt{T} \)] Applying
    \propref{typing/inv(transfertokens)}, we have the following hypothesis.
    \begin{gather}
      \Gamma  \vdash  \Phi_{{\mathrm{1}}}  \ottsym{<:}  \ottsym{\{}   \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \triangleright   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \triangleright   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{address}   \triangleright  \Upsilon  \mid  \varphi  \ottsym{\}} \hyp{1}\\
      \Gamma  \vdash  \ottsym{\{}   \ottmv{x_{{\mathrm{4}}}} \mathord:\allowbreak \ottkw{operation}   \triangleright  \Upsilon  \mid  \exists \,  \ottmv{x_{{\mathrm{1}}}} \mathord:\allowbreak \ottnt{T}   \ottsym{,}   \ottmv{x_{{\mathrm{2}}}} \mathord:\allowbreak \ottkw{int}   \ottsym{,}   \ottmv{x_{{\mathrm{3}}}} \mathord:\allowbreak \ottkw{address}   \ottsym{.}  \varphi  \wedge  \ottmv{x_{{\mathrm{4}}}}  \ottsym{=}   \texttt{Transfer}  (  \ottmv{x_{{\mathrm{1}}}} ,  \ottmv{x_{{\mathrm{2}}}} ,  \ottmv{x_{{\mathrm{3}}}}  )   \ottsym{\}}  \ottsym{<:}  \Phi_{{\mathrm{2}}} \hyp{2}
    \end{gather}
    Applying \propref{eval/inv(transfertokens)}, we have the following
    hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{i}  \triangleright  \ottnt{a}  \triangleright  \ottnt{S}  \hyp{3}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=}  \texttt{Transfer}  (  \ottnt{V} ,  \ottnt{i} ,  \ottnt{a}  )   \triangleright  \ottnt{S}  \hyp{4}
    \end{gather}
    So, \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= V :.*** i :. a :. S : \{x1:T :. x2:int :. x3:address :. xTs \mbox{$\mid$}
      p\} >>}}\) by \propref{subty/sound}, \hypref{semty}, \hypref{1}, \hypref{3}.
    Then, applying \propref{semty/inv} three times, we have the following
    hypothesis.
    \begin{gather}
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}} \hyp{5}\\
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= i : ***int >>}} \hyp{6}\\
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= a : ***address >>}} \hyp{7}\\
      \texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x3:address. (exists x2:int. (exists x1:T. p /\mbox{$\backslash{}$} x1
        = V) /\mbox{$\backslash{}$} x2 = i) /\mbox{$\backslash{}$} x3 = a\} >>}} \hyp{8}
    \end{gather}
    We have \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x1:T, x2:int, x3:address. p\} >>}}\) by
    applying \propref{semty/strengthen(transfertokens)} to \hypref{8}.  We can
    derive \(\texttt{\textcolor{red}{<<no parses (char 26): \mbox{$\mid$}= transaction(V, i, a) : ***operation >>}}\) from \hypref{5},
    \hypref{6}, \hypref{7}.  So,
    \(\texttt{\textcolor{red}{<<no parses (char 9): G \mbox{$\mid$}= S : ***\{xTs \mbox{$\mid$} exists x4:operation. (exists x1:T, x2:int, x3:address. p
      /\mbox{$\backslash{}$} x4 = transaction(V, i, a)) /\mbox{$\backslash{}$} x4 = transaction(V, i, a)\} >>}}\) by
    \propref{semty/strengthen(push)}, from which we can derive
    \(\texttt{\textcolor{red}{<<no parses (char 28): G \mbox{$\mid$}= transaction(V, i, a) :.*** S : \{xTs \mbox{$\mid$} exists x1:T, x2:int,
      x3:address. p /\mbox{$\backslash{}$} x4 = transaction(V, i, a)\} >>}}\) by \ruleref{Sem-Push}.
    Finally, the goal follows by \propref{subty/sound}.
  \end{match}
\end{prop}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper.otex"
%%% End:


==> proofs/vtyping.tex <==
\begin{prop}[name=Every type is inhabited]{vtyping/inhabit}
  \AI{Used (implictly) in theorems of first-order logic.}
  For any \(\ottnt{T}\), there exists \(\ottnt{V}\) such that \( \ottnt{V}  :  \ottnt{T} \).

  \proof The proof is easy by structural induction on \(\ottnt{T}\).  Note that, for
  \(\ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}\), we have \( \ottnt{V_{{\mathrm{2}}}}  :  \ottnt{T_{{\mathrm{2}}}} \) for some \(\ottnt{V_{{\mathrm{2}}}}\) by the
  induction hypothesis, so choosing \(\ottnt{V}  \ottsym{=}   \langle  \ottsym{\{}  \ottkw{DROP}  \ottsym{;}  \ottsym{\{}  \ottkw{PUSH} \, \ottnt{T_{{\mathrm{2}}}} \, \ottnt{V_{{\mathrm{2}}}}  \ottsym{;}  \ottsym{\{}  \ottsym{\}}  \ottsym{\}}  \ottsym{\}}  \rangle \)
  suffices.
\end{prop}

\begin{prop}[name=Inversion for the value typing]{vtyping/inv}
  Every following statement holds.
  \begin{statements}
  \item[pair] If \( \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  :  \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}} \), then \( \ottnt{V_{{\mathrm{1}}}}  :  \ottnt{T_{{\mathrm{1}}}} \) and
    \( \ottnt{V_{{\mathrm{2}}}}  :  \ottnt{T_{{\mathrm{2}}}} \).
  \item[cons] If \( \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  :  \ottnt{T} \, \ottkw{list} \), then \( \ottnt{V_{{\mathrm{1}}}}  :  \ottnt{T} \) and \( \ottnt{V_{{\mathrm{2}}}}  :  \ottnt{T} \, \ottkw{list} \).
  \item[fun] If \(  \langle  \mathit{IS}  \rangle   :  \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}} \), then \(\ottnt{T_{{\mathrm{1}}}}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Rightarrow  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \ddagger\).
  \end{statements}

  \proof Easy by definition.
\end{prop}

\begin{prop}[name=Inversion for the simple typing]{styping/inv}
  Every following statement holds.
  \begin{statements}
  \item[nop] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottsym{\{}  \ottsym{\}}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \bar{T}_{{\mathrm{2}}} \).
  \item[seq] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottsym{\{}  \ottnt{I}  \ottsym{;}  \mathit{IS}  \ottsym{\}}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottnt{I}  \Rightarrow  \bar{T}\) and \(\bar{T}  \vdash  \mathit{IS}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\) for some \(\bar{T}\).
  \item[dip] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{DIP} \, \mathit{IS}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T}  \triangleright  \bar{T}'_{{\mathrm{1}}} \),
    \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T}  \triangleright  \bar{T}'_{{\mathrm{2}}} \), and \(\bar{T}'_{{\mathrm{1}}}  \vdash  \mathit{IS}  \Rightarrow  \bar{T}'_{{\mathrm{2}}}\)
    for some $\ottnt{T}, \bar{T}'_{{\mathrm{1}}}$, and $\bar{T}'_{{\mathrm{2}}}$.
  \item[drop] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{DROP}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T}  \triangleright  \bar{T}_{{\mathrm{2}}} \)
    for some $\ottnt{T}$.
  \item[dup] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{DUP}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T}  \triangleright  \bar{T} \) and
    \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T}  \triangleright  \ottnt{T}  \triangleright  \bar{T} \)
    for some $\ottnt{T}$, and $\bar{T}$.
  \item[swap] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{SWAP}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \triangleright  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T} \)
    and \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T_{{\mathrm{2}}}}  \triangleright  \ottnt{T_{{\mathrm{1}}}}  \triangleright  \bar{T} \)
    for some $\ottnt{T_{{\mathrm{1}}}}, \ottnt{T_{{\mathrm{2}}}}$, and $\bar{T}$.
  \item[push] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{PUSH} \, \ottnt{T} \, \ottnt{V}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T}  \triangleright  \bar{T}_{{\mathrm{1}}} \).
  \item[not] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{NOT}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T} \) and
    \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T} \) for some $\bar{T}$.
  \item[add] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{ADD}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottkw{int}  \triangleright  \ottkw{int}  \triangleright  \bar{T} \)
    and \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T} \) for some $\bar{T}$.
  \item[pair] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{PAIR}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \triangleright  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T} \)
    and \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T} \) for some $\ottnt{T_{{\mathrm{1}}}}, \ottnt{T_{{\mathrm{2}}}}$, and $\bar{T}$.
  \item[car] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{CAR}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T} \) and
    \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \triangleright  \bar{T} \) for some $\ottnt{T_{{\mathrm{1}}}}, \ottnt{T_{{\mathrm{2}}}}$, and $\bar{T}$.
  \item[cdr] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{CDR}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T} \) and
    \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T} \) for some $\ottnt{T_{{\mathrm{1}}}}, \ottnt{T_{{\mathrm{2}}}}$, and $\bar{T}$.
  \item[nil] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{NIL} \, \ottnt{T}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T}_{{\mathrm{1}}} \).
  \item[cons] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{CONS}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T}  \triangleright  \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T} \) and \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T} \)
     for some $\ottnt{T}$ and $\bar{T}$.
  \item[if] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{IF} \, \mathit{IS}_{{\mathrm{1}}} \, \mathit{IS}_{{\mathrm{2}}}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T} \),
    \(\bar{T}  \vdash  \mathit{IS}_{{\mathrm{1}}}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), and \(\bar{T}  \vdash  \mathit{IS}_{{\mathrm{2}}}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\).
     for some $\bar{T}$.
  \item[loop] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{LOOP} \, \mathit{IS}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T}_{{\mathrm{2}}} \) and
    \(\bar{T}_{{\mathrm{2}}}  \vdash  \mathit{IS}  \Rightarrow  \ottkw{int}  \triangleright  \bar{T}_{{\mathrm{2}}}\).
  \item[ifcons] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \texttt{IF\symbol{95}CONS} \, \mathit{IS}_{{\mathrm{1}}} \, \mathit{IS}_{{\mathrm{2}}}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T} \), \(\ottnt{T}  \triangleright  \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T}  \vdash  \mathit{IS}_{{\mathrm{1}}}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), and \(\bar{T}  \vdash  \mathit{IS}_{{\mathrm{2}}}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\)
     for some $\ottnt{T}$ and $\bar{T}$.
  \item[iter] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{ITER} \, \mathit{IS}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T}_{{\mathrm{2}}} \)
    and \(\ottnt{T}  \triangleright  \bar{T}_{{\mathrm{2}}}  \vdash  \mathit{IS}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\)
     for some $\ottnt{T}$.
  \item[lambda] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{LAMBDA} \, \ottnt{T_{{\mathrm{1}}}} \, \ottnt{T_{{\mathrm{2}}}} \, \mathit{IS}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T}_{{\mathrm{1}}} \) and \(\ottnt{T_{{\mathrm{1}}}}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Rightarrow  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \ddagger\).
  \item[exec] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \ottkw{EXEC}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \triangleright  \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T} \) and \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T} \)
     for some $\ottnt{T_{{\mathrm{1}}}}, \ottnt{T_{{\mathrm{2}}}}$, and $\bar{T}$.
  \item[transfertokens] If \(\bar{T}_{{\mathrm{1}}}  \vdash  \texttt{TRANSFER\symbol{95}TOKENS} \, \ottnt{T}  \Rightarrow  \bar{T}_{{\mathrm{2}}}\), then \( \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T}  \triangleright  \ottkw{int}  \triangleright  \ottkw{address}  \triangleright  \bar{T} \) and \( \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottkw{operation}  \triangleright  \bar{T} \)
     for some $\ottnt{T}$ and $\bar{T}$.
  \end{statements}

  \proof Easy by definition.
\end{prop}

\begin{prop}[name=Inversion for the stack typing]{st/inv}
  Every following statement holds.
  \begin{statements}
  \item[bottom] If \( \ddagger  :  \bar{T} \), then \( \bar{T} \ottsym{=} \ddagger \).
  \item[push] If \( \ottnt{V}  \triangleright  \ottnt{S}  :  \bar{T} \), then \( \bar{T} \ottsym{=} \ottnt{T}  \triangleright  \bar{T}' \), \( \ottnt{V}  :  \ottnt{T} \), and \( \ottnt{S}  :  \bar{T}' \) for some \(\ottnt{T}\) and \(\bar{T}'\).
  \end{statements}

  \proof Easy by definition.
\end{prop}

\begin{prop}[name=Soundness of the simple type system]{styping/sound}
  The following two statements hold.
  \begin{statements}
  \item If
    \begin{gather}
      \bar{T}_{{\mathrm{1}}}  \vdash  \mathit{IS}  \Rightarrow  \bar{T}_{{\mathrm{2}}} \hyp{typing1}\\
      \ottnt{S_{{\mathrm{1}}}}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{eval1}\\
       \ottnt{S_{{\mathrm{1}}}}  :  \bar{T}_{{\mathrm{1}}}  \hyp{wf1}
    \end{gather}
    then \( \ottnt{S_{{\mathrm{2}}}}  :  \bar{T}_{{\mathrm{2}}} \).
  \item If
    \begin{gather}
      \bar{T}_{{\mathrm{1}}}  \vdash  \ottnt{I}  \Rightarrow  \bar{T}_{{\mathrm{2}}} \hyp{typing2}\\
      \ottnt{S_{{\mathrm{1}}}}  \vdash  \ottnt{I}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{eval2}\\
       \ottnt{S_{{\mathrm{1}}}}  :  \bar{T}_{{\mathrm{1}}}  \hyp{wf2}
    \end{gather}
    then \( \ottnt{S_{{\mathrm{2}}}}  :  \bar{T}_{{\mathrm{2}}} \).
  \end{statements}

  \proof The proof is straightforward by mutual induction on the given derivation of
  \hypref{eval1} and \hypref{eval2} with case analysis on the last rule used and
  \propref{vtyping/inv}, \propref{styping/inv}, and \propref{st/inv}.  We show
  only the case for \ruleref{E-Exec} in detail.  The others are shown in a
  similar manner.

  Note that we can't prove this by mutual induction on the given derivation of
  \hypref{typing1} and \hypref{typing2} because of the \(\ottkw{EXEC}\) case.
  \begin{match}
  \item[\ruleref{E-Exec}] We have
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{EXEC}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright   \langle  \mathit{IS}  \rangle   \triangleright  \ottnt{S}  \hyp{2}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V'}  \triangleright  \ottnt{S}  \hyp{3}\\
      \ottnt{V}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Downarrow  \ottnt{V'}  \triangleright  \ddagger \hyp{4IH}
    \end{gather}
    for some $\ottnt{V}$, $\mathit{IS}$, $\ottnt{S}$, and $\ottnt{V'}$.  By
    \propref{styping/inv(exec)}, \hypref{typing2}, and \hypref{1}, we have
    \begin{gather}
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \triangleright  \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T}  \hyp{5}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T}  \hyp{6}
    \end{gather}
    for some $\ottnt{T_{{\mathrm{1}}}}$, $\ottnt{T_{{\mathrm{2}}}}$, and $\bar{T}$.  By \propref{vtyping/inv},
    \propref{st/inv}, \hypref{wf2}, \hypref{2}, and \hypref{5}, we have
    \begin{gather}
       \ottnt{V}  :  \ottnt{T_{{\mathrm{1}}}}  \hyp{7}\\
      \ottnt{T_{{\mathrm{1}}}}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Rightarrow  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \ddagger \hyp{8}\\
       \ottnt{S}  :  \bar{T}  \hyp{9}
    \end{gather}
    Thus, \( \ottnt{V}  \triangleright  \ddagger  :  \ottnt{T_{{\mathrm{1}}}}  \triangleright  \ddagger \) by \ruleref{ST-Bottom}, \ruleref{ST-Push},
    and \hypref{7}.  Then, \( \ottnt{V'}  \triangleright  \ddagger  :  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \ddagger \) by IH, \hypref{4IH}, and
    \hypref{8}.  Now, \( \ottnt{V'}  :  \ottnt{T_{{\mathrm{2}}}} \) by \propref{st/inv(push)}.  Finally, the goal
    \( \ottnt{V'}  \triangleright  \ottnt{S}  :  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T} \)can be derived by \ruleref{ST-Push} and
    \hypref{9}. \qedhere
  \end{match}

\begin{comment}
  \proof The proof is done by induction on the given derivation of
  \hypref{eval}.
  \begin{match}
  \item[\ruleref{E-Nop}] We have the following hypothesis.
    \begin{gather}
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{S_{{\mathrm{2}}}}  \hyp{1}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \bar{T}_{{\mathrm{2}}}  \hyp{2}
    \end{gather}
    So, the goal is equivalent to \hypref{wf}.
    
  \item[\ruleref{E-Seq}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottsym{\{}  \ottnt{I_{{\mathrm{1}}}}  \ottsym{;}  \ottnt{I_{{\mathrm{2}}}}  \ottsym{;} \, ... \, \ottsym{;}  \ottnt{I_{\ottmv{n}}}  \ottsym{\}}  \hyp{1}\\
      \ottnt{S_{{\mathrm{1}}}}  \vdash  \ottnt{I_{{\mathrm{1}}}}  \Downarrow  \ottnt{S} \hyp{2IH}\\
      \ottnt{S}  \vdash  \ottsym{\{}  \ottnt{I_{{\mathrm{2}}}}  \ottsym{;} \, ... \, \ottsym{;}  \ottnt{I_{\ottmv{n}}}  \ottsym{\}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{3IH}\\
      \bar{T}_{{\mathrm{1}}}  \vdash  \ottnt{I_{{\mathrm{1}}}}  \Rightarrow  \bar{T} \hyp{4}\\
      \bar{T}  \vdash  \ottsym{\{}  \ottnt{I_{{\mathrm{2}}}}  \ottsym{;} \, ... \, \ottsym{;}  \ottnt{I_{\ottmv{n}}}  \ottsym{\}}  \Rightarrow  \bar{T}_{{\mathrm{2}}} \hyp{5}
    \end{gather}
    So, \( \ottnt{S}  :  \bar{T} \) follows by IH, \hypref{wf}, \hypref{2IH}, \hypref{4};
    and then, the goal follosw by IH, \hypref{3IH}, \hypref{5}.
    
  \item[\ruleref{E-Dip}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{DIP} \, \mathit{IS}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S'_{{\mathrm{1}}}}  \hyp{2}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S'_{{\mathrm{2}}}}  \hyp{3}\\
      \ottnt{S'_{{\mathrm{1}}}}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S'_{{\mathrm{2}}}} \hyp{4IH}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T}  \triangleright  \bar{T}'_{{\mathrm{1}}}  \hyp{5}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T}  \triangleright  \bar{T}'_{{\mathrm{2}}}  \hyp{6}\\
      \bar{T}'_{{\mathrm{1}}}  \vdash  \mathit{IS}  \Rightarrow  \bar{T}'_{{\mathrm{2}}} \hyp{7}\\
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}} \hyp{8}\\
       \ottnt{S'_{{\mathrm{1}}}}  :  \bar{T}'_{{\mathrm{1}}}  \hyp{9}
    \end{gather}
    So, \( \ottnt{S'_{{\mathrm{2}}}}  :  \bar{T}'_{{\mathrm{2}}} \) follows by IH, \hypref{4IH}, \hypref{7},
    \hypref{9}.  Then, the goal follows by \ruleref{ST-Push}.
    
  \item[\ruleref{E-Drop}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{DROP}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S_{{\mathrm{2}}}}  \hyp{2}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T}  \triangleright  \bar{T}_{{\mathrm{2}}}  \hyp{3}
    \end{gather}
    So, the goal follows by \propref{st/inv}, \hypref{wf}.

  \item[\ruleref{E-Dup}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{DUP}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S}  \hyp{2}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{V}  \triangleright  \ottnt{S}  \hyp{3}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T}  \triangleright  \bar{T}  \hyp{4}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T}  \triangleright  \ottnt{T}  \triangleright  \bar{T}  \hyp{5}\\
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}} \hyp{6}\\
       \ottnt{S}  :  \bar{T}  \hyp{7}
    \end{gather}
    So, the goal can be derived by \ruleref{ST-Push}, \hypref{6}, \hypref{7}.

  \item[\ruleref{E-Swap}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{SWAP}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{2}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{S}  \hyp{3}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \triangleright  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T}  \hyp{4}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T_{{\mathrm{2}}}}  \triangleright  \ottnt{T_{{\mathrm{1}}}}  \triangleright  \bar{T}  \hyp{5}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T1 >>}} \hyp{6}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T2 >>}} \hyp{7}\\
       \ottnt{S}  :  \bar{T}  \hyp{8}
    \end{gather}
    So, the goal can be derived by \ruleref{ST-Push}, \hypref{6}, \hypref{7},
    \hypref{8}.

  \item[\ruleref{E-Push}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{PUSH} \, \ottnt{T} \, \ottnt{V}  \hyp{1}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{S_{{\mathrm{1}}}}  \hyp{2}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T}  \triangleright  \bar{T}_{{\mathrm{1}}}  \hyp{3}\\
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}} \hyp{4}
    \end{gather}
    So, the goal can be derived by \ruleref{ST-Push}, \hypref{wf}, \hypref{4}.
    
  \item[\ruleref{E-NotT}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{NOT}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{i}  \triangleright  \ottnt{S}  \hyp{2}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} 0  \triangleright  \ottnt{S}  \hyp{3}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T}  \hyp{5}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T}  \hyp{6}\\
       \ottnt{S}  :  \bar{T}  \hyp{7}
    \end{gather}
    So, the goal can be derived by \ruleref{RTV-Int}, \ruleref{ST-Push},
    \hypref{7}.
    
  \item[\ruleref{E-NotF}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{NOT}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} 0  \triangleright  \ottnt{S}  \hyp{2}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} 1  \triangleright  \ottnt{S}  \hyp{3}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T}  \hyp{5}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T}  \hyp{6}\\
       \ottnt{S}  :  \bar{T}  \hyp{7}
    \end{gather}
    So, the goal can be derived by \ruleref{RTV-Int}, \ruleref{ST-Push},
    \hypref{7}.
    
  \item[\ruleref{E-Add}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{ADD}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{i_{{\mathrm{1}}}}  \triangleright  \ottnt{i_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{2}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{i_{{\mathrm{3}}}}  \triangleright  \ottnt{S}  \hyp{3}\\
       \ottnt{i_{{\mathrm{1}}}}  \ottsym{+}  \ottnt{i_{{\mathrm{2}}}} \ottsym{=} \ottnt{i_{{\mathrm{3}}}}  \hyp{4}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottkw{int}  \triangleright  \ottkw{int}  \triangleright  \bar{T}  \hyp{5}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T}  \hyp{6}\\
       \ottnt{S}  :  \bar{T}  \hyp{7}
    \end{gather}
    So, the goal can be derived by \ruleref{RTV-Int}, \ruleref{ST-Push},
    \hypref{7}.
    
  \item[\ruleref{E-Pair}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{PAIR}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{2}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \triangleright  \ottnt{S}  \hyp{3}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \triangleright  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T}  \hyp{4}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T}  \hyp{5}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T1 >>}} \hyp{6}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T2 >>}} \hyp{7}\\
       \ottnt{S}  :  \bar{T}  \hyp{8}
    \end{gather}
    So, the goal can be derived by \ruleref{RTV-Pair}, \ruleref{ST-Push},
    \hypref{6}, \hypref{7}, \hypref{8}.
    
  \item[\ruleref{E-CAR}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{CAR}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \triangleright  \ottnt{S}  \hyp{2}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{S}  \hyp{3}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T}  \hyp{4}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \triangleright  \bar{T}  \hyp{5}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T1 >>}} \hyp{6}\\
       \ottnt{S}  :  \bar{T}  \hyp{7}
    \end{gather}
    So, the goal can be derived by \ruleref{ST-Push}, \hypref{6}, \hypref{7}.
    
  \item[\ruleref{E-CDR}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{CDR}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{(}  \ottnt{V_{{\mathrm{1}}}}  \ottsym{,}  \ottnt{V_{{\mathrm{2}}}}  \ottsym{)}  \triangleright  \ottnt{S}  \hyp{2}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{3}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \times  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T}  \hyp{4}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T}  \hyp{5}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T2 >>}} \hyp{6}\\
       \ottnt{S}  :  \bar{T}  \hyp{7}
    \end{gather}
    So, the goal can be derived by \ruleref{ST-Push}, \hypref{6}, \hypref{7}.
    
  \item[\ruleref{E-Nil}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{NIL} \, \ottnt{T}  \hyp{1}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottsym{[}  \ottsym{]}  \triangleright  \ottnt{S_{{\mathrm{1}}}}  \hyp{2}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T}_{{\mathrm{1}}}  \hyp{3}
    \end{gather}
    So, the goal can be derived by \ruleref{RTV-Nil}, \ruleref{ST-Push},
    \hypref{wf}.
    
  \item[\ruleref{E-Cons}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{CONS}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{2}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{3}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T}  \triangleright  \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T}  \hyp{4}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T}  \hyp{5}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T >>}} \hyp{6}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T list >>}} \hyp{7}\\
       \ottnt{S}  :  \bar{T}  \hyp{8}
    \end{gather}
    So, the goal can be derived by \ruleref{RTV-Cons}, \ruleref{ST-Push},
    \hypref{6}, \hypref{7}, \hypref{8}.
    
  \item[\ruleref{E-IfT}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{IF} \, \mathit{IS}_{{\mathrm{1}}} \, \mathit{IS}_{{\mathrm{2}}}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{i}  \triangleright  \ottnt{S}  \hyp{2}\\
      \ottnt{S}  \vdash  \mathit{IS}_{{\mathrm{1}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{3IH}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T}  \hyp{4}\\
      \bar{T}  \vdash  \mathit{IS}_{{\mathrm{1}}}  \Rightarrow  \bar{T}_{{\mathrm{2}}} \hyp{5}\\
       \ottnt{S}  :  \bar{T}  \hyp{6}
    \end{gather}
    So, the goal follows by IH, \hypref{3IH}, \hypref{5}, \hypref{6}.
    
  \item[\ruleref{E-IfF}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{IF} \, \mathit{IS}_{{\mathrm{1}}} \, \mathit{IS}_{{\mathrm{2}}}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} 0  \triangleright  \ottnt{S}  \hyp{2}\\
      \ottnt{S}  \vdash  \mathit{IS}_{{\mathrm{2}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{3IH}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T}  \hyp{4}\\
      \bar{T}  \vdash  \mathit{IS}_{{\mathrm{2}}}  \Rightarrow  \bar{T}_{{\mathrm{2}}} \hyp{5}\\
       \ottnt{S}  :  \bar{T}  \hyp{6}
    \end{gather}
    So, the goal follows by IH, \hypref{3IH}, \hypref{5}, \hypref{6}.
    
  \item[\ruleref{E-LoopT}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{LOOP} \, \mathit{IS}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{i}  \triangleright  \ottnt{S}  \hyp{2}\\
      \ottnt{S}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S'} \hyp{3IH}\\
      \ottnt{S'}  \vdash  \ottkw{LOOP} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{4IH}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T}_{{\mathrm{2}}}  \hyp{5}\\
      \bar{T}_{{\mathrm{2}}}  \vdash  \mathit{IS}  \Rightarrow  \ottkw{int}  \triangleright  \bar{T}_{{\mathrm{2}}} \hyp{6}\\
       \ottnt{S}  :  \bar{T}_{{\mathrm{2}}}  \hyp{7}
    \end{gather}
    So, \( \ottnt{S'}  :  \ottkw{int}  \triangleright  \bar{T}_{{\mathrm{2}}} \) follows by IH, \hypref{3IH}, \hypref{6},
    \hypref{7}.  Then, the goal follows by IH, \hypref{4IH}, \hypref{typing}.
    
  \item[\ruleref{E-LoopF}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{LOOP} \, \mathit{IS}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} 0  \triangleright  \ottnt{S_{{\mathrm{2}}}}  \hyp{2}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottkw{int}  \triangleright  \bar{T}_{{\mathrm{2}}}  \hyp{3}\\
       \ottnt{S_{{\mathrm{2}}}}  :  \bar{T}_{{\mathrm{2}}}  \hyp{4}
    \end{gather}
    The goal is \hypref{4}.
    
  \item[\ruleref{E-IfConsT}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \texttt{IF\symbol{95}CONS} \, \mathit{IS}_{{\mathrm{1}}} \, \mathit{IS}_{{\mathrm{2}}}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{2}\\
      \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \vdash  \mathit{IS}_{{\mathrm{1}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{3IH}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T}  \hyp{3}\\
      \ottnt{T}  \triangleright  \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T}  \vdash  \mathit{IS}_{{\mathrm{1}}}  \Rightarrow  \bar{T}_{{\mathrm{2}}} \hyp{4}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T >>}} \hyp{5}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T list >>}} \hyp{6}\\
       \ottnt{S}  :  \bar{T}  \hyp{7}
    \end{gather}
    We have \( \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  :  \ottnt{T}  \triangleright  \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T} \) by \ruleref{ST-Push},
    \hypref{5}, \hypref{6}, \hypref{7}.  So, the goal follows by IH,
    \hypref{3IH}, \hypref{4}.
    
  \item[\ruleref{E-IfConsF}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \texttt{IF\symbol{95}CONS} \, \mathit{IS}_{{\mathrm{1}}} \, \mathit{IS}_{{\mathrm{2}}}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{[}  \ottsym{]}  \triangleright  \ottnt{S}  \hyp{2}\\
      \ottnt{S}  \vdash  \mathit{IS}_{{\mathrm{2}}}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{3IH}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T}  \hyp{4}\\
      \bar{T}  \vdash  \mathit{IS}_{{\mathrm{2}}}  \Rightarrow  \bar{T}_{{\mathrm{2}}} \hyp{5}\\
       \ottnt{S}  :  \bar{T}  \hyp{6}
    \end{gather}
    So, the goal follows by IH, \hypref{3IH}, \hypref{5}, \hypref{6}.
    
  \item[\ruleref{E-IterNil}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{ITER} \, \mathit{IS}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottsym{[}  \ottsym{]}  \triangleright  \ottnt{S_{{\mathrm{2}}}}  \hyp{2}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T}_{{\mathrm{2}}}  \hyp{3}\\
       \ottnt{S_{{\mathrm{2}}}}  :  \bar{T}_{{\mathrm{2}}}  \hyp{4}
    \end{gather}
    So, the goal is \hypref{4}

  \item[\ruleref{E-IterCons}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{ITER} \, \mathit{IS}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V_{{\mathrm{1}}}}  ::  \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S}  \hyp{2}\\
      \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{S}  \vdash  \mathit{IS}  \Downarrow  \ottnt{S'} \hyp{3IH}\\
      \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S'}  \vdash  \ottkw{ITER} \, \mathit{IS}  \Downarrow  \ottnt{S_{{\mathrm{2}}}} \hyp{4IH}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T}_{{\mathrm{2}}}  \hyp{5}\\
      \ottnt{T}  \triangleright  \bar{T}_{{\mathrm{2}}}  \vdash  \mathit{IS}  \Rightarrow  \bar{T}_{{\mathrm{2}}} \hyp{6}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V1 : ***T >>}} \hyp{7}\\
      \texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V2 : ***T list >>}} \hyp{8}\\
       \ottnt{S}  :  \bar{T}_{{\mathrm{2}}}  \hyp{9}
    \end{gather}
    So, \( \ottnt{V_{{\mathrm{1}}}}  \triangleright  \ottnt{S}  :  \ottnt{T}  \triangleright  \bar{T}_{{\mathrm{2}}} \) by \ruleref{ST-Push}, \hypref{7},
    \hypref{9}.  Then, \( \ottnt{S'}  :  \bar{T}_{{\mathrm{2}}} \) by IH, \hypref{3IH}, \hypref{6}.
    Now, \( \ottnt{V_{{\mathrm{2}}}}  \triangleright  \ottnt{S'}  :  \ottnt{T} \, \ottkw{list}  \triangleright  \bar{T}_{{\mathrm{2}}} \) by \ruleref{ST-Push}, \hypref{8}.
    Finally, the goal follows by IH, \hypref{4IH}, \hypref{typing}.

  \item[\ruleref{E-Lambda}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{LAMBDA} \, \ottnt{T_{{\mathrm{1}}}} \, \ottnt{T_{{\mathrm{2}}}} \, \mathit{IS}  \hyp{1}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=}  \langle  \mathit{IS}  \rangle   \triangleright  \ottnt{S_{{\mathrm{1}}}}  \hyp{2}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T}_{{\mathrm{1}}}  \hyp{3}\\
      \ottnt{T_{{\mathrm{1}}}}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Rightarrow  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \ddagger \hyp{4}
    \end{gather}
    The goal can be derived by \ruleref{RTV-Fun}, \ruleref{ST-Push},
    \hypref{wf}, \hypref{3}.
    
  \item[\ruleref{E-Exec}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \ottkw{EXEC}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright   \langle  \mathit{IS}  \rangle   \triangleright  \ottnt{S}  \hyp{2}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=} \ottnt{V'}  \triangleright  \ottnt{S}  \hyp{3}\\
      \ottnt{V}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Downarrow  \ottnt{V'}  \triangleright  \ddagger \hyp{4IH}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T_{{\mathrm{1}}}}  \triangleright  \ottnt{T_{{\mathrm{1}}}}  \to  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T}  \hyp{5}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottnt{T_{{\mathrm{2}}}}  \triangleright  \bar{T}  \hyp{6}\\
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T1 >>}} \hyp{7}\\
      \ottnt{T_{{\mathrm{1}}}}  \triangleright  \ddagger  \vdash  \mathit{IS}  \Rightarrow  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \ddagger \hyp{8}\\
       \ottnt{S}  :  \bar{T}  \hyp{9}
    \end{gather}
    So, \( \ottnt{V}  \triangleright  \ddagger  :  \ottnt{T_{{\mathrm{1}}}}  \triangleright  \ddagger \) by \ruleref{ST-Bottom}, \ruleref{ST-Push},
    \hypref{7}.  Then, \( \ottnt{V'}  \triangleright  \ddagger  :  \ottnt{T_{{\mathrm{2}}}}  \triangleright  \ddagger \) by IH, \hypref{4IH},
    \hypref{8}.  Now, \(\texttt{\textcolor{red}{<<no parses (char 8): \mbox{$\mid$}= V' : ***T2 >>}}\) by \propref{st/inv}.  Finally, the goal
    can be derived by \ruleref{ST-Push}, \hypref{9}.
    
  \item[\ruleref{E-TransferTokens}] We have the following hypothesis.
    \begin{gather}
       \ottnt{I} \ottsym{=} \texttt{TRANSFER\symbol{95}TOKENS} \, \ottnt{T}  \hyp{1}\\
       \ottnt{S_{{\mathrm{1}}}} \ottsym{=} \ottnt{V}  \triangleright  \ottnt{i}  \triangleright  \ottnt{a}  \triangleright  \ottnt{S}  \hyp{2}\\
       \ottnt{S_{{\mathrm{2}}}} \ottsym{=}  \texttt{Transfer}  (  \ottnt{V} ,  \ottnt{i} ,  \ottnt{a}  )   \triangleright  \ottnt{S}  \hyp{3}\\
       \bar{T}_{{\mathrm{1}}} \ottsym{=} \ottnt{T}  \triangleright  \ottkw{int}  \triangleright  \ottkw{address}  \triangleright  \bar{T}  \hyp{4}\\
       \bar{T}_{{\mathrm{2}}} \ottsym{=} \ottkw{operation}  \triangleright  \bar{T}  \hyp{5}\\
      \texttt{\textcolor{red}{<<no parses (char 7): \mbox{$\mid$}= V : ***T >>}} \hyp{6}\\
       \ottnt{S}  :  \bar{T}  \hyp{9}
    \end{gather}
    We can derive \(\texttt{\textcolor{red}{<<no parses (char 27): \mbox{$\mid$}= transaction (V, i, a) : ***operation >>}}\) by
    \ruleref{RTV-Operation}, \hypref{6}.  So, the goal can be derived by
    \ruleref{ST-Push}, \hypref{9}.
  \end{match}
\end{comment}
\end{prop}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper.otex"
%%% End:

